A JWST/MIRI view of k Andromedae b: Refining its mass, age, and physical parameters

Context. kAndb is a substellar companion near the planet-brown dwarf boundary, orbiting a B9IV star at 50-100 au. Estimates of its age and mass vary, fueling a decade-long debate. Atmospheric parameters (Teff 1650-2050 K, log(g) 3.5-5.5) remain poorly constrained due to model differences and heterogeneous datasets. Aims. We refine the characterization of kAndb using mid-infrared data to capture its bolometric emission. Combined with NIR measurements, we constrain Teff, log(g), and radius to reduce uncertainties in age and mass. Methods. We obtained JWST/MIRI coronagraphic data (F1065C, F1140C, F1550C) and recalibrated NIR photometry with an updated ATLAS stellar model. MIRI color-magnitude diagrams (CMDs) probe the likelihood of species (CH4, NH3, silicates). We compared H and F1140C colors and magnitudes to isochrones to constrain age and mass. We modeled the spectral energy distribution with atmosphere models to refine Teff, radius, and log(g), and to constrain age and mass using evolutionary models. Results. Cloudy atmosphere models fit best, consistent with the L0/L2 spectral type and position near silicate-atmosphere field objects in the MIRI CMD. We derived an age of 47+-7 Myr and mass of 17.3+-1.8 MJup by weighted-mean model combination. Modeling yielded Teff = 1791+-68 K and radius = 1.42+-0.06 RJup, improving precision by 30%. Log(g) = 4.35+-0.07 dex represents a 70% improvement over the previous best value (4.75+-0.25). Conclusions. The new mass places kAndb just above the deuterium-burning limit. The age is 75% more precise and consistent with the Columba association (42 Myr). The Teff suggests silicate clouds, requiring spectroscopic confirmation. MIRI data were crucial to refining radius and temperature, which led to stronger constraints on age and mass and improving the overall characterization of kAndb.

==> kappaAnd_JWST_bib.tex <==

@ARTICLE{Carter+2022,
       author = {{Carter}, Aarynn L. and {Hinkley}, Sasha and {Kammerer}, Jens and {Skemer}, Andrew and {Biller}, Beth A. and {Leisenring}, Jarron M. and {Millar-Blanchaer}, Maxwell A. and {Petrus}, Simon and {Stone}, Jordan M. and {Ward-Duong}, Kimberly and {Wang}, Jason J. and {Girard}, Julien H. and {Hines}, Dean C. and {Perrin}, Marshall D. and {Pueyo}, Laurent and {Balmer}, William O. and {Bonavita}, Mariangela and {Bonnefoy}, Mickael and {Chauvin}, Gael and {Choquet}, Elodie and {Christiaens}, Valentin and {Danielski}, Camilla and {Kennedy}, Grant M. and {Matthews}, Elisabeth C. and {Miles}, Brittany E. and {Patapis}, Polychronis and {Ray}, Shrishmoy and {Rickman}, Emily and {Sallum}, Steph and {Stapelfeldt}, Karl R. and {Whiteford}, Niall and {Zhou}, Yifan and {Absil}, Olivier and {Boccaletti}, Anthony and {Booth}, Mark and {Bowler}, Brendan P. and {Chen}, Christine H. and {Currie}, Thayne and {Fortney}, Jonathan J. and {Grady}, Carol A. and {Greebaum}, Alexandra Z. and {Henning}, Thomas and {Hoch}, Kielan K.~W. and {Janson}, Markus and {Kalas}, Paul and {Kenworthy}, Matthew A. and {Kervella}, Pierre and {Kraus}, Adam L. and {Lagage}, Pierre-Olivier and {Liu}, Michael C. and {Macintosh}, Bruce and {Marino}, Sebastian and {Marley}, Mark S. and {Marois}, Christian and {Matthews}, Brenda C. and {Mawet}, Dimitri and {McElwain}, Michael W. and {Metchev}, Stanimir and {Meyer}, Michael R. and {Molliere}, Paul and {Moran}, Sarah E. and {Morley}, Caroline V. and {Mukherjee}, Sagnick and {Pantin}, Eric and {Quirrenbach}, Andreas and {Rebollido}, Isabel and {Ren}, Bin B. and {Schneider}, Glenn and {Vasist}, Malavika and {Worthen}, Kadin and {Wyatt}, Mark C. and {Briesemeister}, Zackery W. and {Bryan}, Marta L. and {Calissendorff}, Per and {Cantalloube}, Faustine and {Cugno}, Gabriele and {De Furio}, Matthew and {Dupuy}, Trent J. and {Factor}, Samuel M. and {Faherty}, Jacqueline K. and {Fitzgerald}, Michael P. and {Franson}, Kyle and {Gonzales}, Eileen C. and {Hood}, Callie E. and {Howe}, Alex R. and {Kuzuhara}, Masayuki and {Lagrange}, Anne-Marie and {Lawson}, Kellen and {Lazzoni}, Cecilia and {Lew}, Ben W.~P. and {Liu}, Pengyu and {Llop-Sayson}, Jorge and {Lloyd}, James P. and {Martinez}, Raquel A. and {Mazoyer}, Johan and {Palma-Bifani}, Paulina and {Quanz}, Sascha P. and {Redai}, Jea Adams and {Samland}, Matthias and {Schlieder}, Joshua E. and {Tamura}, Motohide and {Tan}, Xianyu and {Uyama}, Taichi and {Vigan}, Arthur and {Vos}, Johanna M. and {Wagner}, Kevin and {Wolff}, Schuyler G. and {Ygouf}, Marie and {Zhang}, Xi and {Zhang}, Keming and {Zhang}, Zhoujian},
        title = "{The JWST Early Release Science Program for Direct Observations of Exoplanetary Systems I: High-contrast Imaging of the Exoplanet HIP 65426 b from 2 to 16 {\ensuremath{\mu}}m}",
      journal = {\apjl},
     keywords = {Exoplanets, Exoplanet astronomy, Extrasolar gaseous planets, 498, 486, 2172, Astrophysics - Earth and Planetary Astrophysics},
         year = 2023,
        month = jul,
       volume = {951},
       number = {1},
          eid = {L20},
        pages = {L20},
          doi = {10.3847/2041-8213/acd93e},
archivePrefix = {arXiv},
       eprint = {2208.14990},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...951L..20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang+2023,
       author = {{Zhang}, Stella Yimiao and {Duch{\^e}ne}, Gaspard and {De Rosa}, Robert J. and {Ansdell}, Megan and {Konopacky}, Quinn and {Esposito}, Thomas and {Chiang}, Eugene and {Rice}, Malena and {Matthews}, Brenda and {Kalas}, Paul and {Macintosh}, Bruce and {Marchis}, Franck and {Metchev}, Stan and {Patience}, Jenny and {Rameau}, Julien and {Ward-Duong}, Kimberly and {Wolff}, Schuyler and {Fitzgerald}, Michael P. and {Bailey}, Vanessa P. and {Barman}, Travis S. and {Bulger}, Joanna and {Chen}, Christine H. and {Chilcotte}, Jeffrey K. and {Cotten}, Tara and {Doyon}, Ren{\'e} and {Follette}, Katherine B. and {Gerard}, Benjamin L. and {Goodsell}, Stephen and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Maire}, J{\'e}r{\^o}me and {Marley}, Mark S. and {Marois}, Christian and {Millar-Blanchaer}, Maxwell A. and {Nielsen}, Eric L. and {Oppenheimer}, Rebecca and {Palmer}, David W. and {Perrin}, Marshall D. and {Poyneer}, Lisa A. and {Pueyo}, Laurent and {Rajan}, Abhijith and {Rantakyr{\"o}}, Fredrik T. and {Ruffio}, Jean-Baptiste and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wang}, Jason J. and {Wiktorowicz}, Sloane J.},
        title = "{Testing the Interaction between a Substellar Companion and a Debris Disk in the HR 2562 System}",
      journal = {\aj},
     keywords = {Debris disks, Substellar companion stars, Brown dwarfs, Orbit determination, Gravitational interaction, 363, 1648, 185, 1175, 669},
         year = 2023,
        month = may,
       volume = {165},
       number = {5},
          eid = {219},
        pages = {219},
          doi = {10.3847/1538-3881/acbafb},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....165..219Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mesa+2018,
       author = {{Mesa}, D. and {Baudino}, J. -L. and {Charnay}, B. and {D'Orazi}, V. and {Desidera}, S. and {Boccaletti}, A. and {Gratton}, R. and {Bonnefoy}, M. and {Delorme}, P. and {Langlois}, M. and {Vigan}, A. and {Zurlo}, A. and {Maire}, A. -L. and {Janson}, M. and {Antichi}, J. and {Baruffolo}, A. and {Bruno}, P. and {Cascone}, E. and {Chauvin}, G. and {Claudi}, R.~U. and {De Caprio}, V. and {Fantinel}, D. and {Farisato}, G. and {Feldt}, M. and {Giro}, E. and {Hagelberg}, J. and {Incorvaia}, S. and {Lagadec}, E. and {Lagrange}, A. -M. and {Lazzoni}, C. and {Lessio}, L. and {Salasnich}, B. and {Scuderi}, S. and {Sissa}, E. and {Turatto}, M.},
        title = "{New spectro-photometric characterization of the substellar object HR 2562 B using SPHERE}",
      journal = {\aap},
     keywords = {instrumentation: spectrographs, methods: data analysis, techniques: imaging spectroscopy, planetary systems, stars: late-type, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = may,
       volume = {612},
          eid = {A92},
        pages = {A92},
          doi = {10.1051/0004-6361/201731649},
archivePrefix = {arXiv},
       eprint = {1712.05828},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A\&A...612A..92M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moor+2006,
       author = {{Mo{\'o}r}, A. and {{\'A}brah{\'a}m}, P. and {Derekas}, A. and {Kiss}, Cs. and {Kiss}, L.~L. and {Apai}, D. and {Grady}, C. and {Henning}, Th.},
        title = "{Nearby Debris Disk Systems with High Fractional Luminosity Reconsidered}",
      journal = {\apj},
     keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Kinematics, Astrophysics},
         year = 2006,
        month = jun,
       volume = {644},
       number = {1},
        pages = {525-542},
          doi = {10.1086/503381},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603729},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...644..525M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Moor+2015,
       author = {{Mo{\'o}r}, A. and {K{\'o}sp{\'a}l}, {\'A}. and {{\'A}brah{\'a}m}, P. and {Apai}, D. and {Balog}, Z. and {Grady}, C. and {Henning}, Th. and {Juh{\'a}sz}, A. and {Kiss}, Cs. and {Krivov}, A.~V. and {Pawellek}, N. and {Szab{\'o}}, Gy. M.},
        title = "{Stirring in massive, young debris discs from spatially resolved Herschel images}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: individual: HD 9672, stars: individual: HD 16743, stars: individual: HD 21997, stars: individual: HD 95086, infrared: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = feb,
       volume = {447},
       number = {1},
        pages = {577-597},
          doi = {10.1093/mnras/stu2442},
archivePrefix = {arXiv},
       eprint = {1411.5829},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447..577M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moor+2011,
       author = {{Mo{\'o}r}, A. and {Pascucci}, I. and {K{\'o}sp{\'a}l}, {\'A}. and {{\'A}brah{\'a}m}, P. and {Csengeri}, T. and {Kiss}, L.~L. and {Apai}, D. and {Grady}, C. and {Henning}, Th. and {Kiss}, Cs. and {Bayliss}, D. and {Juh{\'a}sz}, A. and {Kov{\'a}cs}, J. and {Szalai}, T.},
        title = "{Structure and Evolution of Debris Disks Around F-type Stars. I. Observations, Database, and Basic Evolutionary Aspects}",
      journal = {\apjs},
     keywords = {circumstellar matter, infrared: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = mar,
       volume = {193},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1088/0067-0049/193/1/4},
archivePrefix = {arXiv},
       eprint = {1012.3631},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..193....4M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Asiain+1999,
       author = {{Asiain}, R. and {Figueras}, F. and {Torra}, J. and {Chen}, B.},
        title = "{Detection of moving groups among early type stars}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: FUNDAMENTAL PARAMETERS, STARS: HERTZSPRUNG-RUSSEL (HR) AND C-M DIAGRAMS, STARS: KINEMATICS GALAXY: SOLAR NEIGHBOURHOOD},
         year = 1999,
        month = jan,
       volume = {341},
        pages = {427-436},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A\&A...341..427A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rhee+2007,
       author = {{Rhee}, Joseph H. and {Song}, Inseok and {Zuckerman}, B. and {McElwain}, Michael},
        title = "{Characterization of Dusty Debris Disks: The IRAS and Hipparcos Catalogs}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Planetary Systems: Protoplanetary Disks, Astrophysics},
         year = 2007,
        month = may,
       volume = {660},
       number = {2},
        pages = {1556-1571},
          doi = {10.1086/509912},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609555},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...660.1556R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Konopacky+2016,
       author = {{Konopacky}, Quinn M. and {Rameau}, Julien and {Duch{\^e}ne}, Gaspard and {Filippazzo}, Joseph C. and {Giorla Godfrey}, Paige A. and {Marois}, Christian and {Nielsen}, Eric L. and {Pueyo}, Laurent and {Rafikov}, Roman R. and {Rice}, Emily L. and {Wang}, Jason J. and {Ammons}, S. Mark and {Bailey}, Vanessa P. and {Barman}, Travis S. and {Bulger}, Joanna and {Bruzzone}, Sebastian and {Chilcote}, Jeffrey K. and {Cotten}, Tara and {Dawson}, Rebekah I. and {De Rosa}, Robert J. and {Doyon}, Ren{\'e} and {Esposito}, Thomas M. and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Goodsell}, Stephen and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Kalas}, Paul and {Lafreni{\`e}re}, David and {Larkin}, James E. and {Macintosh}, Bruce A. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marley}, Mark S. and {Matthews}, Brenda C. and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Oppenheimer}, Rebecca and {Palmer}, David W. and {Patience}, Jenny and {Perrin}, Marshall D. and {Poyneer}, Lisa A. and {Rajan}, Abhijith and {Rantakyr{\"o}}, Fredrik T. and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane J. and {Wolff}, Schuyler G.},
        title = "{Discovery of a Substellar Companion to the Nearby Debris Disk Host HR 2562}",
      journal = {\apjl},
     keywords = {brown dwarfs, instrumentation: adaptive optics, planet{\textendash}disk interactions, stars: individual: HR 2562, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = sep,
       volume = {829},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.3847/2041-8205/829/1/L4},
archivePrefix = {arXiv},
       eprint = {1608.06660},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...829L...4K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chen+2014,
       author = {{Chen}, Christine H. and {Mittal}, Tushar and {Kuchner}, Marc and {Forrest}, William J. and {Lisse}, Carey M. and {Manoj}, P. and {Sargent}, Benjamin A. and {Watson}, Dan M.},
        title = "{The Spitzer Infrared Spectrograph Debris Disk Catalog. I. Continuum Analysis of Unresolved Targets}",
      journal = {\apjs},
     keywords = {catalogs, circumstellar matter, infrared: stars, zodiacal dust},
         year = 2014,
        month = apr,
       volume = {211},
       number = {2},
          eid = {25},
        pages = {25},
          doi = {10.1088/0067-0049/211/2/25},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..211...25C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gray+2006,
       author = {{Gray}, R.~O. and {Corbally}, C.~J. and {Garrison}, R.~F. and {McFadden}, M.~T. and {Bubar}, E.~J. and {McGahee}, C.~E. and {O'Donoghue}, A.~A. and {Knox}, E.~R.},
        title = "{Contributions to the Nearby Stars (NStars) Project: Spectroscopy of Stars Earlier than M0 within 40 pc-The Southern Sample}",
      journal = {\aj},
     keywords = {Galaxy: Solar Neighborhood, Stars: Abundances, Stars: Activity, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Statistics, Astrophysics},
         year = 2006,
        month = jul,
       volume = {132},
       number = {1},
        pages = {161-170},
          doi = {10.1086/504637},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603770},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....132..161G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia-EDR3,
       author = {{Gaia Collaboration}},
        title = "{VizieR Online Data Catalog: Gaia EDR3 (Gaia Collaboration, 2020)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Gaia},
         year = 2020,
        month = nov,
          eid = {I/350},
        pages = {I/350},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020yCat.1350....0G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia+2016,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland}, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A\&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maire+2018,
       author = {{Maire}, A. -L. and {Rodet}, L. and {Lazzoni}, C. and {Boccaletti}, A. and {Brandner}, W. and {Galicher}, R. and {Cantalloube}, F. and {Mesa}, D. and {Klahr}, H. and {Beust}, H. and {Chauvin}, G. and {Desidera}, S. and {Janson}, M. and {Keppler}, M. and {Olofsson}, J. and {Augereau}, J. -C. and {Daemgen}, S. and {Henning}, T. and {Th{\'e}bault}, P. and {Bonnefoy}, M. and {Feldt}, M. and {Gratton}, R. and {Lagrange}, A. -M. and {Langlois}, M. and {Meyer}, M.~R. and {Vigan}, A. and {D'Orazi}, V. and {Hagelberg}, J. and {Le Coroller}, H. and {Ligi}, R. and {Rouan}, D. and {Samland}, M. and {Schmidt}, T. and {Udry}, S. and {Zurlo}, A. and {Abe}, L. and {Carle}, M. and {Delboulb{\'e}}, A. and {Feautrier}, P. and {Magnard}, Y. and {Maurel}, D. and {Moulin}, T. and {Pavlov}, A. and {Perret}, D. and {Petit}, C. and {Ramos}, J.~R. and {Rigal}, F. and {Roux}, A. and {Weber}, L.},
        title = "{VLT/SPHERE astrometric confirmation and orbital analysis of the brown dwarf companion HR 2562 B}",
      journal = {\aap},
     keywords = {brown dwarfs, methods: data analysis, stars: individual: HR 2562, planets and satellites: dynamical evolution and stability, techniques: high angular resolution, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jul,
       volume = {615},
          eid = {A177},
        pages = {A177},
          doi = {10.1051/0004-6361/201732476},
archivePrefix = {arXiv},
       eprint = {1804.04584},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A\&A...615A.177M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kervella+2022,
       author = {{Kervella}, Pierre and {Arenou}, Fr{\'e}d{\'e}ric and {Th{\'e}venin}, Fr{\'e}d{\'e}ric},
        title = "{Stellar and substellar companions from Gaia EDR3. Proper-motion anomaly and resolved common proper-motion pairs}",
      journal = {\aap},
     keywords = {astrometry, planets and satellites: detection, proper motions, binaries: visual, solar neighborhood, catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jan,
       volume = {657},
          eid = {A7},
        pages = {A7},
          doi = {10.1051/0004-6361/202142146},
archivePrefix = {arXiv},
       eprint = {2109.10912},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A\&A...657A...7K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Casagrande+2011,
       author = {{Casagrande}, L. and {Sch{\"o}nrich}, R. and {Asplund}, M. and {Cassisi}, S. and {Ram{\'\i}rez}, I. and {Mel{\'e}ndez}, J. and {Bensby}, T. and {Feltzing}, S.},
        title = "{New constraints on the chemical evolution of the solar neighbourhood and Galactic disc(s). Improved astrophysical parameters for the Geneva-Copenhagen Survey}",
      journal = {\aap},
     keywords = {stars: abundances, stars: fundamental parameters, Hertzsprung-Russell and C-M diagrams, stars: kinematics and dynamics, Galaxy: disk, solar neighborhood, Astrophysics - Galaxy Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A138},
        pages = {A138},
          doi = {10.1051/0004-6361/201016276},
archivePrefix = {arXiv},
       eprint = {1103.4651},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A\&A...530A.138C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sutlieff+2021,
       author = {{Sutlieff}, Ben J. and {Bohn}, Alexander J. and {Birkby}, Jayne L. and {Kenworthy}, Matthew A. and {Morzinski}, Katie M. and {Doelman}, David S. and {Males}, Jared R. and {Snik}, Frans and {Close}, Laird M. and {Hinz}, Philip M. and {Charbonneau}, David},
        title = "{High-contrast observations of brown dwarf companion HR 2562 B with the vector Apodizing Phase Plate coronagraph}",
      journal = {\mnras},
     keywords = {instrumentation: high angular resolution, planets and satellites: atmospheres, planets and satellites: detection, brown dwarfs, stars: individual: HR 2562, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = sep,
       volume = {506},
       number = {3},
        pages = {3224-3238},
          doi = {10.1093/mnras/stab1893},
archivePrefix = {arXiv},
       eprint = {2106.14890},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.506.3224S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{Morales+2006,
       author = {{Morales Dur{\'a}n}, C. and {Alfonso Garz{\'o}n}, J. and {Freire Ferrero}, R.},
        title = "{The Rv extinction factor}",
     keywords = {interstellar extinction, extinction law, Rv extinction factor},
    booktitle = {Lecture Notes and Essays in Astrophysics},
         year = 2006,
       editor = {{Ulla}, Ana and {Manteiga}, Minia},
       volume = {2},
        pages = {189-198},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006LNEA....2..189M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boccaletti+2022,
       author = {{Boccaletti}, A. and {Cossou}, C. and {Baudoz}, P. and {Lagage}, P.~O. and {Dicken}, D. and {Glasse}, A. and {Hines}, D.~C. and {Aguilar}, J. and {Detre}, O. and {Nickson}, B. and {Noriega-Crespo}, A. and {G{\'a}sp{\'a}r}, A. and {Labiano}, A. and {Stark}, C. and {Rouan}, D. and {Reess}, J.~M. and {Wright}, G.~S. and {Rieke}, G. and {Garcia Marin}, M. and {Lajoie}, C. and {Girard}, J. and {Perrin}, M. and {Soummer}, R. and {Pueyo}, L.},
        title = "{JWST/MIRI coronagraphic performances as measured on-sky}",
      journal = {\aap},
     keywords = {instrumentation: high angular resolution, techniques: high angular resolution, techniques: image processing, planetary systems, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = nov,
       volume = {667},
          eid = {A165},
        pages = {A165},
          doi = {10.1051/0004-6361/202244578},
archivePrefix = {arXiv},
       eprint = {2207.11080},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A\&A...667A.165B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rieke+2015,
       author = {{Rieke}, G.~H. and {Ressler}, M.~E. and {Morrison}, Jane E. and {Bergeron}, L. and {Bouchet}, Patrice and {Garc{\'\i}a-Mar{\'\i}n}, Macarena and {Greene}, T.~P. and {Regan}, M.~W. and {Sukhatme}, K.~G. and {Walker}, Helen},
        title = "{The Mid-Infrared Instrument for the James Webb Space Telescope, VII: The MIRI Detectors}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = jul,
       volume = {127},
       number = {953},
        pages = {665},
          doi = {10.1086/682257},
archivePrefix = {arXiv},
       eprint = {1508.02362},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PASP..127..665R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wright+2015,
       author = {{Wright}, G.~S. and {Wright}, David and {Goodson}, G.~B. and {Rieke}, G.~H. and {Aitink-Kroes}, Gabby and {Amiaux}, J. and {Aricha-Yanguas}, Ana and {Azzollini}, Ruym{\'a}n and {Banks}, Kimberly and {Barrado-Navascues}, D. and {Belenguer-Davila}, T. and {Blommaert}, J.~A.~D.~L. and {Bouchet}, Patrice and {Brandl}, B.~R. and {Colina}, L. and {Detre}, {\"O}rs and {Diaz-Catala}, Eva and {Eccleston}, Paul and {Friedman}, Scott D. and {Garc{\'\i}a-Mar{\'\i}n}, Macarena and {G{\"u}del}, Manuel and {Glasse}, Alistair and {Glauser}, Adrian M. and {Greene}, T.~P. and {Groezinger}, Uli and {Grundy}, Tim and {Hastings}, Peter and {Henning}, Th. and {Hofferbert}, Ralph and {Hunter}, Faye and {Jessen}, N.~C. and {Justtanont}, K. and {Karnik}, Avinash R. and {Khorrami}, Mori A. and {Krause}, Oliver and {Labiano}, Alvaro and {Lagage}, P. -O. and {Langer}, Ulrich and {Lemke}, Dietrich and {Lim}, Tanya and {Lorenzo-Alvarez}, Jose and {Mazy}, Emmanuel and {McGowan}, Norman and {Meixner}, M.~E. and {Morris}, Nigel and {Morrison}, Jane E. and {M{\"u}ller}, Friedrich and {rgaard-Nielson}, H. -U. N{\o} and {Olofsson}, G{\"o}ran and {O'Sullivan}, Brian and {Pel}, J. -W. and {Penanen}, Konstantin and {Petach}, M.~B. and {Pye}, J.~P. and {Ray}, T.~P. and {Renotte}, Etienne and {Renouf}, Ian and {Ressler}, M.~E. and {Samara-Ratna}, Piyal and {Scheithauer}, Silvia and {Schneider}, Analyn and {Shaughnessy}, Bryan and {Stevenson}, Tim and {Sukhatme}, Kalyani and {Swinyard}, Bruce and {Sykes}, Jon and {Thatcher}, John and {Tikkanen}, Tuomo and {van Dishoeck}, E.~F. and {Waelkens}, C. and {Walker}, Helen and {Wells}, Martyn and {Zhender}, Alex},
        title = "{The Mid-Infrared Instrument for the James Webb Space Telescope, II: Design and Build}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = jul,
       volume = {127},
       number = {953},
        pages = {595},
          doi = {10.1086/682253},
archivePrefix = {arXiv},
       eprint = {1508.02333},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PASP..127..595W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rouan+2000,
       author = {{Rouan}, D. and {Riaud}, P. and {Boccaletti}, A. and {Cl{\'e}net}, Y. and {Labeyrie}, A.},
        title = "{The Four-Quadrant Phase-Mask Coronagraph. I. Principle}",
      journal = {\pasp},
     keywords = {Instrumentation: Adaptive Optics, Methods: Numerical, Stars: Planetary Systems, Stars: Low-Mass, Brown Dwarfs},
         year = 2000,
        month = nov,
       volume = {112},
       number = {777},
        pages = {1479-1486},
          doi = {10.1086/317707},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000PASP..112.1479R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Smith+Terrile-1984,
       author = {{Smith}, B.~A. and {Terrile}, R.~J.},
        title = "{A Circumstellar Disk around {\ensuremath{\beta}} Pictoris}",
      journal = {Science},
     keywords = {Dwarf Stars, Main Sequence Stars, Planetary Evolution, Stellar Envelopes, Brightness, Disks, Infrared Astronomy Satellite, Scattering Cross Sections, Visible Spectrum, Astrophysics},
         year = 1984,
        month = dec,
       volume = {226},
       number = {4681},
        pages = {1421-1424},
          doi = {10.1126/science.226.4681.1421},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984Sci...226.1421S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Houk+1975,
       author = {{Houk}, N. and {Cowley}, A.~P.},
        title = "{University of Michigan Catalogue of two-dimensional spectral types for the HD stars. Volume I. Declinations -90\_ to -53\_{\textflorin}0.}",
         year = 1975,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975mcts.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cutri+2003,
       author = {{Cutri}, R.~M. and {Skrutskie}, M.~F. and {van Dyk}, S. and {Beichman}, C.~A. and {Carpenter}, J.~M. and {Chester}, T. and {Cambresy}, L. and {Evans}, T. and {Fowler}, J. and {Gizis}, J. and {Howard}, E. and {Huchra}, J. and {Jarrett}, T. and {Kopan}, E.~L. and {Kirkpatrick}, J.~D. and {Light}, R.~M. and {Marsh}, K.~A. and {McCallon}, H. and {Schneider}, S. and {Stiening}, R. and {Sykes}, M. and {Weinberg}, M. and {Wheaton}, W.~A. and {Wheelock}, S. and {Zacarias}, N.},
        title = "{VizieR Online Data Catalog: 2MASS All-Sky Catalog of Point Sources (Cutri+ 2003)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Infrared sources, Photometry: infrared, Surveys},
         year = 2003,
        month = jun,
          eid = {II/246},
        pages = {II/246},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003yCat.2246....0C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Rodrigo+2012,
       author = {{Rodrigo}, Carlos and {Solano}, Enrique and {Bayo}, Amelia},
        title = "{SVO Filter Profile Service Version 1.0}",
 howpublished = {IVOA Working Draft 15 October 2012},
         year = 2012,
        month = oct,
        pages = {1015},
          doi = {10.5479/ADS/bib/2012ivoa.rept.1015R},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ivoa.rept.1015R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Rodrigo+2020,
       author = {{Rodrigo}, C. and {Solano}, E.},
        title = "{The SVO Filter Profile Service}",
    booktitle = {XIV.0 Scientific Meeting (virtual) of the Spanish Astronomical Society},
         year = 2020,
        month = jul,
          eid = {182},
        pages = {182},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020sea..confE.182R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sutlieff+2023,
       author = {{Sutlieff}, Ben J. and {Birkby}, Jayne L. and {Stone}, Jordan M. and {Doelman}, David S. and {Kenworthy}, Matthew A. and {Panwar}, Vatsal and {Bohn}, Alexander J. and {Ertel}, Steve and {Snik}, Frans and {Woodward}, Charles E. and {Skemer}, Andrew J. and {Leisenring}, Jarron M. and {Strassmeier}, Klaus G. and {Charbonneau}, David},
        title = "{Measuring the variability of directly imaged exoplanets using vector Apodizing Phase Plates combined with ground-based differential spectrophotometry}",
      journal = {\mnras},
     keywords = {instrumentation: high angular resolution, techniques: imaging spectroscopy, planets and satellites: atmospheres, planets and satellites: detection, brown dwarfs, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = apr,
       volume = {520},
       number = {3},
        pages = {4235-4257},
          doi = {10.1093/mnras/stad249},
archivePrefix = {arXiv},
       eprint = {2301.08689},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.520.4235S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GRAVIY+2020,
       author = {{GRAVITY Collaboration} and {Nowak}, M. and {Lacour}, S. and {Molli{\`e}re}, P. and {Wang}, J. and {Charnay}, B. and {van Dishoeck}, E.~F. and {Abuter}, R. and {Amorim}, A. and {Berger}, J.~P. and {Beust}, H. and {Bonnefoy}, M. and {Bonnet}, H. and {Brandner}, W. and {Buron}, A. and {Cantalloube}, F. and {Collin}, C. and {Chapron}, F. and {Cl{\'e}net}, Y. and {Coud{\'e} Du Foresto}, V. and {de Zeeuw}, P.~T. and {Dembet}, R. and {Dexter}, J. and {Duvert}, G. and {Eckart}, A. and {Eisenhauer}, F. and {F{\"o}rster Schreiber}, N.~M. and {F{\'e}dou}, P. and {Garcia Lopez}, R. and {Gao}, F. and {Gendron}, E. and {Genzel}, R. and {Gillessen}, S. and {Hau{\ss}mann}, F. and {Henning}, T. and {Hippler}, S. and {Hubert}, Z. and {Jocou}, L. and {Kervella}, P. and {Lagrange}, A. -M. and {Lapeyr{\`e}re}, V. and {Le Bouquin}, J. -B. and {L{\'e}na}, P. and {Maire}, A. -L. and {Ott}, T. and {Paumard}, T. and {Paladini}, C. and {Perraut}, K. and {Perrin}, G. and {Pueyo}, L. and {Pfuhl}, O. and {Rabien}, S. and {Rau}, C. and {Rodr{\'\i}guez-Coira}, G. and {Rousset}, G. and {Scheithauer}, S. and {Shangguan}, J. and {Straub}, O. and {Straubmeier}, C. and {Sturm}, E. and {Tacconi}, L.~J. and {Vincent}, F. and {Widmann}, F. and {Wieprecht}, E. and {Wiezorrek}, E. and {Woillez}, J. and {Yazici}, S. and {Ziegler}, D.},
        title = "{Peering into the formation history of {\ensuremath{\beta}} Pictoris b with VLTI/GRAVITY long-baseline interferometry}",
      journal = {\aap},
     keywords = {planets and satellites: formation, planets and satellites: atmospheres, techniques: interferometric, stars: individual: {\ensuremath{\beta}} Pictoris, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jan,
       volume = {633},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201936898},
archivePrefix = {arXiv},
       eprint = {1912.04651},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A\&A...633A.110G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Phillips+2020,
       author = {{Phillips}, M.~W. and {Tremblin}, P. and {Baraffe}, I. and {Chabrier}, G. and {Allard}, N.~F. and {Spiegelman}, F. and {Goyal}, J.~M. and {Drummond}, B. and {H{\'e}brard}, E.},
        title = "{A new set of atmosphere and evolution models for cool T-Y brown dwarfs and giant exoplanets}",
      journal = {\aap},
     keywords = {brown dwarfs, planets and satellites: atmospheres, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = may,
       volume = {637},
          eid = {A38},
        pages = {A38},
          doi = {10.1051/0004-6361/201937381},
archivePrefix = {arXiv},
       eprint = {2003.13717},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A\&A...637A..38P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Dohlen+2008,
       author = {{Dohlen}, Kjetil and {Langlois}, Maud and {Saisse}, Michel and {Hill}, Lucien and {Origne}, Alain and {Jacquet}, Marc and {Fabron}, Christophe and {Blanc}, Jean-Claude and {Llored}, Marc and {Carle}, Michael and {Moutou}, Claire and {Vigan}, Arthur and {Boccaletti}, Anthony and {Carbillet}, Marcel and {Mouillet}, David and {Beuzit}, Jean-Luc},
        title = "{The infra-red dual imaging and spectrograph for SPHERE: design and performance}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy II},
         year = 2008,
       editor = {{McLean}, Ian S. and {Casali}, Mark M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7014},
        month = jul,
          eid = {70143L},
        pages = {70143L},
          doi = {10.1117/12.789786},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7014E..3LD},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Claudi+2008,
       author = {{Claudi}, R.~U. and {Turatto}, M. and {Gratton}, R.~G. and {Antichi}, J. and {Bonavita}, M. and {Bruno}, P. and {Cascone}, E. and {De Caprio}, V. and {Desidera}, S. and {Giro}, E. and {Mesa}, D. and {Scuderi}, S. and {Dohlen}, K. and {Beuzit}, J.~L. and {Puget}, P.},
        title = "{SPHERE IFS: the spectro differential imager of the VLT for exoplanets search}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy II},
         year = 2008,
       editor = {{McLean}, Ian S. and {Casali}, Mark M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7014},
        month = jul,
          eid = {70143E},
        pages = {70143E},
          doi = {10.1117/12.788366},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7014E..3EC},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beuzit+2019,
       author = {{Beuzit}, J. -L. and {Vigan}, A. and {Mouillet}, D. and {Dohlen}, K. and
         {Gratton}, R. and {Boccaletti}, A. and {Sauvage}, J. -F. and
         {Schmid}, H.~M. and {Langlois}, M. and {Petit}, C. and {Baruffolo}, A. and
         {Feldt}, M. and {Milli}, J. and {Wahhaj}, Z. and {Abe}, L. and
         {Anselmi}, U. and {Antichi}, J. and {Barette}, R. and {Baudrand}, J. and
         {Baudoz}, P. and {Bazzon}, A. and {Bernardi}, P. and {Blanchard}, P. and
         {Brast}, R. and {Bruno}, P. and {Buey}, T. and {Carbillet}, M. and
         {Carle}, M. and {Cascone}, E. and {Chapron}, F. and {Charton}, J. and
         {Chauvin}, G. and {Claudi}, R. and {Costille}, A. and {De Caprio}, V. and
         {de Boer}, J. and {Delboulb{\'e}}, A. and {Desidera}, S. and
         {Dominik}, C. and {Downing}, M. and {Dupuis}, O. and {Fabron}, C. and
         {Fantinel}, D. and {Farisato}, G. and {Feautrier}, P. and
         {Fedrigo}, E. and {Fusco}, T. and {Gigan}, P. and {Ginski}, C. and
         {Girard}, J. and {Giro}, E. and {Gisler}, D. and {Gluck}, L. and
         {Gry}, C. and {Henning}, T. and {Hubin}, N. and {Hugot}, E. and
         {Incorvaia}, S. and {Jaquet}, M. and {Kasper}, M. and {Lagadec}, E. and
         {Lagrange}, A. -M. and {Le Coroller}, H. and {Le Mignant}, D. and
         {Le Ruyet}, B. and {Lessio}, G. and {Lizon}, J. -L. and {Llored}, M. and
         {Lundin}, L. and {Madec}, F. and {Magnard}, Y. and {Marteaud}, M. and
         {Martinez}, P. and {Maurel}, D. and {M{\'e}nard}, F. and {Mesa}, D. and
         {M{\"o}ller-Nilsson}, O. and {Moulin}, T. and {Moutou}, C. and
         {Orign{\'e}}, A. and {Parisot}, J. and {Pavlov}, A. and {Perret}, D. and
         {Pragt}, J. and {Puget}, P. and {Rabou}, P. and {Ramos}, J. and
         {Reess}, J. -M. and {Rigal}, F. and {Rochat}, S. and {Roelfsema}, R. and
         {Rousset}, G. and {Roux}, A. and {Saisse}, M. and {Salasnich}, B. and
         {Santambrogio}, E. and {Scuderi}, S. and {Segransan}, D. and
         {Sevin}, A. and {Siebenmorgen}, R. and {Soenke}, C. and {Stadler}, E. and
         {Suarez}, M. and {Tiph{\`e}ne}, D. and {Turatto}, M. and {Udry}, S. and
         {Vakili}, F. and {Waters}, L.~B.~F.~M. and {Weber}, L. and {Wildi}, F. and
         {Zins}, G. and {Zurlo}, A.},
        title = "{SPHERE: the exoplanet imager for the Very Large Telescope}",
      journal = {\aap},
     keywords = {instrumentation: high angular resolution, instrumentation: adaptive optics, instrumentation: polarimeters, instrumentation: spectrographs, planets and satellites: detection, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A155},
        pages = {A155},
          doi = {10.1051/0004-6361/201935251},
archivePrefix = {arXiv},
       eprint = {1902.04080},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A\&A...631A.155B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Metchev+2015,
       author = {{Metchev}, Stanimir A. and {Heinze}, Aren and {Apai}, D{\'a}niel and {Flateau}, Davin and {Radigan}, Jacqueline and {Burgasser}, Adam and {Marley}, Mark S. and {Artigau}, {\'E}tienne and {Plavchan}, Peter and {Goldman}, Bertrand},
        title = "{Weather on Other Worlds. II. Survey Results: Spots are Ubiquitous on L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: low-mass, stars: rotation, starspots, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {154},
        pages = {154},
          doi = {10.1088/0004-637X/799/2/154},
archivePrefix = {arXiv},
       eprint = {1411.3051},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..154M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gomez-Gonzalez+2017,
       author = {{Gomez Gonzalez}, Carlos Alberto and {Wertz}, Olivier and {Absil}, Olivier and {Christiaens}, Valentin and {Defr{\`e}re}, Denis and {Mawet}, Dimitri and {Milli}, Julien and {Absil}, Pierre-Antoine and {Van Droogenbroeck}, Marc and {Cantalloube}, Faustine and {Hinz}, Philip M. and {Skemer}, Andrew J. and {Karlsson}, Mikael and {Surdej}, Jean},
        title = "{VIP: Vortex Image Processing Package for High-contrast Direct Imaging}",
      journal = {\aj},
     keywords = {methods: data analysis, planetary systems, planets and satellites: detection, techniques: high angular resolution, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = jul,
       volume = {154},
       number = {1},
          eid = {7},
        pages = {7},
          doi = {10.3847/1538-3881/aa73d7},
archivePrefix = {arXiv},
       eprint = {1705.06184},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154....7G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Christiaens+2023,
       author = {{Christiaens}, Valentin and {Gonzalez}, Carlos and {Farkas}, Ralf and {Dahlqvist}, Carl-Henrik and {Nasedkin}, Evert and {Milli}, Julien and {Absil}, Olivier and {Ngo}, Henry and {Cantero}, Carles and {Rainot}, Alan and {Hammond}, Iain and {Bonse}, Markus and {Cantalloube}, Faustine and {Vigan}, Arthur and {Kompella}, Vijay and {Hancock}, Paul},
        title = "{VIP: A Python package for high-contrast imaging}",
      journal = {The Journal of Open Source Software},
     keywords = {Python, high-contrast, astronomy, exoplanets, direct imaging},
         year = 2023,
        month = jan,
       volume = {8},
       number = {81},
          eid = {4774},
        pages = {4774},
          doi = {10.21105/joss.04774},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023JOSS....8.4774C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bayo+2008,
       author = {{Bayo}, A. and {Rodrigo}, C. and {Barrado Y Navascu{\'e}s}, D. and {Solano}, E. and {Guti{\'e}rrez}, R. and {Morales-Calder{\'o}n}, M. and {Allard}, F.},
        title = "{VOSA: virtual observatory SED analyzer. An application to the Collinder 69 open cluster}",
      journal = {\aap},
     keywords = {astronomical data bases: miscellaneous, stars: formation, stars: circumstellar matter, stars: low-mass, brown dwarfs, stars: Hertzsprung-Russell (HR) and C-M diagrams, Galaxy: open clusters and associations: individual: Collinder 69, Astrophysics},
         year = 2008,
        month = dec,
       volume = {492},
       number = {1},
        pages = {277-287},
          doi = {10.1051/0004-6361:200810395},
archivePrefix = {arXiv},
       eprint = {0808.0270},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A\&A...492..277B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{HIPPARCOS,
        title = "{The HIPPARCOS and TYCHO catalogues. Astrometric and photometric star catalogues derived from the ESA HIPPARCOS Space Astrometry Mission}",
     keywords = {SPACE ASTROMETRY, STAR CATALOGS, POSITIONS, ARTIFICIAL SATELLITES},
    booktitle = {ESA Special Publication},
         year = 1997,
       series = {ESA Special Publication},
       volume = {1200},
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ESASP1200.....E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2MASS,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% galaxy spectra
@ARTICLE{Bruzual+Charlot-2003,
       author = {{Bruzual}, G. and {Charlot}, S.},
        title = "{Stellar population synthesis at the resolution of 2003}",
      journal = {\mnras},
     keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = oct,
       volume = {344},
       number = {4},
        pages = {1000-1028},
          doi = {10.1046/j.1365-8711.2003.06897.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309134},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marois+2008,
       author = {{Marois}, Christian and {Macintosh}, Bruce and {Barman}, Travis and {Zuckerman}, B. and {Song}, Inseok and {Patience}, Jennifer and {Lafreni{\`e}re}, David and {Doyon}, Ren{\'e}},
        title = "{Direct Imaging of Multiple Planets Orbiting the Star HR 8799}",
      journal = {Science},
     keywords = {Astrophysics},
         year = 2008,
        month = nov,
       volume = {322},
       number = {5906},
        pages = {1348},
          doi = {10.1126/science.1166585},
archivePrefix = {arXiv},
       eprint = {0811.2606},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008Sci...322.1348M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chauvin+2004,
       author = {{Chauvin}, G. and {Lagrange}, A. -M. and {Dumas}, C. and {Zuckerman}, B. and {Mouillet}, D. and {Song}, I. and {Beuzit}, J. -L. and {Lowrance}, P.},
        title = "{A giant planet candidate near a young brown dwarf. Direct VLT/NACO observations using IR wavefront sensing}",
      journal = {\aap},
     keywords = {2MASSWJ 1207334-393254, brown dwarf, giant planet, adaptive optics imaging and spectroscopy, Astrophysics},
         year = 2004,
        month = oct,
       volume = {425},
        pages = {L29-L32},
          doi = {10.1051/0004-6361:200400056},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409323},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A\&A...425L..29C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macintosh+2015,
       author = {{Macintosh}, B. and {Graham}, J.~R. and {Barman}, T. and {De Rosa}, R.~J. and {Konopacky}, Q. and {Marley}, M.~S. and {Marois}, C. and {Nielsen}, E.~L. and {Pueyo}, L. and {Rajan}, A. and {Rameau}, J. and {Saumon}, D. and {Wang}, J.~J. and {Patience}, J. and {Ammons}, M. and {Arriaga}, P. and {Artigau}, E. and {Beckwith}, S. and {Brewster}, J. and {Bruzzone}, S. and {Bulger}, J. and {Burningham}, B. and {Burrows}, A.~S. and {Chen}, C. and {Chiang}, E. and {Chilcote}, J.~K. and {Dawson}, R.~I. and {Dong}, R. and {Doyon}, R. and {Draper}, Z.~H. and {Duch{\^e}ne}, G. and {Esposito}, T.~M. and {Fabrycky}, D. and {Fitzgerald}, M.~P. and {Follette}, K.~B. and {Fortney}, J.~J. and {Gerard}, B. and {Goodsell}, S. and {Greenbaum}, A.~Z. and {Hibon}, P. and {Hinkley}, S. and {Cotten}, T.~H. and {Hung}, L. -W. and {Ingraham}, P. and {Johnson-Groh}, M. and {Kalas}, P. and {Lafreniere}, D. and {Larkin}, J.~E. and {Lee}, J. and {Line}, M. and {Long}, D. and {Maire}, J. and {Marchis}, F. and {Matthews}, B.~C. and {Max}, C.~E. and {Metchev}, S. and {Millar-Blanchaer}, M.~A. and {Mittal}, T. and {Morley}, C.~V. and {Morzinski}, K.~M. and {Murray-Clay}, R. and {Oppenheimer}, R. and {Palmer}, D.~W. and {Patel}, R. and {Perrin}, M.~D. and {Poyneer}, L.~A. and {Rafikov}, R.~R. and {Rantakyr{\"o}}, F.~T. and {Rice}, E.~L. and {Rojo}, P. and {Rudy}, A.~R. and {Ruffio}, J. -B. and {Ruiz}, M.~T. and {Sadakuni}, N. and {Saddlemyer}, L. and {Salama}, M. and {Savransky}, D. and {Schneider}, A.~C. and {Sivaramakrishnan}, A. and {Song}, I. and {Soummer}, R. and {Thomas}, S. and {Vasisht}, G. and {Wallace}, J.~K. and {Ward-Duong}, K. and {Wiktorowicz}, S.~J. and {Wolff}, S.~G. and {Zuckerman}, B.},
        title = "{Discovery and spectroscopy of the young jovian planet 51 Eri b with the Gemini Planet Imager}",
      journal = {Science},
     keywords = {ASTRONOMY, PLANET SCI, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {350},
       number = {6256},
        pages = {64-67},
          doi = {10.1126/science.aac5891},
archivePrefix = {arXiv},
       eprint = {1508.03084},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015Sci...350...64M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lagrange+2010,
       author = {{Lagrange}, A. -M. and {Bonnefoy}, M. and {Chauvin}, G. and {Apai}, D. and {Ehrenreich}, D. and {Boccaletti}, A. and {Gratadour}, D. and {Rouan}, D. and {Mouillet}, D. and {Lacour}, S. and {Kasper}, M.},
        title = "{A Giant Planet Imaged in the Disk of the Young Star {\ensuremath{\beta}} Pictoris}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jul,
       volume = {329},
       number = {5987},
        pages = {57},
          doi = {10.1126/science.1187187},
archivePrefix = {arXiv},
       eprint = {1006.3314},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Sci...329...57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Janson+2019,
       author = {{Janson}, Markus and {Asensio-Torres}, Ruben and {Andr{\'e}}, Damien and {Bonnefoy}, Micka{\"e}l and {Delorme}, Philippe and {Reffert}, Sabine and {Desidera}, Silvano and {Langlois}, Maud and {Chauvin}, Ga{\"e}l and {Gratton}, Raffaele and {Bohn}, Alexander J. and {Eriksson}, Simon C. and {Marleau}, Gabriel-Dominique and {Mamajek}, Eric E. and {Vigan}, Arthur and {Carson}, Joseph C.},
        title = "{The B-Star Exoplanet Abundance Study: a co-moving 16-25 M$_{Jup}$ companion to the young binary system HIP 79098}",
      journal = {\aap},
     keywords = {brown dwarfs, stars: early-type, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {626},
          eid = {A99},
        pages = {A99},
          doi = {10.1051/0004-6361/201935687},
archivePrefix = {arXiv},
       eprint = {1906.02787},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A\&A...626A..99J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miles+2023,
       author = {{Miles}, Brittany E. and {Biller}, Beth A. and {Patapis}, Polychronis and {Worthen}, Kadin and {Rickman}, Emily and {Hoch}, Kielan K.~W. and {Skemer}, Andrew and {Perrin}, Marshall D. and {Whiteford}, Niall and {Chen}, Christine H. and {Sargent}, B. and {Mukherjee}, Sagnick and {Morley}, Caroline V. and {Moran}, Sarah E. and {Bonnefoy}, Mickael and {Petrus}, Simon and {Carter}, Aarynn L. and {Choquet}, Elodie and {Hinkley}, Sasha and {Ward-Duong}, Kimberly and {Leisenring}, Jarron M. and {Millar-Blanchaer}, Maxwell A. and {Pueyo}, Laurent and {Ray}, Shrishmoy and {Sallum}, Steph and {Stapelfeldt}, Karl R. and {Stone}, Jordan M. and {Wang}, Jason J. and {Absil}, Olivier and {Balmer}, William O. and {Boccaletti}, Anthony and {Bonavita}, Mariangela and {Booth}, Mark and {Bowler}, Brendan P. and {Chauvin}, Gael and {Christiaens}, Valentin and {Currie}, Thayne and {Danielski}, Camilla and {Fortney}, Jonathan J. and {Girard}, Julien H. and {Grady}, Carol A. and {Greenbaum}, Alexandra Z. and {Henning}, Thomas and {Hines}, Dean C. and {Janson}, Markus and {Kalas}, Paul and {Kammerer}, Jens and {Kennedy}, Grant M. and {Kenworthy}, Matthew A. and {Kervella}, Pierre and {Lagage}, Pierre-Olivier and {Lew}, Ben W.~P. and {Liu}, Michael C. and {Macintosh}, Bruce and {Marino}, Sebastian and {Marley}, Mark S. and {Marois}, Christian and {Matthews}, Elisabeth C. and {Matthews}, Brenda C. and {Mawet}, Dimitri and {McElwain}, Michael W. and {Metchev}, Stanimir and {Meyer}, Michael R. and {Molliere}, Paul and {Pantin}, Eric and {Quirrenbach}, Andreas and {Rebollido}, Isabel and {Ren}, Bin B. and {Schneider}, Glenn and {Vasist}, Malavika and {Wyatt}, Mark C. and {Zhou}, Yifan and {Briesemeister}, Zackery W. and {Bryan}, Marta L. and {Calissendorff}, Per and {Cantalloube}, Faustine and {Cugno}, Gabriele and {De Furio}, Matthew and {Dupuy}, Trent J. and {Factor}, Samuel M. and {Faherty}, Jacqueline K. and {Fitzgerald}, Michael P. and {Franson}, Kyle and {Gonzales}, Eileen C. and {Hood}, Callie E. and {Howe}, Alex R. and {Kraus}, Adam L. and {Kuzuhara}, Masayuki and {Lagrange}, Anne-Marie and {Lawson}, Kellen and {Lazzoni}, Cecilia and {Liu}, Pengyu and {Llop-Sayson}, Jorge and {Lloyd}, James P. and {Martinez}, Raquel A. and {Mazoyer}, Johan and {Quanz}, Sascha P. and {Redai}, Jea Adams and {Samland}, Matthias and {Schlieder}, Joshua E. and {Tamura}, Motohide and {Tan}, Xianyu and {Uyama}, Taichi and {Vigan}, Arthur and {Vos}, Johanna M. and {Wagner}, Kevin and {Wolff}, Schuyler G. and {Ygouf}, Marie and {Zhang}, Xi and {Zhang}, Keming and {Zhang}, Zhoujian},
        title = "{The JWST Early-release Science Program for Direct Observations of Exoplanetary Systems II: A 1 to 20 {\ensuremath{\mu}}m Spectrum of the Planetary-mass Companion VHS 1256-1257 b}",
      journal = {\apjl},
     keywords = {Brown dwarfs, Exoplanet atmospheres, Extrasolar gaseous giant planets, 185, 487, 509, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = mar,
       volume = {946},
       number = {1},
          eid = {L6},
        pages = {L6},
          doi = {10.3847/2041-8213/acb04a},
archivePrefix = {arXiv},
       eprint = {2209.00620},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...946L...6M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Suarez+Metchev-2022,
       author = {{Su{\'a}rez}, Genaro and {Metchev}, Stanimir},
        title = "{Ultracool dwarfs observed with the Spitzer infrared spectrograph - II. Emergence and sedimentation of silicate clouds in L dwarfs, and analysis of the full M5-T9 field dwarf spectroscopic sample}",
      journal = {\mnras},
     keywords = {stars: atmospheres, brown dwarfs, infrared: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = jul,
       volume = {513},
       number = {4},
        pages = {5701-5726},
          doi = {10.1093/mnras/stac1205},
archivePrefix = {arXiv},
       eprint = {2205.00168},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513.5701S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{Marley+2013,
       author = {{Marley}, M.~S. and {Ackerman}, A.~S. and {Cuzzi}, J.~N. and {Kitzmann}, D.},
        title = "{Clouds and Hazes in Exoplanet Atmospheres}",
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Comparative Climatology of Terrestrial Planets},
         year = 2013,
       editor = {{Mackwell}, Stephen J. and {Simon-Miller}, Amy A. and {Harder}, Jerald W. and {Bullock}, Mark A.},
        pages = {367-392},
          doi = {10.2458/azu\_uapress\_9780816530595-ch015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013cctp.book..367M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nielsen+2019,
       author = {{Nielsen}, Eric L. and {De Rosa}, Robert J. and {Macintosh}, Bruce and {Wang}, Jason J. and {Ruffio}, Jean-Baptiste and {Chiang}, Eugene and {Marley}, Mark S. and {Saumon}, Didier and {Savransky}, Dmitry and {Ammons}, S. Mark and {Bailey}, Vanessa P. and {Barman}, Travis and {Blain}, C{\'e}lia and {Bulger}, Joanna and {Burrows}, Adam and {Chilcote}, Jeffrey and {Cotten}, Tara and {Czekala}, Ian and {Doyon}, Rene and {Duch{\^e}ne}, Gaspard and {Esposito}, Thomas M. and {Fabrycky}, Daniel and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Fortney}, Jonathan J. and {Gerard}, Benjamin L. and {Goodsell}, Stephen J. and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hinkley}, Sasha and {Hirsch}, Lea A. and {Hom}, Justin and {Hung}, Li-Wei and {Dawson}, Rebekah Ilene and {Ingraham}, Patrick and {Kalas}, Paul and {Konopacky}, Quinn and {Larkin}, James E. and {Lee}, Eve J. and {Lin}, Jonathan W. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marois}, Christian and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Morzinski}, Katie M. and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Pueyo}, Laurent and {Rafikov}, Roman R. and {Rajan}, Abhijith and {Rameau}, Julien and {Rantakyr{\"o}}, Fredrik T. and {Ren}, Bin and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Tallis}, Melisa and {Thomas}, Sandrine and {Ward-Duong}, Kimberly and {Wolff}, Schuyler},
        title = "{The Gemini Planet Imager Exoplanet Survey: Giant Planet and Brown Dwarf Demographics from 10 to 100 au}",
      journal = {\aj},
     keywords = {instrumentation: adaptive optics, planetary systems, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {158},
       number = {1},
          eid = {13},
        pages = {13},
          doi = {10.3847/1538-3881/ab16e9},
archivePrefix = {arXiv},
       eprint = {1904.05358},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....158...13N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vigan+2021,
       author = {{Vigan}, A. and {Fontanive}, C. and {Meyer}, M. and {Biller}, B. and {Bonavita}, M. and {Feldt}, M. and {Desidera}, S. and {Marleau}, G. -D. and {Emsenhuber}, A. and {Galicher}, R. and {Rice}, K. and {Forgan}, D. and {Mordasini}, C. and {Gratton}, R. and {Le Coroller}, H. and {Maire}, A. -L. and {Cantalloube}, F. and {Chauvin}, G. and {Cheetham}, A. and {Hagelberg}, J. and {Lagrange}, A. -M. and {Langlois}, M. and {Bonnefoy}, M. and {Beuzit}, J. -L. and {Boccaletti}, A. and {D'Orazi}, V. and {Delorme}, P. and {Dominik}, C. and {Henning}, Th. and {Janson}, M. and {Lagadec}, E. and {Lazzoni}, C. and {Ligi}, R. and {Menard}, F. and {Mesa}, D. and {Messina}, S. and {Moutou}, C. and {M{\"u}ller}, A. and {Perrot}, C. and {Samland}, M. and {Schmid}, H.~M. and {Schmidt}, T. and {Sissa}, E. and {Turatto}, M. and {Udry}, S. and {Zurlo}, A. and {Abe}, L. and {Antichi}, J. and {Asensio-Torres}, R. and {Baruffolo}, A. and {Baudoz}, P. and {Baudrand}, J. and {Bazzon}, A. and {Blanchard}, P. and {Bohn}, A.~J. and {Brown Sevilla}, S. and {Carbillet}, M. and {Carle}, M. and {Cascone}, E. and {Charton}, J. and {Claudi}, R. and {Costille}, A. and {De Caprio}, V. and {Delboulb{\'e}}, A. and {Dohlen}, K. and {Engler}, N. and {Fantinel}, D. and {Feautrier}, P. and {Fusco}, T. and {Gigan}, P. and {Girard}, J.~H. and {Giro}, E. and {Gisler}, D. and {Gluck}, L. and {Gry}, C. and {Hubin}, N. and {Hugot}, E. and {Jaquet}, M. and {Kasper}, M. and {Le Mignant}, D. and {Llored}, M. and {Madec}, F. and {Magnard}, Y. and {Martinez}, P. and {Maurel}, D. and {M{\"o}ller-Nilsson}, O. and {Mouillet}, D. and {Moulin}, T. and {Orign{\'e}}, A. and {Pavlov}, A. and {Perret}, D. and {Petit}, C. and {Pragt}, J. and {Puget}, P. and {Rabou}, P. and {Ramos}, J. and {Rickman}, E.~L. and {Rigal}, F. and {Rochat}, S. and {Roelfsema}, R. and {Rousset}, G. and {Roux}, A. and {Salasnich}, B. and {Sauvage}, J. -F. and {Sevin}, A. and {Soenke}, C. and {Stadler}, E. and {Suarez}, M. and {Wahhaj}, Z. and {Weber}, L. and {Wildi}, F.},
        title = "{The SPHERE infrared survey for exoplanets (SHINE). III. The demographics of young giant exoplanets below 300 au with SPHERE}",
      journal = {\aap},
     keywords = {techniques: high angular resolution, methods: statistical, infrared: planetary systems, planetary systems, planets and satellites: formation, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jul,
       volume = {651},
          eid = {A72},
        pages = {A72},
          doi = {10.1051/0004-6361/202038107},
archivePrefix = {arXiv},
       eprint = {2007.06573},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A\&A...651A..72V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Konopacky+2013,
       author = {{Konopacky}, Quinn M. and {Barman}, Travis S. and {Macintosh}, Bruce A. and {Marois}, Christian},
        title = "{Detection of Carbon Monoxide and Water Absorption Lines in an Exoplanet Atmosphere}",
      journal = {Science},
     keywords = {ASTRONOMY Astronomy, Ecology, Chemistry, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = mar,
       volume = {339},
       number = {6126},
        pages = {1398-1401},
          doi = {10.1126/science.1232003},
archivePrefix = {arXiv},
       eprint = {1303.3280},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Sci...339.1398K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brandt+2021,
       author = {{Brandt}, G. Mirek and {Brandt}, Timothy D. and {Dupuy}, Trent J. and {Li}, Yiting and {Michalik}, Daniel},
        title = "{Precise Dynamical Masses and Orbital Fits for {\ensuremath{\beta}} Pic b and {\ensuremath{\beta}} Pic c}",
      journal = {\aj},
     keywords = {Exoplanet astronomy, Exoplanet dynamics, Exoplanet systems, Exoplanet formation, Radial velocity, Pulsating variable stars, Brown dwarfs, Exoplanet evolution, 486, 490, 484, 492, 1332, 1307, 185, 491, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = apr,
       volume = {161},
       number = {4},
          eid = {179},
        pages = {179},
          doi = {10.3847/1538-3881/abdc2e},
archivePrefix = {arXiv},
       eprint = {2011.06215},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..179B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chilcote+2017,
       author = {{Chilcote}, Jeffrey and {Pueyo}, Laurent and {De Rosa}, Robert J. and {Vargas}, Jeffrey and {Macintosh}, Bruce and {Bailey}, Vanessa P. and {Barman}, Travis and {Bauman}, Brian and {Bruzzone}, Sebastian and {Bulger}, Joanna and {Burrows}, Adam S. and {Cardwell}, Andrew and {Chen}, Christine H. and {Cotten}, Tara and {Dillon}, Daren and {Doyon}, Rene and {Draper}, Zachary H. and {Duch{\^e}ne}, Gaspard and {Dunn}, Jennifer and {Erikson}, Darren and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Gavel}, Donald and {Goodsell}, Stephen J. and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hartung}, Markus and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Kalas}, Paul and {Konopacky}, Quinn and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marley}, Mark S. and {Marois}, Christian and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Morzinski}, Katie M. and {Nielsen}, Eric L. and {Norton}, Andrew and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Rajan}, Abhijith and {Rameau}, Julien and {Rantakyr{\"o}}, Fredrik T. and {Sadakuni}, Naru and {Saddlemyer}, Leslie and {Savransky}, Dmitry and {Schneider}, Adam C. and {Serio}, Andrew and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Wang}, Jason J. and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{1-2.4 {\ensuremath{\mu}}m Near-IR Spectrum of the Giant Planet {\ensuremath{\beta}} Pictoris b Obtained with the Gemini Planet Imager}",
      journal = {\aj},
     keywords = {instrumentation: adaptive optics, planetary systems, stars: individual: beta Pictoris, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = apr,
       volume = {153},
       number = {4},
          eid = {182},
        pages = {182},
          doi = {10.3847/1538-3881/aa63e9},
archivePrefix = {arXiv},
       eprint = {1703.00011},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....153..182C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Suarez+2021,
       author = {{Su{\'a}rez}, Genaro and {Metchev}, Stanimir and {Leggett}, Sandy K. and {Saumon}, Didier and {Marley}, Mark S.},
        title = "{Ultracool Dwarfs Observed with the Spitzer Infrared Spectrograph. I. An Accurate Look at the L-to-T Transition at  300 Myr from Optical Through Mid-infrared Spectrophotometry}",
      journal = {\apj},
     keywords = {Brown dwarfs, 185, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {99},
        pages = {99},
          doi = {10.3847/1538-4357/ac1418},
archivePrefix = {arXiv},
       eprint = {2107.14282},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920...99S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tannock+2022,
       author = {{Tannock}, Megan E. and {Metchev}, Stanimir and {Hood}, Callie E. and {Mace}, Gregory N. and {Fortney}, Jonathan J. and {Morley}, Caroline V. and {Jaffe}, Daniel T. and {Lupu}, Roxana},
        title = "{A 1.46-2.48 {\ensuremath{\mu}}m spectroscopic atlas of a T6 dwarf (1060 K) atmosphere with IGRINS: first detections of H$_{2}$S and H$_{2}$, and verification of H$_{2}$O, CH$_{4}$, and NH$_{3}$ line lists}",
      journal = {\mnras},
     keywords = {techniques: spectroscopic, planets and satellites: atmospheres, stars: atmospheres, brown dwarfs, stars: individual: 2MASS J08173001-6155158, line: identification, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = aug,
       volume = {514},
       number = {3},
        pages = {3160-3178},
          doi = {10.1093/mnras/stac1412},
archivePrefix = {arXiv},
       eprint = {2206.03519},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.514.3160T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley+2012,
       author = {{Marley}, Mark S. and {Saumon}, Didier and {Cushing}, Michael and {Ackerman}, Andrew S. and {Fortney}, Jonathan J. and {Freedman}, Richard},
        title = "{Masses, Radii, and Cloud Properties of the HR 8799 Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: individual: HR 8799, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = aug,
       volume = {754},
       number = {2},
          eid = {135},
        pages = {135},
          doi = {10.1088/0004-637X/754/2/135},
archivePrefix = {arXiv},
       eprint = {1205.6488},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...754..135M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirkpatrick+2008,
       author = {{Kirkpatrick}, J. Davy and {Cruz}, Kelle L. and {Barman}, Travis S. and {Burgasser}, Adam J. and {Looper}, Dagny L. and {Tinney}, C.~G. and {Gelino}, Christopher R. and {Lowrance}, Patrick J. and {Liebert}, James and {Carpenter}, John M. and {Hillenbrand}, Lynne A. and {Stauffer}, John R.},
        title = "{A Sample of Very Young Field L Dwarfs and Implications for the Brown Dwarf ``Lithium Test'' at Early Ages}",
      journal = {\apj},
     keywords = {binaries: general, stars: fundamental parameters, stars: late-type, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = dec,
       volume = {689},
       number = {2},
        pages = {1295-1326},
          doi = {10.1086/592768},
archivePrefix = {arXiv},
       eprint = {0808.3153},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...689.1295K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Curri+2011,
       author = {{Currie}, Thayne and {Burrows}, Adam and {Itoh}, Yoichi and {Matsumura}, Soko and {Fukagawa}, Misato and {Apai}, Daniel and {Madhusudhan}, Nikku and {Hinz}, Philip M. and {Rodigas}, T.~J. and {Kasper}, Markus and {Pyo}, T. -S. and {Ogino}, Satoshi},
        title = "{A Combined Subaru/VLT/MMT 1-5 {\ensuremath{\mu}}m Study of Planets Orbiting HR 8799: Implications for Atmospheric Properties, Masses, and Formation}",
      journal = {\apj},
     keywords = {brown dwarfs, instrumentation: adaptive optics, planetary systems, stars: individual: HR 8799, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = mar,
       volume = {729},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.1088/0004-637X/729/2/128},
archivePrefix = {arXiv},
       eprint = {1101.1973},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729..128C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Exo-DMC,
       author = {{Bonavita}, Mariangela},
        title = "{Exo-DMC: Exoplanet Detection Map Calculator}",
     keywords = {Software},
 howpublished = {Astrophysics Source Code Library, record ascl:2010.008},
         year = 2020,
        month = oct,
          eid = {ascl:2010.008},
        pages = {ascl:2010.008},
archivePrefix = {ascl},
       eprint = {2010.008},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ascl.soft10008B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dupuy+2023,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C. and {Evans}, Elise L. and {Best}, William M.~J. and {Pearce}, Logan A. and {Sanghi}, Aniket and {Phillips}, Mark W. and {Bardalez Gagliuffi}, Daniella C.},
        title = "{On the masses, age, and architecture of the VHS J1256-1257AB b system}",
      journal = {\mnras},
     keywords = {astrometry, planetary systems, binaries: visual, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = feb,
       volume = {519},
       number = {2},
        pages = {1688-1694},
          doi = {10.1093/mnras/stac3557},
archivePrefix = {arXiv},
       eprint = {2208.08448},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.519.1688D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petrus+2023,
       author = {{Petrus}, S. and {Chauvin}, G. and {Bonnefoy}, M. and {Tremblin}, P. and {Charnay}, B. and {Delorme}, P. and {Marleau}, G. -D. and {Bayo}, A. and {Manjavacas}, E. and {Lagrange}, A. -M. and {Molli{\`e}re}, P. and {Palma-Bifani}, P. and {Biller}, B. and {Jenkins}, J. -S. and {Goyal}, J. -M. and {Hoch}, K.},
        title = "{X-SHYNE: X-shooter spectra of young exoplanet analogs. I. A medium-resolution 0.65-2.5 {\ensuremath{\mu}}m one-shot spectrum of VHS 1256{\ensuremath{-}}1257 b}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, planets and satellites: atmospheres, planets and satellites: formation, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = feb,
       volume = {670},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/202244494},
archivePrefix = {arXiv},
       eprint = {2207.06622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A\&A...670L...9P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Charnay+2018,
       author = {{Charnay}, B. and {B{\'e}zard}, B. and {Baudino}, J. -L. and {Bonnefoy}, M. and {Boccaletti}, A. and {Galicher}, R.},
        title = "{A Self-consistent Cloud Model for Brown Dwarfs and Young Giant Exoplanets: Comparison with Photometric and Spectroscopic Observations}",
      journal = {\apj},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = feb,
       volume = {854},
       number = {2},
          eid = {172},
        pages = {172},
          doi = {10.3847/1538-4357/aaac7d},
archivePrefix = {arXiv},
       eprint = {1711.11483},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...854..172C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baudino+2015,
       author = {{Baudino}, J. -L. and {B{\'e}zard}, B. and {Boccaletti}, A. and {Bonnefoy}, M. and {Lagrange}, A. -M. and {Galicher}, R.},
        title = "{Interpreting the photometry and spectroscopy of directly imaged planets: a new atmospheric model applied to {\ensuremath{\beta}} Pictoris b and SPHERE observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, stars: individual: beta Pictoris, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A83},
        pages = {A83},
          doi = {10.1051/0004-6361/201526332},
archivePrefix = {arXiv},
       eprint = {1504.04876},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A\&A...582A..83B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blain+2021,
       author = {{Blain}, D. and {Charnay}, B. and {B{\'e}zard}, B.},
        title = "{1D atmospheric study of the temperate sub-Neptune K2-18b}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, infrared: planetary systems, planets and satellites: gaseous planets, molecular data, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = feb,
       volume = {646},
          eid = {A15},
        pages = {A15},
          doi = {10.1051/0004-6361/202039072},
archivePrefix = {arXiv},
       eprint = {2011.10459},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A\&A...646A..15B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stolker+2020,
       author = {{Stolker}, T. and {Quanz}, S.~P. and {Todorov}, K.~O. and {K{\"u}hn}, J. and {Molli{\`e}re}, P. and {Meyer}, M.~R. and {Currie}, T. and {Daemgen}, S. and {Lavie}, B.},
        title = "{MIRACLES: atmospheric characterization of directly imaged planets and substellar companions at 4-5 {\ensuremath{\mu}}m. I. Photometric analysis of {\ensuremath{\beta}} Pic b, HIP 65426 b, PZ Tel B, and HD 206893 B}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, methods: data analysis, techniques: high angular resolution, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = mar,
       volume = {635},
          eid = {A182},
        pages = {A182},
          doi = {10.1051/0004-6361/201937159},
archivePrefix = {arXiv},
       eprint = {1912.13316},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A\&A...635A.182S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Linder+2019,
       author = {{Linder}, Esther F. and {Mordasini}, Christoph and {Molli{\`e}re}, Paul and {Marleau}, Gabriel-Dominique and {Malik}, Matej and {Quanz}, Sascha P. and {Meyer}, Michael R.},
        title = "{Evolutionary models of cold and low-mass planets: cooling curves, magnitudes, and detectability}",
      journal = {\aap},
     keywords = {planets and satellites: physical evolution, planets and satellites: atmospheres, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A85},
        pages = {A85},
          doi = {10.1051/0004-6361/201833873},
archivePrefix = {arXiv},
       eprint = {1812.02027},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A\&A...623A..85L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard+2001,
       author = {{Allard}, France and {Hauschildt}, Peter H. and {Alexander}, David R. and {Tamanai}, Akemi and {Schweitzer}, Andreas},
        title = "{The Limiting Effects of Dust in Brown Dwarf Model Atmospheres}",
      journal = {\apj},
     keywords = {Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2001,
        month = jul,
       volume = {556},
       number = {1},
        pages = {357-372},
          doi = {10.1086/321547},
archivePrefix = {arXiv},
       eprint = {astro-ph/0104256},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...556..357A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cushing+2005,
       author = {{Cushing}, Michael C. and {Rayner}, John T. and {Vacca}, William D.},
        title = "{An Infrared Spectroscopic Sequence of M, L, and T Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: 2MASS J2224381-0158521, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2005,
        month = apr,
       volume = {623},
       number = {2},
        pages = {1115-1140},
          doi = {10.1086/428040},
archivePrefix = {arXiv},
       eprint = {astro-ph/0412313},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...623.1115C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mawet+2014,
       author = {{Mawet}, D. and {Milli}, J. and {Wahhaj}, Z. and {Pelat}, D. and {Absil}, O. and {Delacroix}, C. and {Boccaletti}, A. and {Kasper}, M. and {Kenworthy}, M. and {Marois}, C. and {Mennesson}, B. and {Pueyo}, L.},
        title = "{Fundamental Limitations of High Contrast Imaging Set by Small Sample Statistics}",
      journal = {\apj},
     keywords = {methods: statistical, techniques: high angular resolution, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = sep,
       volume = {792},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.1088/0004-637X/792/2/97},
archivePrefix = {arXiv},
       eprint = {1407.2247},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792...97M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kammerer+2022,
       author = {{Kammerer}, Jens and {Girard}, Julien and {Carter}, Aarynn L. and {Perrin}, Marshall D. and {Cooper}, Rachel and {Thatte}, Deepashri and {Vandal}, Thomas and {Leisenring}, Jarron and {Wang}, Jason and {Balmer}, William O. and {Sivaramakrishnan}, Anand and {Pueyo}, Laurent and {Ward-Duong}, Kimberly and {Sunnquist}, Ben and {Adams Redai}, J{\'e}a.},
        title = "{Performance of near-infrared high-contrast imaging methods with JWST from commissioning}",
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Space Telescopes and Instrumentation 2022: Optical, Infrared, and Millimeter Wave},
         year = 2022,
       editor = {{Coyle}, Laura E. and {Matsuura}, Shuji and {Perrin}, Marshall D.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {12180},
        month = aug,
          eid = {121803N},
        pages = {121803N},
          doi = {10.1117/12.2628865},
archivePrefix = {arXiv},
       eprint = {2208.00996},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022SPIE12180E..3NK},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Bushouse+2022,
       author = {{Bushouse}, Howard and {Eisenhamer}, Jonathan and {Dencheva}, Nadia and {Davies}, James and {Greenfield}, Perry and {Morrison}, Jane and {Hodge}, Phil and {Simon}, Bernie and {Grumm}, David and {Droettboom}, Michael and {Slavich}, Edward and {Sosey}, Megan and {Pauly}, Tyler and {Miller}, Todd and {Jedrzejewski}, Robert and {Hack}, Warren and {Davis}, David and {Crawford}, Steven and {Law}, David and {Gordon}, Karl and {Regan}, Michael and {Cara}, Mihai and {MacDonald}, Ken and {Bradley}, Larry and {Shanahan}, Clare and {Jamieson}, William},
        title = "{spacetelescope/jwst: JWST 1.6.2}",
 howpublished = {Zenodo},
         year = 2022,
        month = aug,
          eid = {10.5281/zenodo.6984366},
          doi = {10.5281/zenodo.6984366},
      version = {1.6.2},
    publisher = {Zenodo},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022zndo...6984366B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Wang+2015,
       author = {{Wang}, Jason J. and {Ruffio}, Jean-Baptise and {De Rosa}, Robert J. and {Aguilar}, Jonathan and {Wolff}, Schuyler G. and {Pueyo}, Laurent},
        title = "{pyKLIP: PSF Subtraction for Exoplanets and Disks}",
     keywords = {Software},
 howpublished = {Astrophysics Source Code Library, record ascl:1506.001},
         year = 2015,
        month = jun,
          eid = {ascl:1506.001},
        pages = {ascl:1506.001},
archivePrefix = {ascl},
       eprint = {1506.001},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ascl.soft06001W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Soummer+2012,
       author = {{Soummer}, R{\'e}mi and {Pueyo}, Laurent and {Larkin}, James},
        title = "{Detection and Characterization of Exoplanets and Disks Using Projections on Karhunen-Lo{\`e}ve Eigenimages}",
      journal = {\apjl},
     keywords = {methods: data analysis, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = aug,
       volume = {755},
       number = {2},
          eid = {L28},
        pages = {L28},
          doi = {10.1088/2041-8205/755/2/L28},
archivePrefix = {arXiv},
       eprint = {1207.4197},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...755L..28S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Close+2012,
       author = {{Close}, Laird M. and {Males}, Jared R. and {Kopon}, Derek A. and {Gasho}, Victor and {Follette}, Katherine B. and {Hinz}, Phil and {Morzinski}, Katie and {Uomoto}, Alan and {Hare}, Tyson and {Riccardi}, Armando and {Esposito}, Simone and {Puglisi}, Alfio and {Pinna}, Enrico and {Busoni}, Lorenzo and {Arcidiacono}, Carmelo and {Xompero}, Marco and {Briguglio}, Runa and {Quiros-Pacheco}, Fernando and {Argomedo}, Javier},
        title = "{First closed-loop visible AO test results for the advanced adaptive secondary AO system for the Magellan Telescope: MagAO's performance and status}",
    booktitle = {Adaptive Optics Systems III},
         year = 2012,
       editor = {{Ellerbroek}, Brent L. and {Marchetti}, Enrico and {V{\'e}ran}, Jean-Pierre},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {8447},
        month = jul,
          eid = {84470X},
        pages = {84470X},
          doi = {10.1117/12.926545},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SPIE.8447E..0XC},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Morzinski+2014,
       author = {{Morzinski}, Katie M. and {Close}, Laird M. and {Males}, Jared R. and {Kopon}, Derek and {Hinz}, Phil M. and {Esposito}, Simone and {Riccardi}, Armando and {Puglisi}, Alfio and {Pinna}, Enrico and {Briguglio}, Runa and {Xompero}, Marco and {Quir{\'o}s-Pacheco}, Fernando and {Bailey}, Vanessa and {Follette}, Katherine B. and {Rodigas}, T.~J. and {Wu}, Ya-Lin and {Arcidiacono}, Carmelo and {Argomedo}, Javier and {Busoni}, Lorenzo and {Hare}, Tyson and {Uomoto}, Alan and {Weinberger}, Alycia},
        title = "{MagAO: Status and on-sky performance of the Magellan adaptive optics system}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Adaptive Optics Systems IV},
         year = 2014,
       editor = {{Marchetti}, Enrico and {Close}, Laird M. and {Vran}, Jean-Pierre},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9148},
        month = jul,
          eid = {914804},
        pages = {914804},
          doi = {10.1117/12.2057048},
archivePrefix = {arXiv},
       eprint = {1407.5098},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9148E..04M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allers+2013,
       author = {{Allers}, K.~N. and {Liu}, Michael C.},
        title = "{A Near-infrared Spectroscopic Study of Young Field Ultracool Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, planets and satellites: atmospheres, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = aug,
       volume = {772},
       number = {2},
          eid = {79},
        pages = {79},
          doi = {10.1088/0004-637X/772/2/79},
archivePrefix = {arXiv},
       eprint = {1305.4418},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...772...79A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Filippazzo+2015,
       author = {{Filippazzo}, Joseph C. and {Rice}, Emily L. and {Faherty}, Jacqueline and {Cruz}, Kelle L. and {Van Gordon}, Mollie M. and {Looper}, Dagny L.},
        title = "{Fundamental Parameters and Spectral Energy Distributions of Young and Field Age Objects with Masses Spanning the Stellar to Planetary Regime}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: fundamental parameters, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {810},
       number = {2},
          eid = {158},
        pages = {158},
          doi = {10.1088/0004-637X/810/2/158},
archivePrefix = {arXiv},
       eprint = {1508.01767},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...810..158F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodders+Fegley-2002,
       author = {{Lodders}, Katharina and {Fegley}, Bruce},
        title = "{Atmospheric Chemistry in Giant Planets, Brown Dwarfs, and Low-Mass Dwarf Stars. I. Carbon, Nitrogen, and Oxygen}",
      journal = {\icarus},
     keywords = {Earth Science, Earth Science},
         year = 2002,
        month = feb,
       volume = {155},
       number = {2},
        pages = {393-424},
          doi = {10.1006/icar.2001.6740},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002Icar..155..393L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoch+2022,
       author = {{Hoch}, Kielan K.~W. and {Konopacky}, Quinn M. and {Barman}, Travis S. and {Theissen}, Christopher A. and {Brock}, Laci and {Perrin}, Marshall D. and {Ruffio}, Jean-Baptiste and {Macintosh}, Bruce and {Marois}, Christian},
        title = "{Moderate-resolution K-band Spectroscopy of the Substellar Companion VHS 1256 b}",
      journal = {\aj},
     keywords = {Direct imaging, Exoplanet atmospheres, High resolution spectroscopy, Exoplanet formation, Brown dwarfs, 387, 487, 2096, 492, 185, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = oct,
       volume = {164},
       number = {4},
          eid = {155},
        pages = {155},
          doi = {10.3847/1538-3881/ac84d4},
archivePrefix = {arXiv},
       eprint = {2207.03819},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....164..155H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Fusco+2013,
       author = {{Fusco}, Thierry and {Sauvage}, Jean-Fran{\c{c}}ois and {Petit}, Cyril and {Costille}, Anne and {Dohlen}, Kjetil and {Beuzit}, Jean-Luc and {Mouillet}, David and {Puget}, Pascal and {Gluck}, Laurence and {Rochat}, Sylvain and {Baruffolo}, Andrea and {Salasnich}, Bernardo and {Kasper}, Markus and {Suarez}, Marcos and {Soenke}, Christian and {Fedrigo}, Enrico and {Baudoz}, Pierre and {Sevin}, Arnaud and {Perret}, Denis and {Wildi}, Fran{\c{c}}ois},
        title = "{Integration of SAXO, the VLT-SPHERE extreme AO : final performance}",
     keywords = {AO pathfinders and new ideas},
    booktitle = {Proceedings of the Third AO4ELT Conference},
         year = 2013,
       editor = {{Esposito}, Simone and {Fini}, Luca},
        month = dec,
          eid = {69},
        pages = {69},
          doi = {10.12839/AO4ELT3.13327},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013aoel.confE..69F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Danielski+2018,
       author = {{Danielski}, Camilla and {Baudino}, Jean-Loup and {Lagage}, Pierre-Olivier and {Boccaletti}, Anthony and {Gastaud}, Ren{\'e} and {Coulais}, Alain and {B{\'e}zard}, Bruno},
        title = "{Atmospheric Characterization of Directly Imaged Exoplanets with JWST/MIRI}",
      journal = {\aj},
     keywords = {instrumentation: high angular resolution, instrumentation: spectrographs, planets and satellites: atmospheres, planets and satellites: fundamental parameters, planets and satellites: gaseous planets, telescopes, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = dec,
       volume = {156},
       number = {6},
          eid = {276},
        pages = {276},
          doi = {10.3847/1538-3881/aae651},
archivePrefix = {arXiv},
       eprint = {1810.00894},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..276D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Malin+2023,
       author = {{M{\^a}lin}, M. and {Boccaletti}, A. and {Charnay}, B. and {Kiefer}, F. and {B{\'e}zard}, B.},
        title = "{Simulated performance of the molecular mapping for young giant exoplanets with the Medium-Resolution Spectrometer of JWST/MIRI}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, techniques: imaging spectroscopy, planets and satellites: gaseous planets, space vehicles: instruments, methods: data analysis, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = mar,
       volume = {671},
          eid = {A109},
        pages = {A109},
          doi = {10.1051/0004-6361/202245094},
archivePrefix = {arXiv},
       eprint = {2301.02116},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A\&A...671A.109M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rigby+2023,
       author = {{Rigby}, Jane and {Perrin}, Marshall and {McElwain}, Michael and {Kimble}, Randy and {Friedman}, Scott and {Lallo}, Matt and {Doyon}, Ren{\'e} and {Feinberg}, Lee and {Ferruit}, Pierre and {Glasse}, Alistair and {Rieke}, Marcia and {Rieke}, George and {Wright}, Gillian and {Willott}, Chris and {Colon}, Knicole and {Milam}, Stefanie and {Neff}, Susan and {Stark}, Christopher and {Valenti}, Jeff and {Abell}, Jim and {Abney}, Faith and {Abul-Huda}, Yasin and {Acton}, D. Scott and {Adams}, Evan and {Adler}, David and {Aguilar}, Jonathan and {Ahmed}, Nasif and {Albert}, Lo{\"\i}c and {Alberts}, Stacey and {Aldridge}, David and {Allen}, Marsha and {Altenburg}, Martin and {{\'A}lvarez-M{\'a}rquez}, Javier and {Alves de Oliveira}, Catarina and {Andersen}, Greg and {Anderson}, Harry and {Anderson}, Sara and {Argyriou}, Ioannis and {Armstrong}, Amber and {Arribas}, Santiago and {Artigau}, Etienne and {Arvai}, Amanda and {Atkinson}, Charles and {Bacon}, Gregory and {Bair}, Thomas and {Banks}, Kimberly and {Barrientes}, Jaclyn and {Barringer}, Bruce and {Bartosik}, Peter and {Bast}, William and {Baudoz}, Pierre and {Beatty}, Thomas and {Bechtold}, Katie and {Beck}, Tracy and {Bergeron}, Eddie and {Bergkoetter}, Matthew and {Bhatawdekar}, Rachana and {Birkmann}, Stephan and {Blazek}, Ronald and {Blome}, Claire and {Boccaletti}, Anthony and {B{\"o}ker}, Torsten and {Boia}, John and {Bonaventura}, Nina and {Bond}, Nicholas and {Bosley}, Kari and {Boucarut}, Ray and {Bourque}, Matthew and {Bouwman}, Jeroen and {Bower}, Gary and {Bowers}, Charles and {Boyer}, Martha and {Bradley}, Larry and {Brady}, Greg and {Braun}, Hannah and {Breda}, David and {Bresnahan}, Pamela and {Bright}, Stacey and {Britt}, Christopher and {Bromenschenkel}, Asa and {Brooks}, Brian and {Brooks}, Keira and {Brown}, Bob and {Brown}, Matthew and {Brown}, Patricia and {Bunker}, Andy and {Burger}, Matthew and {Bushouse}, Howard and {Cale}, Steven and {Cameron}, Alex and {Cameron}, Peter and {Canipe}, Alicia and {Caplinger}, James and {Caputo}, Francis and {Cara}, Mihai and {Carey}, Larkin and {Carniani}, Stefano and {Carrasquilla}, Maria and {Carruthers}, Margaret and {Case}, Michael and {Catherine}, Riggs and {Chance}, Don and {Chapman}, George and {Charlot}, St{\'e}phane and {Charlow}, Brian and {Chayer}, Pierre and {Chen}, Bin and {Cherinka}, Brian and {Chichester}, Sarah and {Chilton}, Zack and {Chonis}, Taylor and {Clampin}, Mark and {Clark}, Charles and {Clark}, Kerry and {Coe}, Dan and {Coleman}, Benee and {Comber}, Brian and {Comeau}, Tom and {Connolly}, Dennis and {Cooper}, James and {Cooper}, Rachel and {Coppock}, Eric and {Correnti}, Matteo and {Cossou}, Christophe and {Coulais}, Alain and {Coyle}, Laura and {Cracraft}, Misty and {Curti}, Mirko and {Cuturic}, Steven and {Davis}, Katherine and {Davis}, Michael and {Dean}, Bruce and {DeLisa}, Amy and {deMeester}, Wim and {Dencheva}, Nadia and {Dencheva}, Nadezhda and {DePasquale}, Joseph and {Deschenes}, Jeremy and {Hunor Detre}, {\"O}rs and {Diaz}, Rosa and {Dicken}, Dan and {DiFelice}, Audrey and {Dillman}, Matthew and {Dixon}, William and {Doggett}, Jesse and {Donaldson}, Tom and {Douglas}, Rob and {DuPrie}, Kimberly and {Dupuis}, Jean and {Durning}, John and {Easmin}, Nilufar and {Eck}, Weston and {Edeani}, Chinwe and {Egami}, Eiichi and {Ehrenwinkler}, Ralf and {Eisenhamer}, Jonathan and {Eisenhower}, Michael and {Elie}, Michelle and {Elliott}, James and {Elliott}, Kyle and {Ellis}, Tracy and {Engesser}, Michael and {Espinoza}, Nestor and {Etienne}, Odessa and {Etxaluze}, Mireya and {Falini}, Patrick and {Feeney}, Matthew and {Ferry}, Malcolm and {Filippazzo}, Joseph and {Fincham}, Brian and {Fix}, Mees and {Flagey}, Nicolas and {Florian}, Michael and {Flynn}, Jim and {Fontanella}, Erin and {Ford}, Terrance and {Forshay}, Peter and {Fox}, Ori and {Franz}, David and {Fu}, Henry and {Fullerton}, Alexander and {Galkin}, Sergey and {Galyer}, Anthony and {Garc{\'\i}a Mar{\'\i}n}, Macarena and {Gardner}, Jonathan P. and {Gardner}, Lisa and {Garland}, Dennis and {Garrett}, Bruce and {Gasman}, Danny and {Gaspar}, Andras and {Gaudreau}, Daniel and {Gauthier}, Peter and {Geers}, Vincent and {Geithner}, Paul and {Gennaro}, Mario and {Giardino}, Giovanna and {Girard}, Julien and {Giuliano}, Mark and {Glassmire}, Kirk and {Glauser}, Adrian and {Glazer}, Stuart and {Godfrey}, John and {Golimowski}, David and {Gollnitz}, David and {Gong}, Fan and {Gonzaga}, Shireen and {Gordon}, Michael and {Gordon}, Karl and {Goudfrooij}, Paul and {Greene}, Thomas and {Greenhouse}, Matthew and {Grimaldi}, Stefano and {Groebner}, Andrew and {Grundy}, Timothy and {Guillard}, Pierre and {Gutman}, Irvin and {Ha}, Kong Q. and {Haderlein}, Peter and {Hagedorn}, Andria and {Hainline}, Kevin and {Haley}, Craig and {Hami}, Maryam and {Hamilton}, Forrest and {Hammel}, Heidi and {Hansen}, Carl and {Harkins}, Tom and {Harr}, Michael and {Hart}, Jessica and {Hart}, Quyen and {Hartig}, George and {Hashimoto}, Ryan and {Haskins}, Sujee and {Hathaway}, William and {Havey}, Keith and {Hayden}, Brian and {Hecht}, Karen and {Heller-Boyer}, Chris and {Henriques}, Caroline and {Henry}, Alaina and {Hermann}, Karl and {Hernandez}, Scarlin and {Hesman}, Brigette and {Hicks}, Brian and {Hilbert}, Bryan and {Hines}, Dean and {Hoffman}, Melissa and {Holfeltz}, Sherie and {Holler}, Bryan J. and {Hoppa}, Jennifer and {Hott}, Kyle and {Howard}, Joseph M. and {Howard}, Rick and {Hunter}, Alexander and {Hunter}, David and {Hurst}, Brendan and {Husemann}, Bernd and {Hustak}, Leah and {Ilinca Ignat}, Luminita and {Illingworth}, Garth and {Irish}, Sandra and {Jackson}, Wallace and {Jahromi}, Amir and {Jakobsen}, Peter and {James}, LeAndrea and {James}, Bryan and {Januszewski}, William and {Jenkins}, Ann and {Jirdeh}, Hussein and {Johnson}, Phillip and {Johnson}, Timothy and {Jones}, Vicki and {Jones}, Ron and {Jones}, Danny and {Jones}, Olivia and {Jordan}, Ian and {Jordan}, Margaret and {Jurczyk}, Sarah and {Jurling}, Alden and {Kaleida}, Catherine and {Kalmanson}, Phillip and {Kammerer}, Jens and {Kang}, Huijo and {Kao}, Shaw-Hong and {Karakla}, Diane and {Kavanagh}, Patrick and {Kelly}, Doug and {Kendrew}, Sarah and {Kennedy}, Herbert and {Kenny}, Deborah and {Keski-kuha}, Ritva and {Keyes}, Charles and {Kidwell}, Richard and {Kinzel}, Wayne and {Kirk}, Jeff and {Kirkpatrick}, Mark and {Kirshenblat}, Danielle and {Klaassen}, Pamela and {Knapp}, Bryan and {Knight}, J. Scott and {Knollenberg}, Perry and {Koehler}, Robert and {Koekemoer}, Anton and {Kovacs}, Aiden and {Kulp}, Trey and {Kumari}, Nimisha and {Kyprianou}, Mark and {La Massa}, Stephanie and {Labador}, Aurora and {Labiano}, Alvaro and {Lagage}, Pierre-Olivier and {Lajoie}, Charles-Philippe and {Lallo}, Matthew and {Lam}, May and {Lamb}, Tracy and {Lambros}, Scott and {Lampenfield}, Richard and {Langston}, James and {Larson}, Kirsten and {Law}, David and {Lawrence}, Jon and {Lee}, David and {Leisenring}, Jarron and {Lepo}, Kelly and {Leveille}, Michael and {Levenson}, Nancy and {Levine}, Marie and {Levy}, Zena and {Lewis}, Dan and {Lewis}, Hannah and {Libralato}, Mattia and {Lightsey}, Paul and {Link}, Miranda and {Liu}, Lily and {Lo}, Amy and {Lockwood}, Alexandra and {Logue}, Ryan and {Long}, Chris and {Long}, Douglas and {Loomis}, Charles and {Lopez-Caniego}, Marcos and {Lorenzo Alvarez}, Jose and {Love-Pruitt}, Jennifer and {Lucy}, Adrian and {Luetzgendorf}, Nora and {Maghami}, Peiman and {Maiolino}, Roberto and {Major}, Melissa and {Malla}, Sunita and {Malumuth}, Eliot and {Manjavacas}, Elena and {Mannfolk}, Crystal and {Marrione}, Amanda and {Marston}, Anthony and {Martel}, Andr{\'e} and {Maschmann}, Marc and {Masci}, Gregory and {Masciarelli}, Michaela and {Maszkiewicz}, Michael and {Mather}, John and {McKenzie}, Kenny and {McLean}, Brian and {McMaster}, Matthew and {Melbourne}, Katie and {Mel{\'e}ndez}, Marcio and {Menzel}, Michael and {Merz}, Kaiya and {Meyett}, Michele and {Meza}, Luis and {Miskey}, Cherie and {Misselt}, Karl and {Moller}, Christopher and {Morrison}, Jane and {Morse}, Ernie and {Moseley}, Harvey and {Mosier}, Gary and {Mountain}, Matt and {Mueckay}, Julio and {Mueller}, Michael and {Mullally}, Susan and {Murphy}, Jess and {Murray}, Katherine and {Murray}, Claire and {Mustelier}, David and {Muzerolle}, James and {Mycroft}, Matthew and {Myers}, Richard and {Myrick}, Kaila and {Nanavati}, Shashvat and {Nance}, Elizabeth and {Nayak}, Omnarayani and {Naylor}, Bret and {Nelan}, Edmund and {Nickson}, Bryony and {Nielson}, Alethea and {Nieto-Santisteban}, Maria and {Nikolov}, Nikolay and {Noriega-Crespo}, Alberto and {O'Shaughnessy}, Brian and {O'Sullivan}, Brian and {Ochs}, William and {Ogle}, Patrick and {Oleszczuk}, Brenda and {Olmsted}, Joseph and {Osborne}, Shannon and {Ottens}, Richard and {Owens}, Beverly and {Pacifici}, Camilla and {Pagan}, Alyssa and {Page}, James and {Park}, Sang and {Parrish}, Keith and {Patapis}, Polychronis and {Paul}, Lee and {Pauly}, Tyler and {Pavlovsky}, Cheryl and {Pedder}, Andrew and {Peek}, Matthew and {Pena-Guerrero}, Maria and {Penanen}, Konstantin and {Perez}, Yesenia and {Perna}, Michele and {Perriello}, Beth and {Phillips}, Kevin and {Pietraszkiewicz}, Martin and {Pinaud}, Jean-Paul and {Pirzkal}, Norbert and {Pitman}, Joseph and {Piwowar}, Aidan and {Platais}, Vera and {Player}, Danielle and {Plesha}, Rachel and {Pollizi}, Joe and {Polster}, Ethan and {Pontoppidan}, Klaus and {Porterfield}, Blair and {Proffitt}, Charles and {Pueyo}, Laurent and {Pulliam}, Christine and {Quirt}, Brian and {Quispe Neira}, Irma and {Ramos Alarcon}, Rafael and {Ramsay}, Leah and {Rapp}, Greg and {Rapp}, Robert and {Rauscher}, Bernard and {Ravindranath}, Swara and {Rawle}, Timothy and {Regan}, Michael and {Reichard}, Timothy A. and {Reis}, Carl and {Ressler}, Michael E. and {Rest}, Armin and {Reynolds}, Paul and {Rhue}, Timothy and {Richon}, Karen and {Rickman}, Emily and {Ridgaway}, Michael and {Ritchie}, Christine and {Rix}, Hans-Walter and {Robberto}, Massimo and {Robinson}, Gregory and {Robinson}, Michael and {Robinson}, Orion and {Rock}, Frank and {Rodriguez}, David and {Rodriguez Del Pino}, Bruno and {Roellig}, Thomas and {Rohrbach}, Scott and {Roman}, Anthony and {Romelfanger}, Fred and {Rose}, Perry and {Roteliuk}, Anthony and {Roth}, Marc and {Rothwell}, Braden and {Rowlands}, Neil and {Roy}, Arpita and {Royer}, Pierre and {Royle}, Patricia and {Rui}, Chunlei and {Rumler}, Peter and {Runnels}, Joel and {Russ}, Melissa and {Rustamkulov}, Zafar and {Ryden}, Grant and {Ryer}, Holly and {Sabata}, Modhumita and {Sabatke}, Derek and {Sabbi}, Elena and {Samuelson}, Bridget and {Sapp}, Benjamin and {Sappington}, Bradley and {Sargent}, B. and {Sauer}, Arne and {Scheithauer}, Silvia and {Schlawin}, Everett and {Schlitz}, Joseph and {Schmitz}, Tyler and {Schneider}, Analyn and {Schreiber}, J{\"u}rgen and {Schulze}, Vonessa and {Schwab}, Ryan and {Scott}, John and {Sembach}, Kenneth and {Shanahan}, Clare and {Shaughnessy}, Bryan and {Shaw}, Richard and {Shawger}, Nanci and {Shay}, Christopher and {Sheehan}, Evan and {Shen}, Sharon and {Sherman}, Allan and {Shiao}, Bernard and {Shih}, Hsin-Yi and {Shivaei}, Irene and {Sienkiewicz}, Matthew and {Sing}, David and {Sirianni}, Marco and {Sivaramakrishnan}, Anand and {Skipper}, Joy and {Sloan}, G.~C. and {Slocum}, Christine and {Slowinski}, Steven and {Smith}, Erin and {Smith}, Eric and {Smith}, Denise and {Smith}, Corbett and {Snyder}, Gregory and {Soh}, Warren and {Sohn}, Sangmo Tony and {Soto}, Christian and {Spencer}, Richard and {Stallcup}, Scott and {Stansberry}, John and {Starr}, Carl and {Starr}, Elysia and {Stewart}, Alphonso and {Stiavelli}, Massimo and {Straughn}, Amber and {Strickland}, David and {Stys}, Jeff and {Summers}, Francis and {Sun}, Fengwu and {Sunnquist}, Ben and {Swade}, Daryl and {Swam}, Michael and {Swaters}, Robert and {Swoish}, Robby and {Taylor}, Joanna M. and {Taylor}, Rolanda and {Te Plate}, Maurice and {Tea}, Mason and {Teague}, Kelly and {Telfer}, Randal and {Temim}, Tea and {Thatte}, Deepashri and {Thompson}, Christopher and {Thompson}, Linda and {Thomson}, Shaun and {Tikkanen}, Tuomo and {Tippet}, William and {Todd}, Connor and {Toolan}, Sharon and {Tran}, Hien and {Trejo}, Edwin and {Truong}, Justin and {Tsukamoto}, Chris and {Tustain}, Samuel and {Tyra}, Harrison and {Ubeda}, Leonardo and {Underwood}, Kelli and {Uzzo}, Michael and {Van Campen}, Julie and {Vandal}, Thomas and {Vandenbussche}, Bart and {Vila}, Bego{\~n}a and {Volk}, Kevin and {Wahlgren}, Glenn and {Waldman}, Mark and {Walker}, Chanda and {Wander}, Michel and {Warfield}, Christine and {Warner}, Gerald and {Wasiak}, Matthew and {Watkins}, Mitchell and {Weaver}, Andrew and {Weilert}, Mark and {Weiser}, Nick and {Weiss}, Ben and {Weissman}, Sarah and {Welty}, Alan and {West}, Garrett and {Wheate}, Lauren and {Wheatley}, Elizabeth and {Wheeler}, Thomas and {White}, Rick and {Whiteaker}, Kevin and {Whitehouse}, Paul and {Whiteleather}, Jennifer and {Whitman}, William and {Williams}, Christina and {Willmer}, Christopher and {Willoughby}, Scott and {Wilson}, Andrew and {Wirth}, Gregory and {Wislowski}, Emily and {Wolf}, Erin and {Wolfe}, David and {Wolff}, Schuyler and {Workman}, Bill and {Wright}, Ray and {Wu}, Carl and {Wu}, Rai and {Wymer}, Kristen and {Yates}, Kayla and {Yeager}, Christopher and {Yeates}, Jared and {Yerger}, Ethan and {Yoon}, Jinmi and {Young}, Alice and {Yu}, Susan and {Zak}, Dean and {Zeidler}, Peter and {Zhou}, Julia and {Zielinski}, Thomas and {Zincke}, Cristian and {Zonak}, Stephanie},
        title = "{The Science Performance of JWST as Characterized in Commissioning}",
      journal = {\pasp},
     keywords = {Observatories, Infrared astronomy, Astronomical instrumentation, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = apr,
       volume = {135},
       number = {1046},
          eid = {048001},
        pages = {048001},
          doi = {10.1088/1538-3873/acb293},
archivePrefix = {arXiv},
       eprint = {2207.05632},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023PASP..135d8001R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boccaletti+2015,
       author = {{Boccaletti}, A. and {Lagage}, P. -O. and {Baudoz}, P. and {Beichman}, C. and {Bouchet}, P. and {Cavarroc}, C. and {Dubreuil}, D. and {Glasse}, Alistair and {Glauser}, A.~M. and {Hines}, D.~C. and {Lajoie}, C. -P. and {Lebreton}, J. and {Perrin}, M.~D. and {Pueyo}, L. and {Reess}, J.~M. and {Rieke}, G.~H. and {Ronayette}, S. and {Rouan}, D. and {Soummer}, R. and {Wright}, G.~S.},
        title = "{The Mid-Infrared Instrument for the James Webb Space Telescope, V: Predicted Performance of the MIRI Coronagraphs}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = jul,
       volume = {127},
       number = {953},
        pages = {633},
          doi = {10.1086/682256},
archivePrefix = {arXiv},
       eprint = {1508.02352},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PASP..127..633B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lafreniere+2009,
       author = {{Lafreni{\`e}re}, David and {Marois}, Christian and {Doyon}, Ren{\'e} and {Barman}, Travis},
        title = "{HST/NICMOS Detection of HR 8799 b in 1998}",
      journal = {\apjl},
     keywords = {planetary systems, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2009,
        month = apr,
       volume = {694},
       number = {2},
        pages = {L148-L152},
          doi = {10.1088/0004-637X/694/2/L148},
archivePrefix = {arXiv},
       eprint = {0902.3247},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...694L.148L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Soummer+2011,
       author = {{Soummer}, R{\'e}mi and {Hagan}, J. Brendan and {Pueyo}, Laurent and {Thormann}, Adrien and {Rajan}, Abhijith and {Marois}, Christian},
        title = "{Orbital Motion of HR 8799 b, c, d Using Hubble Space Telescope Data from 1998: Constraints on Inclination, Eccentricity, and Stability}",
      journal = {\apj},
     keywords = {planetary systems, stars: individual: HR 8799, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = nov,
       volume = {741},
       number = {1},
          eid = {55},
        pages = {55},
          doi = {10.1088/0004-637X/741/1/55},
archivePrefix = {arXiv},
       eprint = {1110.1382},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...741...55S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schneider+2014,
       author = {{Schneider}, Glenn and {Grady}, Carol A. and {Hines}, Dean C. and {Stark}, Christopher C. and {Debes}, John H. and {Carson}, Joe and {Kuchner}, Marc J. and {Perrin}, Marshall D. and {Weinberger}, Alycia J. and {Wisniewski}, John P. and {Silverstone}, Murray D. and {Jang-Condell}, Hannah and {Henning}, Thomas and {Woodgate}, Bruce E. and {Serabyn}, Eugene and {Moro-Martin}, Amaya and {Tamura}, Motohide and {Hinz}, Phillip M. and {Rodigas}, Timothy J.},
        title = "{Probing for Exoplanets Hiding in Dusty Debris Disks: Disk Imaging, Characterization, and Exploration with HST/STIS Multi-roll Coronagraphy}",
      journal = {\aj},
     keywords = {methods: observational, planet-disk interactions, stars: individual: HD 15115 HD 15745 HD 32297 HD 53143 HD 61005 HD 92945 HD 107146 HD 139664 HD 181327 Au Mic MP Mus, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = oct,
       volume = {148},
       number = {4},
          eid = {59},
        pages = {59},
          doi = {10.1088/0004-6256/148/4/59},
archivePrefix = {arXiv},
       eprint = {1406.7303},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....148...59S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hagan+2018,
       author = {{Hagan}, J. Brendan and {Choquet}, {\'E}lodie and {Soummer}, R{\'e}mi and {Vigan}, Arthur},
        title = "{ALICE Data Release: A Revaluation of HST-NICMOS Coronagraphic Images}",
      journal = {\aj},
     keywords = {catalogs, methods: data analysis, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = apr,
       volume = {155},
       number = {4},
          eid = {179},
        pages = {179},
          doi = {10.3847/1538-3881/aab14b},
archivePrefix = {arXiv},
       eprint = {1802.07754},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....155..179H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Lajoie+2016,
       author = {{Lajoie}, Charles-Philippe and {Soummer}, R{\'e}mi and {Pueyo}, Laurent and {Hines}, Dean C. and {Nelan}, Edmund P. and {Perrin}, Marshall and {Clampin}, Mark and {Isaacs}, John C.},
        title = "{Small-grid dithers for the JWST coronagraphs}",
    booktitle = {Space Telescopes and Instrumentation 2016: Optical, Infrared, and Millimeter Wave},
         year = 2016,
       editor = {{MacEwen}, Howard A. and {Fazio}, Giovanni G. and {Lystrup}, Makenzie and {Batalha}, Natalie and {Siegler}, Nicholas and {Tong}, Edward C.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9904},
        month = jul,
          eid = {99045K},
        pages = {99045K},
          doi = {10.1117/12.2233032},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9904E..5KL},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fabricius+2021,
       author = {{Fabricius}, C. and {Luri}, X. and {Arenou}, F. and {Babusiaux}, C. and {Helmi}, A. and {Muraveva}, T. and {Reyl{\'e}}, C. and {Spoto}, F. and {Vallenari}, A. and {Antoja}, T. and {Balbinot}, E. and {Barache}, C. and {Bauchet}, N. and {Bragaglia}, A. and {Busonero}, D. and {Cantat-Gaudin}, T. and {Carrasco}, J.~M. and {Diakit{\'e}}, S. and {Fabrizio}, M. and {Figueras}, F. and {Garcia-Gutierrez}, A. and {Garofalo}, A. and {Jordi}, C. and {Kervella}, P. and {Khanna}, S. and {Leclerc}, N. and {Licata}, E. and {Lambert}, S. and {Marrese}, P.~M. and {Masip}, A. and {Ramos}, P. and {Robichon}, N. and {Robin}, A.~C. and {Romero-G{\'o}mez}, M. and {Rubele}, S. and {Weiler}, M.},
        title = "{Gaia Early Data Release 3. Catalogue validation}",
      journal = {\aap},
     keywords = {catalogs, astrometry, techniques: photometric, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A5},
        pages = {A5},
          doi = {10.1051/0004-6361/202039834},
archivePrefix = {arXiv},
       eprint = {2012.06242},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A\&A...649A...5F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia-EDR3+2020-cat,
       author = {{Gaia Collaboration}},
        title = "{VizieR Online Data Catalog: Gaia EDR3 (Gaia Collaboration, 2020)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Gaia},
         year = 2020,
        month = nov,
          eid = {I/350},
        pages = {I/350},
          doi = {10.26093/cds/vizier.1350},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020yCat.1350....0G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rajan+2015,
       author = {{Rajan}, Abhijith and {Barman}, Travis and {Soummer}, R{\'e}mi and {Hagan}, J. Brendan and {Patience}, Jennifer and {Pueyo}, Laurent and {Choquet}, {\'E}lodie and {Konopacky}, Quinn and {Macintosh}, Bruce and {Marois}, Christian},
        title = "{Characterizing the Atmospheres of the HR8799 Planets with HST/WFC3}",
      journal = {\apjl},
     keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = aug,
       volume = {809},
       number = {2},
          eid = {L33},
        pages = {L33},
          doi = {10.1088/2041-8205/809/2/L33},
archivePrefix = {arXiv},
       eprint = {1508.02395},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...809L..33R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Schneider+2017,
       author = {{Schneider}, Glenn and {Gaspar}, Andras and {Debes}, John and {Gull}, Theodore and {Hines}, Dean and {Apai}, Daniel and {Rieke}, George},
        title = "{Enabling Narrow(est) IWA Coronagraphy with STIS BAR5 and BAR10 Occulters}",
     keywords = {Hubble Space Telescope, HST, Space Telescope Science Institute, STScI, Space Telescope Imaging Spectrograph, STIS, Astrophysics - Instrumentation and Methods for Astrophysics},
 howpublished = {Instrument Science Report STIS 2017-3, 35 pages},
         year = 2017,
        month = sep,
        pages = {3},
          doi = {10.48550/arXiv.1708.02643},
archivePrefix = {arXiv},
       eprint = {1708.02643},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017stis.rept....3S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@dataset{Best+2021,
  author       = {Best, William M. J. and
                  Dupuy, Trent J. and
                  Liu, Michael C. and
                  Siverd, Robert J. and
                  Zhang, Zhoujian},
  title        = {{The UltracoolSheet: Photometry, Astrometry, 
                   Spectroscopy, and Multiplicity for 3000+ Ultracool
                   Dwarfs and Imaged Exoplanets}},
  month        = mar,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {1.0.1},
  doi          = {10.5281/zenodo.4570814},
  url          = {https://doi.org/10.5281/zenodo.4570814}
}

@ARTICLE{Marois+2006,
   author = {{Marois}, C. and {Lafreni{\`e}re}, D. and {Doyon}, R. and {Macintosh}, B. and 
	{Nadeau}, D.},
    title = "{Angular Differential Imaging: A Powerful High-Contrast Imaging Technique}",
  journal = {\apj},
   eprint = {astro-ph/0512335},
 keywords = {Instrumentation: Adaptive Optics, Stars: Planetary Systems, Stars: Imaging},
     year = 2006,
    month = apr,
   volume = 641,
    pages = {556-564},
      doi = {10.1086/500401},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...641..556M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boccaletti+2023,
       author = {{Boccaletti}, A. and {M{\^a}lin}, M. and {Baudoz}, P. and {Tremplin}, P. and {Perrot}, C. and {Rouan}, D. and {-O.}, Lagage P. and {Whiteford}, N. and {Molli{\`e}re}, P. and {Waters}, R. and {Henning}, T. and {Decin}, L. and {G{\"u}del}, M. and {Vadenbussche}, B. and {Absil}, O. and {Argyriou}, I. and {Bouwman}, J. and {Cossou}, C. and {Coulais}, A. and {Gastaud}, R. and {Glasse}, A. and {Glauser}, A. and {Kamp}, I. and {Kendrew}, S. and {Krause}, O. and {Lahuis}, F. and {Mueller}, M. and {Olofsson}, G. and {Patapis}, P. and {Pye}, J. and {Royer}, P. and {Serabyn}, E. and {Scheithauer}, S. and {Colina}, L. and {van Dischoeck E.}, F. and {Ostlin}, G. and {T.}, Ray and {G}, Wright},
        title = "{Imaging detection of the inner dust belt and the four exoplanets in the HR8799 system with JWST's MIRI coronagraph}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = oct,
          eid = {arXiv:2310.13414},
        pages = {arXiv:2310.13414},
          doi = {10.48550/arXiv.2310.13414},
archivePrefix = {arXiv},
       eprint = {2310.13414},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv231013414B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2MASS+0,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TYCHO,
       author = {{H{\o}g}, E. and {Fabricius}, C. and {Makarov}, V.~V. and {Bastian}, U. and {Schwekendiek}, P. and {Wicenec}, A. and {Urban}, S. and {Corbin}, T. and {Wycoff}, G.},
        title = "{Construction and verification of the Tycho-2 Catalogue}",
      journal = {\aap},
     keywords = {ASTROMETRY, TECHNIQUES: PHOTOMETRIC, CATALOGS, METHODS: DATA ANALYSIS},
         year = 2000,
        month = may,
       volume = {357},
        pages = {367-386},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A\&A...357..367H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vizier-data,
       author = {{Ochsenbein}, F. and {Bauer}, P. and {Marcout}, J.},
        title = "{The VizieR database of astronomical catalogues}",
      journal = {\aaps},
     keywords = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, CATALOGS, Astrophysics},
         year = 2000,
        month = apr,
       volume = {143},
        pages = {23-32},
          doi = {10.1051/aas:2000169},
archivePrefix = {arXiv},
       eprint = {astro-ph/0002122},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A\&AS..143...23O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang-2023,
       author = {{Wang}, Ji},
        title = "{Spectral Retrieval with JWST Photometric data: a Case Study for HIP 65426 b}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanet atmospheric composition, 487, 2021},
         year = 2023,
        month = nov,
       volume = {166},
       number = {5},
          eid = {203},
        pages = {203},
          doi = {10.3847/1538-3881/acfca0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....166..203W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zhou+2022,
       author = {{Zhou}, Yifan and {Bowler}, Brendan P. and {Apai}, D{\'a}niel and {Kataria}, Tiffany and {Morley}, Caroline V. and {Bryan}, Marta L. and {Skemer}, Andrew J. and {Benneke}, Bj{\"o}rn},
        title = "{Roaring Storms in the Planetary-mass Companion VHS 1256-1257 b: Hubble Space Telescope Multiepoch Monitoring Reveals Vigorous Evolution in an Ultracool Atmosphere}",
      journal = {\aj},
     keywords = {Brown dwarfs, L dwarfs, Atmospheric variability, Planetary atmospheres, Spectroscopy, Time series analysis, Atmospheric circulation, Atmospheric clouds, 185, 894, 2119, 1244, 1558, 1916, 112, 2180, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = dec,
       volume = {164},
       number = {6},
          eid = {239},
        pages = {239},
          doi = {10.3847/1538-3881/ac9905},
archivePrefix = {arXiv},
       eprint = {2210.02464},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....164..239Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Best+2020,
       author = {{Best}, William M.~J. and {Liu}, Michael C. and {Magnier}, Eugene A. and {Dupuy}, Trent J.},
        title = "{The Hawaii Infrared Parallax Program. IV. A Comprehensive Parallax Survey of L0-T8 Dwarfs with UKIRT}",
      journal = {\aj},
     keywords = {Late-type dwarf stars, Parallax, Proper motions, Infrared photometry, Trigonometric parallax, L dwarfs, T dwarfs, 906, 1197, 1295, 792, 1713, 894, 1679, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = jun,
       volume = {159},
       number = {6},
          eid = {257},
        pages = {257},
          doi = {10.3847/1538-3881/ab84f4},
archivePrefix = {arXiv},
       eprint = {2010.15850},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159..257B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macintosh+2014,
       author = {{Macintosh}, Bruce and {Graham}, James R. and {Ingraham}, Patrick and {Konopacky}, Quinn and {Marois}, Christian and {Perrin}, Marshall and {Poyneer}, Lisa and {Bauman}, Brian and {Barman}, Travis and {Burrows}, Adam S. and {Cardwell}, Andrew and {Chilcote}, Jeffrey and {De Rosa}, Robert J. and {Dillon}, Daren and {Doyon}, Rene and {Dunn}, Jennifer and {Erikson}, Darren and {Fitzgerald}, Michael P. and {Gavel}, Donald and {Goodsell}, Stephen and {Hartung}, Markus and {Hibon}, Pascale and {Kalas}, Paul and {Larkin}, James and {Maire}, Jerome and {Marchis}, Franck and {Marley}, Mark S. and {McBride}, James and {Millar-Blanchaer}, Max and {Morzinski}, Katie and {Norton}, Andrew and {Oppenheimer}, B.~R. and {Palmer}, David and {Patience}, Jennifer and {Pueyo}, Laurent and {Rantakyro}, Fredrik and {Sadakuni}, Naru and {Saddlemyer}, Leslie and {Savransky}, Dmitry and {Serio}, Andrew and {Soummer}, Remi and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Thomas}, Sandrine and {Wallace}, J. Kent and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{First light of the Gemini Planet Imager}",
      journal = {Proceedings of the National Academy of Science},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = sep,
       volume = {111},
       number = {35},
        pages = {12661-12666},
          doi = {10.1073/pnas.1304215111},
archivePrefix = {arXiv},
       eprint = {1403.7520},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PNAS..11112661M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Otten+2017,
       author = {{Otten}, Gilles P.~P.~L. and {Snik}, Frans and {Kenworthy}, Matthew A. and {Keller}, Christoph U. and {Males}, Jared R. and {Morzinski}, Katie M. and {Close}, Laird M. and {Codona}, Johanan L. and {Hinz}, Philip M. and {Hornburg}, Kathryn J. and {Brickson}, Leandra L. and {Escuti}, Michael J.},
        title = "{On-sky Performance Analysis of the Vector Apodizing Phase Plate Coronagraph on MagAO/Clio2}",
      journal = {\apj},
     keywords = {infrared: planetary systems, instrumentation: high angular resolution, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = jan,
       volume = {834},
       number = {2},
          eid = {175},
        pages = {175},
          doi = {10.3847/1538-4357/834/2/175},
archivePrefix = {arXiv},
       eprint = {1702.04193},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834..175O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Close+2010,
       author = {{Close}, Laird M. and {Gasho}, Victor and {Kopon}, Derek and {Males}, Jared and {Follette}, Katherine B. and {Brutlag}, Kevin and {Uomoto}, Alan and {Hare}, Tyson},
        title = "{The Magellan Telescope Adaptive Secondary AO System: a visible and mid-IR AO facility}",
    booktitle = {Adaptive Optics Systems II},
         year = 2010,
       editor = {{Ellerbroek}, Brent L. and {Hart}, Michael and {Hubin}, Norbert and {Wizinowich}, Peter L.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7736},
        month = jul,
          eid = {773605},
        pages = {773605},
          doi = {10.1117/12.857924},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010SPIE.7736E..05C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Close+2013,
       author = {{Close}, L.~M. and {Males}, J.~R. and {Morzinski}, K. and {Kopon}, D. and {Follette}, K. and {Rodigas}, T.~J. and {Hinz}, P. and {Wu}, Y. -L. and {Puglisi}, A. and {Esposito}, S. and {Riccardi}, A. and {Pinna}, E. and {Xompero}, M. and {Briguglio}, R. and {Uomoto}, A. and {Hare}, T.},
        title = "{Diffraction-limited Visible Light Images of Orion Trapezium Cluster with the Magellan Adaptive Secondary Adaptive Optics System (MagAO)}",
      journal = {\apj},
     keywords = {binaries: general, brown dwarfs, instrumentation: adaptive optics, stars: evolution, stars: formation, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = sep,
       volume = {774},
       number = {2},
          eid = {94},
        pages = {94},
          doi = {10.1088/0004-637X/774/2/94},
archivePrefix = {arXiv},
       eprint = {1308.4155},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...774...94C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Sivanandam+2006,
       author = {{Sivanandam}, Suresh and {Hinz}, Phil M. and {Heinze}, Ari N. and {Freed}, Melanie and {Breuninger}, Andrew H.},
        title = "{Clio: a 3-5 micron AO planet-finding camera}",
     keywords = {Astrophysics},
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy},
         year = 2006,
       editor = {{McLean}, Ian S. and {Iye}, Masanori},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {6269},
        month = jun,
          eid = {62690U},
        pages = {62690U},
          doi = {10.1117/12.672344},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606131},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006SPIE.6269E..0US},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Morzinski+2014,
       author = {{Morzinski}, Katie M. and {Close}, Laird M. and {Males}, Jared R. and {Kopon}, Derek and {Hinz}, Phil M. and {Esposito}, Simone and {Riccardi}, Armando and {Puglisi}, Alfio and {Pinna}, Enrico and {Briguglio}, Runa and {Xompero}, Marco and {Quir{\'o}s-Pacheco}, Fernando and {Bailey}, Vanessa and {Follette}, Katherine B. and {Rodigas}, T.~J. and {Wu}, Ya-Lin and {Arcidiacono}, Carmelo and {Argomedo}, Javier and {Busoni}, Lorenzo and {Hare}, Tyson and {Uomoto}, Alan and {Weinberger}, Alycia},
        title = "{MagAO: Status and on-sky performance of the Magellan adaptive optics system}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Adaptive Optics Systems IV},
         year = 2014,
       editor = {{Marchetti}, Enrico and {Close}, Laird M. and {Vran}, Jean-Pierre},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9148},
        month = jul,
          eid = {914804},
        pages = {914804},
          doi = {10.1117/12.2057048},
archivePrefix = {arXiv},
       eprint = {1407.5098},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9148E..04M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WDSC,
       author = {{Mason}, Brian D. and {Wycoff}, Gary L. and {Hartkopf}, William I. and {Douglass}, Geoffrey G. and {Worley}, Charles E.},
        title = "{The 2001 US Naval Observatory Double Star CD-ROM. I. The Washington Double Star Catalog}",
      journal = {\aj},
     keywords = {Stars: Binaries: General, Stars: Binaries: Visual, Catalogs},
         year = 2001,
        month = dec,
       volume = {122},
       number = {6},
        pages = {3466-3471},
          doi = {10.1086/323920},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001AJ....122.3466M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Radigan+2014,
       author = {{Radigan}, Jacqueline and {Lafreni{\`e}re}, David and {Jayawardhana}, Ray and {Artigau}, Etienne},
        title = "{Strong Brightness Variations Signal Cloudy-to-clear Transition of Brown Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = oct,
       volume = {793},
       number = {2},
          eid = {75},
        pages = {75},
          doi = {10.1088/0004-637X/793/2/75},
archivePrefix = {arXiv},
       eprint = {1404.3247},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...793...75R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia-variables+2023,
       author = {{Lebzelter}, T. and {Mowlavi}, N. and {Lecoeur-Taibi}, I. and {Trabucchi}, M. and {Audard}, M. and {Garc{\'\i}a-Lario}, P. and {Gavras}, P. and {Holl}, B. and {Jevardat de Fombelle}, G. and {Nienartowicz}, K. and {Rimoldini}, L. and {Eyer}, L.},
        title = "{Gaia Data Release 3. The second Gaia catalogue of long-period variable candidates}",
      journal = {\aap},
     keywords = {stars: variables: general, stars: AGB and post-AGB, stars: carbon, galaxies: stellar content, catalogs, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jun,
       volume = {674},
          eid = {A15},
        pages = {A15},
          doi = {10.1051/0004-6361/202244241},
archivePrefix = {arXiv},
       eprint = {2206.05745},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A\&A...674A..15L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burggraaff+2018,
       author = {{Burggraaff}, O. and {Talens}, G.~J.~J. and {Spronck}, J. and {Lesage}, A. -L. and {Stuik}, R. and {Otten}, G.~P.~P.~L. and {Van Eylen}, V. and {Pollacco}, D. and {Snellen}, I.~A.~G.},
        title = "{Studying bright variable stars with the Multi-site All-Sky CAmeRA (MASCARA)}",
      journal = {\aap},
     keywords = {stars: variables: general, stars: variables: Cepheids, binaries: eclipsing, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = sep,
       volume = {617},
          eid = {A32},
        pages = {A32},
          doi = {10.1051/0004-6361/201833142},
archivePrefix = {arXiv},
       eprint = {1806.02247},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A\&A...617A..32B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@dataset{Cannon+Pickering-1993,
       author = {{Cannon}, A.~J. and {Pickering}, E.~C.},
        title = "{VizieR Online Data Catalog: Henry Draper Catalogue and Extension (Cannon+ 1918-1924; ADC 1989)}",
 howpublished = {VizieR On-line Data Catalog: III/135A.  Originally published in: Harv. Ann. 91-100 (1918-1924)},
         year = 1993,
        month = oct,
          eid = {III/135A},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993yCat.3135....0C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hinkley+2022,
       author = {{Hinkley}, Sasha and {Carter}, Aarynn L. and {Ray}, Shrishmoy and {Skemer}, Andrew and {Biller}, Beth and {Choquet}, Elodie and {Millar-Blanchaer}, Maxwell A. and {Sallum}, Stephanie and {Miles}, Brittany and {Whiteford}, Niall and {Patapis}, Polychronis and {Perrin}, Marshall and {Pueyo}, Laurent and {Schneider}, Glenn and {Stapelfeldt}, Karl and {Wang}, Jason and {Ward-Duong}, Kimberly and {Bowler}, Brendan P. and {Boccaletti}, Anthony and {Girard}, Julien H. and {Hines}, Dean and {Kalas}, Paul and {Kammerer}, Jens and {Kervella}, Pierre and {Leisenring}, Jarron and {Pantin}, Eric and {Zhou}, Yifan and {Meyer}, Michael and {Liu}, Michael C. and {Bonnefoy}, Mickael and {Currie}, Thayne and {McElwain}, Michael and {Metchev}, Stanimir and {Wyatt}, Mark and {Absil}, Olivier and {Adams}, Jea and {Barman}, Travis and {Baraffe}, Isabelle and {Bonavita}, Mariangela and {Booth}, Mark and {Bryan}, Marta and {Chauvin}, Gael and {Chen}, Christine and {Danielski}, Camilla and {De Furio}, Matthew and {Factor}, Samuel M. and {Fitzgerald}, Michael P. and {Fortney}, Jonathan J. and {Grady}, Carol and {Greenbaum}, Alexandra and {Henning}, Thomas and {Hoch}, Kielan K.~W. and {Janson}, Markus and {Kennedy}, Grant and {Kenworthy}, Matthew and {Kraus}, Adam and {Kuzuhara}, Masayuki and {Lagage}, Pierre-Olivier and {Lagrange}, Anne-Marie and {Launhardt}, Ralf and {Lazzoni}, Cecilia and {Lloyd}, James and {Marino}, Sebastian and {Marley}, Mark and {Martinez}, Raquel and {Marois}, Christian and {Matthews}, Brenda and {Matthews}, Elisabeth C. and {Mawet}, Dimitri and {Mazoyer}, Johan and {Phillips}, Mark and {Petrus}, Simon and {Quanz}, Sascha P. and {Quirrenbach}, Andreas and {Rameau}, Julien and {Rebollido}, Isabel and {Rickman}, Emily and {Samland}, Matthias and {Sargent}, B. and {Schlieder}, Joshua E. and {Sivaramakrishnan}, Anand and {Stone}, Jordan M. and {Tamura}, Motohide and {Tremblin}, Pascal and {Uyama}, Taichi and {Vasist}, Malavika and {Vigan}, Arthur and {Wagner}, Kevin and {Ygouf}, Marie},
        title = "{The JWST Early Release Science Program for the Direct Imaging and Spectroscopy of Exoplanetary Systems}",
      journal = {\pasp},
     keywords = {Coronagraphic imaging, Direct imaging, Exoplanet detection methods, Space telescopes, Exoplanet atmospheres, 313, 387, 489, 1547, 487, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = sep,
       volume = {134},
       number = {1039},
          eid = {095003},
        pages = {095003},
          doi = {10.1088/1538-3873/ac77bd},
archivePrefix = {arXiv},
       eprint = {2205.12972},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022PASP..134i5003H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ressler+2015,
       author = {{Ressler}, M.~E. and {Sukhatme}, K.~G. and {Franklin}, B.~R. and {Mahoney}, J.~C. and {Thelen}, M.~P. and {Bouchet}, P. and {Colbert}, J.~W. and {Cracraft}, Misty and {Dicken}, D. and {Gastaud}, R. and {Goodson}, G.~B. and {Eccleston}, Paul and {Moreau}, V. and {Rieke}, G.~H. and {Schneider}, Analyn},
        title = "{The Mid-Infrared Instrument for the James Webb Space Telescope, VIII: The MIRI Focal Plane System}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = jul,
       volume = {127},
       number = {953},
        pages = {675},
          doi = {10.1086/682258},
archivePrefix = {arXiv},
       eprint = {1508.02417},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PASP..127..675R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Anderson+Gordon-2011,
       author = {{Anderson}, Rachel E. and {Gordon}, Karl D.},
        title = "{Optimal Cosmic-Ray Detection for Nondestructive Read Ramps}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = oct,
       volume = {123},
       number = {908},
        pages = {1237},
          doi = {10.1086/662593},
archivePrefix = {arXiv},
       eprint = {1109.2626},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011PASP..123.1237A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

##################
# photom
@ARTICLE{Garrison+Gray-1994,
       author = {{Garrison}, R.~F. and {Gray}, R.~O.},
        title = "{The Late B-Type Stars: Refined MK Classification, Confrontation With Stromgren Photometry, And The Effects of Rotation}",
      journal = {\aj},
     keywords = {B Stars, F Stars, Photometry, Spectrum Analysis, Helium Isotopes, Iue, Luminosity, Spectral Sensitivity, Astrophysics, STARS: FUNDAMENTAL PARAMETERS, STARS: PECULIAR},
         year = 1994,
        month = apr,
       volume = {107},
        pages = {1556},
          doi = {10.1086/116967},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994AJ....107.1556G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@dataset{Johnson-UBV,
       author = {{Ducati}, J.~R.},
        title = "{VizieR Online Data Catalog: Catalogue of Stellar Photometry in Johnson's 11-color system.}",
 howpublished = {CDS/ADC Collection of Electronic Catalogues, 2237, 0 (2002)},
         year = 2002,
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002yCat.2237....0D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@dataset{Mermilliod-1997,
       author = {{Mermilliod}, J.~C.},
        title = "{VizieR Online Data Catalog: Homogeneous Means in the UBV System (Mermilliod 1991)}",
 howpublished = {VizieR On-line Data Catalog: II/168.  Originally published in: Institut d'Astronomie, Universite de Lausanne (1991)},
         year = 1997,
        month = sep,
          eid = {II/168},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997yCat.2168....0M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@dataset{IEU,
       author = {{Nasa / Esa /}, Serc},
        title = "{VizieR Online Data Catalog: Final Merged Log of IUE Observations (NASA-ESA, 2000)}",
 howpublished = {VizieR On-line Data Catalog: VI/110.  Originally published in: IUE Newsletters (1978-2000)},
         year = 2004,
        month = mar,
          eid = {VI/110},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004yCat.6110....0N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Paunzen+2015P,
       author = {{Paunzen}, E.},
        title = "{A new catalogue of Str{\"o}mgren-Crawford uvby{\ensuremath{\beta}} photometry}",
      journal = {\aap},
     keywords = {catalogs, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = aug,
       volume = {580},
          eid = {A23},
        pages = {A23},
          doi = {10.1051/0004-6361/201526413},
archivePrefix = {arXiv},
       eprint = {1506.04568},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A\&A...580A..23P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{HIPPARCOS+0,
        title = "{The HIPPARCOS and TYCHO catalogues. Astrometric and photometric star catalogues derived from the ESA HIPPARCOS Space Astrometry Mission}",
     keywords = {SPACE ASTROMETRY, STAR CATALOGS, POSITIONS, ARTIFICIAL SATELLITES},
    booktitle = {ESA Special Publication},
         year = 1997,
       series = {ESA Special Publication},
       volume = {1200},
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ESASP1200.....E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TYCHO+0,
       author = {{H{\o}g}, E. and {Fabricius}, C. and {Makarov}, V.~V. and {Bastian}, U. and {Schwekendiek}, P. and {Wicenec}, A. and {Urban}, S. and {Corbin}, T. and {Wycoff}, G.},
        title = "{Construction and verification of the Tycho-2 Catalogue}",
      journal = {\aap},
     keywords = {ASTROMETRY, TECHNIQUES: PHOTOMETRIC, CATALOGS, METHODS: DATA ANALYSIS},
         year = 2000,
        month = may,
       volume = {357},
        pages = {367-386},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A\&A...357..367H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WISE,
       author = {{Wright}, Edward L. and {Eisenhardt}, Peter R.~M. and {Mainzer}, Amy K. and {Ressler}, Michael E. and {Cutri}, Roc M. and {Jarrett}, Thomas and {Kirkpatrick}, J. Davy and {Padgett}, Deborah and {McMillan}, Robert S. and {Skrutskie}, Michael and {Stanford}, S.~A. and {Cohen}, Martin and {Walker}, Russell G. and {Mather}, John C. and {Leisawitz}, David and {Gautier}, Thomas N., III and {McLean}, Ian and {Benford}, Dominic and {Lonsdale}, Carol J. and {Blain}, Andrew and {Mendez}, Bryan and {Irace}, William R. and {Duval}, Valerie and {Liu}, Fengchuan and {Royer}, Don and {Heinrichsen}, Ingolf and {Howard}, Joan and {Shannon}, Mark and {Kendall}, Martha and {Walsh}, Amy L. and {Larsen}, Mark and {Cardon}, Joel G. and {Schick}, Scott and {Schwalm}, Mark and {Abid}, Mohamed and {Fabinsky}, Beth and {Naes}, Larry and {Tsai}, Chao-Wei},
        title = "{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}",
      journal = {\aj},
     keywords = {infrared: general, space vehicles, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = dec,
       volume = {140},
       number = {6},
        pages = {1868-1881},
          doi = {10.1088/0004-6256/140/6/1868},
archivePrefix = {arXiv},
       eprint = {1008.0031},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....140.1868W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AKARI+0,
       author = {{Onaka}, T. and {Matsuhara}, H. and {Wada}, T. and {Fujishiro}, N. and {Fujiwara}, H. and {Ishigaki}, M. and {Ishihara}, D. and {Ita}, Y. and {Kataza}, H. and {Kim}, W. and {Matsumoto}, T. and {Murakami}, H. and {Ohyama}, Y. and {Oyabu}, S. and {Sakon}, I. and {Tanab{\'e}}, T. and {Takagi}, T. and {Uemizu}, K. and {Ueno}, M. and {Usui}, F. and {Watarai}, H. and {Cohen}, M. and {Enya}, K. and {Ootsubo}, T. and {Pearson}, C.~P. and {Takeyama}, N. and {Yamamuro}, T. and {Ikeda}, Y.},
        title = "{The Infrared Camera (IRC) for AKARI -- Design and Imaging Performance}",
      journal = {\pasj},
     keywords = {Astrophysics},
         year = 2007,
        month = oct,
       volume = {59},
        pages = {S401},
          doi = {10.1093/pasj/59.sp2.S401},
archivePrefix = {arXiv},
       eprint = {0705.4144},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S.401O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AKARI+1,
       author = {{Murakami}, Hiroshi and {Baba}, Hajime and {Barthel}, Peter and {Clements}, David L. and {Cohen}, Martin and {Doi}, Yasuo and {Enya}, Keigo and {Figueredo}, Elysandra and {Fujishiro}, Naofumi and {Fujiwara}, Hideaki and {Fujiwara}, Mikio and {Garcia-Lario}, Pedro and {Goto}, Tomotsugu and {Hasegawa}, Sunao and {Hibi}, Yasunori and {Hirao}, Takanori and {Hiromoto}, Norihisa and {Hong}, Seung Soo and {Imai}, Koji and {Ishigaki}, Miho and {Ishiguro}, Masateru and {Ishihara}, Daisuke and {Ita}, Yoshifusa and {Jeong}, Woong-Seob and {Jeong}, Kyung Sook and {Kaneda}, Hidehiro and {Kataza}, Hirokazu and {Kawada}, Mitsunobu and {Kawai}, Toshihide and {Kawamura}, Akiko and {Kessler}, Martin F. and {Kester}, Do and {Kii}, Tsuneo and {Kim}, Dong Chan and {Kim}, Woojung and {Kobayashi}, Hisato and {Koo}, Bon Chul and {Kwon}, Suk Minn and {Lee}, Hyung Mok and {Lorente}, Rosario and {Makiuti}, Sin'itirou and {Matsuhara}, Hideo and {Matsumoto}, Toshio and {Matsuo}, Hiroshi and {Matsuura}, Shuji and {M{\"U}ller}, Thomas G. and {Murakami}, Noriko and {Nagata}, Hirohisa and {Nakagawa}, Takao and {Naoi}, Takahiro and {Narita}, Masanao and {Noda}, Manabu and {Oh}, Sang Hoon and {Ohnishi}, Akira and {Ohyama}, Youichi and {Okada}, Yoko and {Okuda}, Haruyuki and {Oliver}, Sebastian and {Onaka}, Takashi and {Ootsubo}, Takafumi and {Oyabu}, Shinki and {Pak}, Soojong and {Park}, Yong-Sun and {Pearson}, Chris P. and {Rowan-Robinson}, Michael and {Saito}, Toshinobu and {Sakon}, Itsuki and {Salama}, Alberto and {Sato}, Shinji and {Savage}, Richard S. and {Serjeant}, Stephen and {Shibai}, Hiroshi and {Shirahata}, Mai and {Sohn}, Jungjoo and {Suzuki}, Toyoaki and {Takagi}, Toshinobu and {Takahashi}, Hidenori and {Tanab{\'E}}, Toshihiko and {Takeuchi}, Tsutomu T. and {Takita}, Satoshi and {Thomson}, Matthew and {Uemizu}, Kazunori and {Ueno}, Munetaka and {Usui}, Fumihiko and {Verdugo}, Eva and {Wada}, Takehiko and {Wang}, Lingyu and {Watabe}, Toyoki and {Watarai}, Hidenori and {White}, Glenn J. and {Yamamura}, Issei and {Yamauchi}, Chisato and {Yasuda}, Akiko},
        title = "{The Infrared Astronomical Mission AKARI*}",
      journal = {\pasj},
     keywords = {Astrophysics},
         year = 2007,
        month = oct,
       volume = {59},
        pages = {S369-S376},
          doi = {10.1093/pasj/59.sp2.S369},
archivePrefix = {arXiv},
       eprint = {0708.1796},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASJ...59S.369M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AKARI+2,
       author = {{Ishihara}, D. and {Onaka}, T. and {Kataza}, H. and {Salama}, A. and {Alfageme}, C. and {Cassatella}, A. and {Cox}, N. and {Garc{\'\i}a-Lario}, P. and {Stephenson}, C. and {Cohen}, M. and {Fujishiro}, N. and {Fujiwara}, H. and {Hasegawa}, S. and {Ita}, Y. and {Kim}, W. and {Matsuhara}, H. and {Murakami}, H. and {M{\"u}ller}, T.~G. and {Nakagawa}, T. and {Ohyama}, Y. and {Oyabu}, S. and {Pyo}, J. and {Sakon}, I. and {Shibai}, H. and {Takita}, S. and {Tanab{\'e}}, T. and {Uemizu}, K. and {Ueno}, M. and {Usui}, F. and {Wada}, T. and {Watarai}, H. and {Yamamura}, I. and {Yamauchi}, C.},
        title = "{The AKARI/IRC mid-infrared all-sky survey}",
      journal = {\aap},
     keywords = {infrared: general, techniques: image processing, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {514},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/200913811},
archivePrefix = {arXiv},
       eprint = {1003.0270},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A\&A...514A...1I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@PROCEEDINGS{IRAS+0,
        title = "{Infrared Astronomical Satellite (IRAS) Catalogs and Atlases.Volume 1: Explanatory Supplement.}",
     keywords = {All Sky Photography, Catalogs, Indexes (Documentation), Infrared Astronomy Satellite, Cosmology, Galaxies, Star Formation, Stellar Evolution, Astrophysics},
    booktitle = {Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 1: Explanatory supplement},
         year = 1988,
       editor = {{Beichman}, C.~A. and {Neugebauer}, G. and {Habing}, H.~J. and {Clegg}, P.~E. and {Chester}, Thomas J.},
       volume = {1},
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988iras....1.....B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{IRAS+1,
        title = "{Infrared Astronomical Satellite (IRAS) Catalogs and Atlases.Volume 7: The Small Scale Structure Catalog.}",
     keywords = {All Sky Photography, Catalogs, Cosmology, Infrared Astronomy Satellite, Stars, Galaxies, Interstellar Matter, Point Sources, Star Formation, Astrophysics, ALL SKY PHOTOGRAPHY, CATALOGS, COSMOLOGY, INFRARED ASTRONOMY SATELLITE, STARS, GALAXIES, INTERSTELLAR MATTER, POINT SOURCES, STAR FORMATION},
    booktitle = {Infrared astronomical satellite (IRAS) catalogs and atlases. Volume 7},
         year = 1988,
       editor = {{Helou}, George and {Walker}, D.~W.},
       volume = {7},
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988iras....7.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



###################

@ARTICLE{Jones+2016,
       author = {{Jones}, Jeremy and {White}, R.~J. and {Quinn}, S. and {Ireland}, M. and {Boyajian}, T. and {Schaefer}, G. and {Baines}, E.~K.},
        title = "{The Age of the Directly Imaged Planet Host Star {\ensuremath{\kappa}} Andromedae Determined from Interferometric Observations}",
      journal = {\apjl},
     keywords = {planetary systems, stars: early-type, stars: evolution, stars: individual: kappa Andromedae, stars: rotation, techniques: interferometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = may,
       volume = {822},
       number = {1},
          eid = {L3},
        pages = {L3},
          doi = {10.3847/2041-8205/822/1/L3},
archivePrefix = {arXiv},
       eprint = {1604.02176},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...822L...3J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Currie+2018,
       author = {{Currie}, Thayne and {Brandt}, Timothy D. and {Uyama}, Taichi and {Nielsen}, Eric L. and {Blunt}, Sarah and {Guyon}, Olivier and {Tamura}, Motohide and {Marois}, Christian and {Mede}, Kyle and {Kuzuhara}, Masayuki and {Groff}, Tyler D. and {Jovanovic}, Nemanja and {Kasdin}, N. Jeremy and {Lozi}, Julien and {Hodapp}, Klaus and {Chilcote}, Jeffrey and {Carson}, Joseph and {Martinache}, Frantz and {Goebel}, Sean and {Grady}, Carol and {McElwain}, Michael and {Akiyama}, Eiji and {Asensio-Torres}, Ruben and {Hayashi}, Masa and {Janson}, Markus and {Knapp}, Gillian R. and {Kwon}, Jungmi and {Nishikawa}, Jun and {Oh}, Daehyeon and {Schlieder}, Joshua and {Serabyn}, Eugene and {Sitko}, Michael and {Skaf}, Nour},
        title = "{SCExAO/CHARIS Near-infrared Direct Imaging, Spectroscopy, and Forward-Modeling of {\ensuremath{\kappa}} And b: A Likely Young, Low-gravity Superjovian Companion}",
      journal = {\aj},
     keywords = {planetary systems, stars: early-type, stars: individual:: HD 222439, techniques: high angular resolution, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = dec,
       volume = {156},
       number = {6},
          eid = {291},
        pages = {291},
          doi = {10.3847/1538-3881/aae9ea},
archivePrefix = {arXiv},
       eprint = {1810.09457},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..291C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonnefoy+2014,
       author = {{Bonnefoy}, M. and {Currie}, T. and {Marleau}, G. -D. and {Schlieder}, J.~E. and {Wisniewski}, J. and {Carson}, J. and {Covey}, K.~R. and {Henning}, T. and {Biller}, B. and {Hinz}, P. and {Klahr}, H. and {Marsh Boyer}, A.~N. and {Zimmerman}, N. and {Janson}, M. and {McElwain}, M. and {Mordasini}, C. and {Skemer}, A. and {Bailey}, V. and {Defr{\`e}re}, D. and {Thalmann}, C. and {Skrutskie}, M. and {Allard}, F. and {Homeier}, D. and {Tamura}, M. and {Feldt}, M. and {Cumming}, A. and {Grady}, C. and {Brandner}, W. and {Helling}, C. and {Witte}, S. and {Hauschildt}, P. and {Kandori}, R. and {Kuzuhara}, M. and {Fukagawa}, M. and {Kwon}, J. and {Kudo}, T. and {Hashimoto}, J. and {Kusakabe}, N. and {Abe}, L. and {Brandt}, T. and {Egner}, S. and {Guyon}, O. and {Hayano}, Y. and {Hayashi}, M. and {Hayashi}, S. and {Hodapp}, K. and {Ishii}, M. and {Iye}, M. and {Knapp}, G. and {Matsuo}, T. and {Mede}, K. and {Miyama}, M. and {Morino}, J. -I. and {Moro-Martin}, A. and {Nishimura}, T. and {Pyo}, T. and {Serabyn}, E. and {Suenaga}, T. and {Suto}, H. and {Suzuki}, R. and {Takahashi} and {Takami}, M. and {Takato}, N. and {Terada}, H. and {Tomono}, D. and {Turner}, E. and {Watanabe}, M. and {Yamada}, T. and {Takami}, H. and {Usuda}, T.},
        title = "{Characterization of the gaseous companion {\ensuremath{\kappa}} Andromedae b. New Keck and LBTI high-contrast observations}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, techniques: photometric, planetary systems, stars: individual: kappa Andromedae, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {562},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/201322119},
archivePrefix = {arXiv},
       eprint = {1308.3859},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A\&A...562A.111B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Carson+2013,
       author = {{Carson}, J. and {Thalmann}, C. and {Janson}, M. and {Kozakis}, T. and {Bonnefoy}, M. and {Biller}, B. and {Schlieder}, J. and {Currie}, T. and {McElwain}, M. and {Goto}, M. and {Henning}, T. and {Brandner}, W. and {Feldt}, M. and {Kandori}, R. and {Kuzuhara}, M. and {Stevens}, L. and {Wong}, P. and {Gainey}, K. and {Fukagawa}, M. and {Kuwada}, Y. and {Brandt}, T. and {Kwon}, J. and {Abe}, L. and {Egner}, S. and {Grady}, C. and {Guyon}, O. and {Hashimoto}, J. and {Hayano}, Y. and {Hayashi}, M. and {Hayashi}, S. and {Hodapp}, K. and {Ishii}, M. and {Iye}, M. and {Knapp}, G. and {Kudo}, T. and {Kusakabe}, N. and {Matsuo}, T. and {Miyama}, S. and {Morino}, J. and {Moro-Martin}, A. and {Nishimura}, T. and {Pyo}, T. and {Serabyn}, E. and {Suto}, H. and {Suzuki}, R. and {Takami}, M. and {Takato}, N. and {Terada}, H. and {Tomono}, D. and {Turner}, E. and {Watanabe}, M. and {Wisniewski}, J. and {Yamada}, T. and {Takami}, H. and {Usuda}, T. and {Tamura}, M.},
        title = "{Direct Imaging Discovery of a ``Super-Jupiter'' around the Late B-type Star  {\ensuremath{\kappa}}  And}",
      journal = {\apjl},
     keywords = {brown dwarfs, planets and satellites: detection, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = feb,
       volume = {763},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.1088/2041-8205/763/2/L32},
archivePrefix = {arXiv},
       eprint = {1211.3744},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...763L..32C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hinkley+2013,
       author = {{Hinkley}, Sasha and {Pueyo}, Laurent and {Faherty}, Jacqueline K. and {Oppenheimer}, Ben R. and {Mamajek}, Eric E. and {Kraus}, Adam L. and {Rice}, Emily L. and {Ireland}, Michael J. and {David}, Trevor and {Hillenbrand}, Lynne A. and {Vasisht}, Gautam and {Cady}, Eric and {Brenner}, Douglas and {Veicht}, Aaron and {Nilsson}, Ricky and {Zimmerman}, Neil and {Parry}, Ian R. and {Beichman}, Charles and {Dekany}, Richard and {Roberts}, Jennifer E. and {Roberts}, Lewis C., Jr. and {Baranec}, Christoph and {Crepp}, Justin R. and {Burruss}, Rick and {Wallace}, J. Kent and {King}, David and {Zhai}, Chengxing and {Lockhart}, Thomas and {Shao}, Michael and {Soummer}, R{\'e}mi and {Sivaramakrishnan}, Anand and {Wilson}, Louis A.},
        title = "{The {\ensuremath{\kappa}} Andromedae System: New Constraints on the Companion Mass, System Age, and Further Multiplicity}",
      journal = {\apj},
     keywords = {instrumentation: adaptive optics, instrumentation: interferometers, planetary systems, planets and satellites: detection, stars: individual: {\ensuremath{\kappa}} Andromedae, techniques: high angular resolution, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = dec,
       volume = {779},
       number = {2},
          eid = {153},
        pages = {153},
          doi = {10.1088/0004-637X/779/2/153},
archivePrefix = {arXiv},
       eprint = {1309.3372},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...779..153H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kuhn+2018,
       author = {{K{\"u}hn}, J. and {Serabyn}, E. and {Lozi}, J. and {Jovanovic}, N. and {Currie}, T. and {Guyon}, O. and {Kudo}, T. and {Martinache}, F. and {Liewer}, K. and {Singh}, G. and {Tamura}, M. and {Mawet}, D. and {Hagelberg}, J. and {Defrere}, D.},
        title = "{An H-band Vector Vortex Coronagraph for the Subaru Coronagraphic Extreme-adaptive Optics System}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Instrumentation and Detectors},
         year = 2018,
        month = mar,
       volume = {130},
       number = {985},
        pages = {035001},
          doi = {10.1088/1538-3873/aa9fe5},
archivePrefix = {arXiv},
       eprint = {1712.02040},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PASP..130c5001K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoch+2020,
       author = {{Wilcomb}, Kielan K. and {Konopacky}, Quinn M. and {Barman}, Travis S. and {Theissen}, Christopher A. and {Ruffio}, Jean-Baptiste and {Brock}, Laci and {Macintosh}, Bruce and {Marois}, Christian},
        title = "{Moderate-resolution K-band Spectroscopy of Substellar Companion {\ensuremath{\kappa}} Andromedae b}",
      journal = {\aj},
     keywords = {Direct imaging, Exoplanet atmospheres, High resolution spectroscopy, Exoplanet formation, Radial velocity, 387, 487, 2096, 492, 1332, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
       volume = {160},
       number = {5},
          eid = {207},
        pages = {207},
          doi = {10.3847/1538-3881/abb9b1},
archivePrefix = {arXiv},
       eprint = {2009.08959},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160..207W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stone+2020,
       author = {{Stone}, Jordan M. and {Barman}, Travis and {Skemer}, Andrew J. and {Briesemeister}, Zackery W. and {Brock}, Laci S. and {Hinz}, Philip M. and {Leisenring}, Jarron M. and {Woodward}, Charles E. and {Skrutskie}, Michael F. and {Spalding}, Eckhart},
        title = "{High-contrast Thermal Infrared Spectroscopy with ALES: The 3-4 {\ensuremath{\mu}}m Spectrum of {\ensuremath{\kappa}} Andromedae b}",
      journal = {\aj},
     keywords = {L dwarfs, Exoplanet astronomy, Atmospheric composition, 894, 486, 2120, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = dec,
       volume = {160},
       number = {6},
          eid = {262},
        pages = {262},
          doi = {10.3847/1538-3881/abbef3},
archivePrefix = {arXiv},
       eprint = {2010.02928},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160..262S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Uyama+2020,
       author = {{Uyama}, Taichi and {Currie}, Thayne and {Hori}, Yasunori and {De Rosa}, Robert J. and {Mede}, Kyle and {Brandt}, Timothy D. and {Kwon}, Jungmi and {Guyon}, Olivier and {Lozi}, Julien and {Jovanovic}, Nemanja and {Martinache}, Frantz and {Kudo}, Tomoyuki and {Tamura}, Motohide and {Kasdin}, N. Jeremy and {Groff}, Tyler and {Chilcote}, Jeffrey and {Hayashi}, Masahiko and {McElwain}, Michael W. and {Asensio-Torres}, Ruben and {Janson}, Markus and {Knapp}, Gillian R. and {Serabyn}, Eugene},
        title = "{Atmospheric Characterization and Further Orbital Modeling of {\ensuremath{\kappa}} Andromeda b}",
      journal = {\aj},
     keywords = {Exoplanet astronomy, Exoplanet evolution, Exoplanet atmospheres, Exoplanet formation, 486, 491, 487, 492, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = feb,
       volume = {159},
       number = {2},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-3881/ab5afa},
archivePrefix = {arXiv},
       eprint = {1911.09758},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159...40U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@software{ATLAS12,
       author = {{Kurucz}, Robert L.},
        title = "{ATLAS12: Opacity sampling model atmosphere program}",
 howpublished = {Astrophysics Source Code Library, record ascl:1303.024},
         year = 2013,
        month = mar,
          eid = {ascl:1303.024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ascl.soft03024K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{ATLAS12+code,
       author = {{Kurucz}, Robert L.},
        title = "{Model Atmosphere Codes: ATLAS12 and ATLAS9}",
    booktitle = {Determination of Atmospheric Parameters of B},
         year = 2014,
       editor = {{Niemczura}, Ewa and {Smalley}, Barry and {Pych}, Wojtek},
        pages = {39-51},
          doi = {10.1007/978-3-319-06956-2\_4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014dapb.book...39K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Hodapp+2008,
       author = {{Hodapp}, Klaus W. and {Suzuki}, Ryuji and {Tamura}, Motohide and {Abe}, Lyu and {Suto}, Hiroshi and {Kandori}, Ryo and {Morino}, Junichi and {Nishimura}, Tetsuo and {Takami}, Hideki and {Guyon}, Olivier and {Jacobson}, Shane and {Stahlberger}, Vern and {Yamada}, Hubert and {Shelton}, Richard and {Hashimoto}, Jun and {Tavrov}, Alexander and {Nishikawa}, Jun and {Ukita}, Nobuharu and {Izumiura}, Hideyuki and {Hayashi}, Masahiko and {Nakajima}, Tadashi and {Yamada}, Toru and {Usuda}, Tomonori},
        title = "{HiCIAO: the Subaru Telescope's new high-contrast coronographic imager for adaptive optics}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy II},
         year = 2008,
       editor = {{McLean}, Ian S. and {Casali}, Mark M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7014},
        month = jul,
          eid = {701419},
        pages = {701419},
          doi = {10.1117/12.788088},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7014E..19H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Tokunaga+1998,
       author = {{Tokunaga}, Alan T. and {Kobayashi}, Naoto and {Bell}, James and {Ching}, Gregory K. and {Hodapp}, Klaus-Werner and {Hora}, Joseph L. and {Neill}, Doug and {Onaka}, Peter M. and {Rayner}, John T. and {Robertson}, Louis and {Warren}, David W. and {Weber}, Mark and {Young}, Tony T.},
        title = "{Infrared camera and spectrograph for the SUBARU Telescope}",
    booktitle = {Infrared Astronomical Instrumentation},
         year = 1998,
       editor = {{Fowler}, Albert M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {3354},
        month = aug,
        pages = {512-524},
          doi = {10.1117/12.317277},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998SPIE.3354..512T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hinkley+2011c,
       author = {{Hinkley}, Sasha and {Oppenheimer}, Ben R. and {Zimmerman}, Neil and {Brenner}, Douglas and {Parry}, Ian R. and {Crepp}, Justin R. and {Vasisht}, Gautam and {Ligon}, Edgar and {King}, David and {Soummer}, R{\'e}mi and {Sivaramakrishnan}, Anand and {Beichman}, Charles and {Shao}, Michael and {Roberts}, Lewis C., Jr. and {Bouchez}, Antonin and {Dekany}, Richard and {Pueyo}, Laurent and {Roberts}, Jennifer E. and {Lockhart}, Thomas and {Zhai}, Chengxing and {Shelton}, Chris and {Burruss}, Rick},
        title = "{A New High Contrast Imaging Program at Palomar Observatory}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {123},
       number = {899},
        pages = {74},
          doi = {10.1086/658163},
archivePrefix = {arXiv},
       eprint = {1012.0008},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011PASP..123...74H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Oppenheimer+2012,
       author = {{Oppenheimer}, Ben R. and {Beichman}, Charles and {Brenner}, Douglas and {Burruss}, Rick and {Cady}, Eric and {Crepp}, Justin and {Hillenbrand}, Lynne and {Hinkley}, Sasha and {Ligon}, E.~R. and {Lockhart}, Thomas and {Parry}, Ian and {Pueyo}, Laurent and {Rice}, Emily and {Roberts}, Lewis C. and {Roberts}, Jennifer and {Shao}, Michael and {Sivaramakrishnan}, Anand and {Soummer}, R{\'e}mi and {Vasisht}, Gautam and {Vescelus}, Fred and {Wallace}, J. Kent and {Zhai}, Chengxing and {Zimmerman}, Neil},
        title = "{Project 1640: the world's first ExAO coronagraphic hyperspectral imager for comparative planetary science}",
    booktitle = {Adaptive Optics Systems III},
         year = 2012,
       editor = {{Ellerbroek}, Brent L. and {Marchetti}, Enrico and {V{\'e}ran}, Jean-Pierre},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {8447},
        month = jul,
          eid = {844720},
        pages = {844720},
          doi = {10.1117/12.926419},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SPIE.8447E..20O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Hinkley+2008,
       author = {{Hinkley}, Sasha and {Oppenheimer}, Ben R. and {Brenner}, Douglas and {Parry}, Ian R. and {Sivaramakrishnan}, Anand and {Soummer}, Remi and {King}, David},
        title = "{A new integral field spectrograph for exoplanetary science at Palomar}",
    booktitle = {Adaptive Optics Systems},
         year = 2008,
       editor = {{Hubin}, Norbert and {Max}, Claire E. and {Wizinowich}, Peter L.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7015},
        month = jul,
          eid = {701519},
        pages = {701519},
          doi = {10.1117/12.789557},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7015E..19H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pickles-1998,
       author = {{Pickles}, A.~J.},
        title = "{A Stellar Spectral Flux Library: 1150-25000 {\r{A}}}",
      journal = {\pasp},
     keywords = {ATLASES, STARS: GENERAL, GALAXIES: STELLAR CONTENT},
         year = 1998,
        month = jul,
       volume = {110},
       number = {749},
        pages = {863-878},
          doi = {10.1086/316197},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998PASP..110..863P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Clemens+2007,
       author = {{Clemens}, D.~P. and {Sarcia}, D. and {Grabau}, A. and {Tollestrup}, E.~V. and {Buie}, M.~W. and {Dunham}, E. and {Taylor}, B.},
        title = "{Mimir: A Near-Infrared Wide-Field Imager, Spectrometer and Polarimeter}",
      journal = {\pasp},
     keywords = {Astronomical Instrumentation},
         year = 2007,
        month = dec,
       volume = {119},
       number = {862},
        pages = {1385-1402},
          doi = {10.1086/524775},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007PASP..119.1385C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Peters+2012,
       author = {{Peters-Limbach}, Mary A. and {Groff}, Tyler and {Kasdin}, N. Jeremy and {McElwain}, Michael W. and {Galvin}, Michael and {Carr}, Michael A. and {Lupton}, Robert and {Gunn}, James E. and {Knapp}, Gillian and {Gong}, Qian and {Carlotti}, Alexis and {Brandt}, Timothy and {Janson}, Markus and {Guyon}, Olivier and {Martinache}, Frantz and {Hayashi}, Masahiko and {Takato}, Naruhisa},
        title = "{Conceptual design of the Coronagraphic High Angular Resolution Imaging Spectrograph (CHARIS) for the Subaru telescope}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy IV},
         year = 2012,
       editor = {{McLean}, Ian S. and {Ramsay}, Suzanne K. and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {8446},
        month = sep,
          eid = {84467U},
        pages = {84467U},
          doi = {10.1117/12.926381},
archivePrefix = {arXiv},
       eprint = {1208.3190},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SPIE.8446E..7UP},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Groff+2014,
       author = {{Groff}, Tyler D. and {Kasdin}, N.~J. and {Limbach}, Mary A. and {Galvin}, Michael and {Carr}, Michael A. and {Knapp}, Gillian and {Brandt}, Timothy and {Loomis}, Craig and {Jarosik}, Norm and {Mede}, Kyle and {McElwain}, Michael W. and {Janson}, Markus and {Guyon}, Olivier and {Jovanovic}, Nemanja and {Takato}, Naruhisa and {Martinache}, Frantz and {Hayashi}, Masahiko},
        title = "{Construction and status of the CHARIS high contrast imaging spectrograph}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
         year = 2014,
       editor = {{Ramsay}, Suzanne K. and {McLean}, Ian S. and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9147},
        month = jul,
          eid = {91471W},
        pages = {91471W},
          doi = {10.1117/12.2055769},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9147E..1WG},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Groff+2015,
       author = {{Groff}, Tyler D. and {Kasdin}, N. Jeremy and {Limbach}, Mary Anne and {Galvin}, Michael and {Carr}, Michael A. and {Knapp}, Gillian and {Brandt}, Timothy and {Loomis}, Craig and {Jarosik}, Norman and {Mede}, Kyle and {McElwain}, Michael W. and {Leviton}, Douglas B. and {Miller}, Kevin H. and {Quijada}, Manuel A. and {Guyon}, Olivier and {Jovanovic}, Nemanja and {Takato}, Naruhisa and {Hayashi}, Masahiko},
        title = "{The CHARIS IFS for high contrast imaging at Subaru}",
    booktitle = {Techniques and Instrumentation for Detection of Exoplanets VII},
         year = 2015,
       editor = {{Shaklan}, Stuart},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9605},
        month = sep,
          eid = {96051C},
        pages = {96051C},
          doi = {10.1117/12.2188465},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015SPIE.9605E..1CG},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Castelli+Kurucz-2003,
       author = {{Castelli}, F. and {Kurucz}, R.~L.},
        title = "{New Grids of ATLAS9 Model Atmospheres}",
     keywords = {Astrophysics},
    booktitle = {Modelling of Stellar Atmospheres},
         year = 2003,
       editor = {{Piskunov}, N. and {Weiss}, W.~W. and {Gray}, D.~F.},
       series = {IAU Symposium},
       volume = {210},
        month = jan,
        pages = {A20},
          doi = {10.48550/arXiv.astro-ph/0405087},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405087},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003IAUS..210P.A20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Larkin+2006,
       author = {{Larkin}, James and {Barczys}, Matthew and {Krabbe}, Alfred and {Adkins}, Sean and {Aliado}, Ted and {Amico}, Paola and {Brims}, George and {Campbell}, Randy and {Canfield}, John and {Gasaway}, Thomas and {Honey}, Allan and {Iserlohe}, Christof and {Johnson}, Chris and {Kress}, Evan and {LaFreniere}, David and {Magnone}, Ken and {Magnone}, Nick and {McElwain}, Michael and {Moon}, Juleen and {Quirrenbach}, Andreas and {Skulason}, Gunnar and {Song}, Inseok and {Spencer}, Michael and {Weiss}, Jason and {Wright}, Shelley},
        title = "{OSIRIS: A diffraction limited integral field spectrograph for Keck}",
      journal = {\nar},
         year = 2006,
        month = jun,
       volume = {50},
       number = {4-5},
        pages = {362-364},
          doi = {10.1016/j.newar.2006.02.005},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006NewAR..50..362L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt+1999,
       author = {{Hauschildt}, Peter H. and {Allard}, France and {Ferguson}, Jason and {Baron}, E. and {Alexander}, David R.},
        title = "{The NEXTGEN Model Atmosphere Grid. II. Spherically Symmetric Model Atmospheres for Giant Stars with Effective Temperatures between 3000 and 6800 K}",
      journal = {\apj},
     keywords = {RADIATIVE TRANSFER, STARS: ATMOSPHERES, STARS: LATE-TYPE, Radiative Transfer, Stars: Atmospheres, Stars: Late-Type, Astrophysics},
         year = 1999,
        month = nov,
       volume = {525},
       number = {2},
        pages = {871-880},
          doi = {10.1086/307954},
archivePrefix = {arXiv},
       eprint = {astro-ph/9907194},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...525..871H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boccaletti+2024,
       author = {{Boccaletti}, Anthony and {M{\^a}lin}, Mathilde and {Baudoz}, Pierre and {Tremblin}, Pascal and {Perrot}, Cl{\'e}ment and {Rouan}, Daniel and {Lagage}, Pierre-Olivier and {Whiteford}, Niall and {Molli{\`e}re}, Paul and {Waters}, Rens and {Henning}, Thomas and {Decin}, Leen and {G{\"u}del}, Manuel and {Vandenbussche}, Bart and {Absil}, Olivier and {Argyriou}, Ioannis and {Bouwman}, Jeroen and {Cossou}, Christophe and {Coulais}, Alain and {Gastaud}, Ren{\'e} and {Glasse}, Alistair and {Glauser}, Adrian M. and {Kamp}, Inga and {Kendrew}, Sarah and {Krause}, Oliver and {Lahuis}, Fred and {Mueller}, Michael and {Olofsson}, Goran and {Patapis}, Polychronis and {Pye}, John and {Royer}, Pierre and {Serabyn}, Eugene and {Scheithauer}, Silvia and {Colina}, Luis and {van Dishoeck}, Ewine F. and {Ostlin}, G{\"o}ran and {Ray}, Tom P. and {Wright}, Gillian},
        title = "{Imaging detection of the inner dust belt and the four exoplanets in the HR 8799 system with JWST's MIRI coronagraph}",
      journal = {\aap},
     keywords = {techniques: high angular resolution, techniques: image processing, planets and satellites: detection, stars: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = jun,
       volume = {686},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/202347912},
archivePrefix = {arXiv},
       eprint = {2310.13414},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A\&A...686A..33B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Godoy+2024,
       author = {{Godoy}, N. and {Choquet}, E. and {Serabyn}, E. and {Danielski}, C. and {Stolker}, T. and {Charnay}, B. and {Hinkley}, S. and {Lagage}, P.~O. and {Ressler}, M.~E. and {Tremblin}, P. and {Vigan}, A.},
        title = "{A new atmospheric characterization of the sub-stellar companion HR 2562 B with JWST/MIRI observations}",
      journal = {\aap},
     keywords = {instrumentation: high angular resolution, methods: data analysis, techniques: image processing, planets and satellites: atmospheres, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = sep,
       volume = {689},
          eid = {A185},
        pages = {A185},
          doi = {10.1051/0004-6361/202449951},
archivePrefix = {arXiv},
       eprint = {2409.04524},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A\&A...689A.185G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Todorov+2016,
       author = {{Todorov}, Kamen O. and {Line}, Michael R. and {Pineda}, Jaime E. and {Meyer}, Michael R. and {Quanz}, Sascha P. and {Hinkley}, Sasha and {Fortney}, Jonathan J.},
        title = "{The Water Abundance of the Directly Imaged Substellar Companion {\ensuremath{\kappa}} And b Retrieved from a Near Infrared Spectrum}",
      journal = {\apj},
     keywords = {methods: data analysis, planetary systems, planets and satellites: gaseous planets, planets and satellites: individual: {\ensuremath{\kappa}} And b, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = may,
       volume = {823},
       number = {1},
          eid = {14},
        pages = {14},
          doi = {10.3847/0004-637X/823/1/14},
archivePrefix = {arXiv},
       eprint = {1504.00217},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823...14T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morris+2024,
       author = {{Morris}, Evan C. and {Wang}, Jason J. and {Hsu}, Chih-Chun and {Ruffio}, Jean-Baptiste and {Xuan}, Jerry W. and {Delorme}, Jacques-Robert and {Hood}, Callie and {Bryan}, Marta L. and {Martin}, Emily C. and {Pezzato}, Jacklyn and {Mawet}, Dimitri and {Skemer}, Andrew and {Baker}, Ashley and {Bartos}, Randall and {Calvin}, Benjamin and {Cetre}, Sylvain and {Doppmann}, Greg and {Echeverri}, Daniel and {Finnerty}, Luke and {Fitzgerald}, Michael P. and {Jovanovic}, Nemanja and {Liberman}, Joshua and {Lopez}, Ronald and {Sappey}, Ben and {Schofield}, Tobias and {Wallace}, J. Kent and {Wang}, Ji},
        title = "{{\ensuremath{\kappa}} Andromedae b Is a Fast Rotator from KPIC High-resolution Spectroscopy}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanet formation, High angular resolution, High resolution spectroscopy, 487, 492, 2167, 2096, Astrophysics - Earth and Planetary Astrophysics},
         year = 2024,
        month = oct,
       volume = {168},
       number = {4},
          eid = {144},
        pages = {144},
          doi = {10.3847/1538-3881/ad4ecf},
archivePrefix = {arXiv},
       eprint = {2405.13125},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....168..144M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spiegel+Burrows-2012,
       author = {{Spiegel}, David S. and {Burrows}, Adam},
        title = "{Spectral and Photometric Diagnostics of Giant Planet Formation Scenarios}",
      journal = {\apj},
     keywords = {brown dwarfs, radiative transfer, stars: evolution, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = feb,
       volume = {745},
       number = {2},
          eid = {174},
        pages = {174},
          doi = {10.1088/0004-637X/745/2/174},
archivePrefix = {arXiv},
       eprint = {1108.5172},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...745..174S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowler-2016B,
       author = {{Bowler}, Brendan P.},
        title = "{Imaging Extrasolar Giant Planets}",
      journal = {\pasp},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {128},
       number = {968},
        pages = {102001},
          doi = {10.1088/1538-3873/128/968/102001},
archivePrefix = {arXiv},
       eprint = {1605.02731},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PASP..128j2001B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marleau+Cumming-2014,
       author = {{Marleau}, G. -D. and {Cumming}, A.},
        title = "{Constraining the initial entropy of directly detected exoplanets}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, planets and satellites: fundamental parameters, planets and satellites: gaseous planets, stars: individual: {\ensuremath{\beta}} Pictoris, stars: individual: 2MASSWJ 1207334-393254, stars: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = jan,
       volume = {437},
       number = {2},
        pages = {1378-1399},
          doi = {10.1093/mnras/stt1967},
archivePrefix = {arXiv},
       eprint = {1302.1517},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.437.1378M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oberg+2011,
       author = {{{\"O}berg}, Karin I. and {Murray-Clay}, Ruth and {Bergin}, Edwin A.},
        title = "{The Effects of Snowlines on C/O in Planetary Atmospheres}",
      journal = {\apjl},
     keywords = {astrochemistry, circumstellar matter, molecular processes, planetary systems, planet-disk interactions, planets and satellites: atmospheres, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = dec,
       volume = {743},
       number = {1},
          eid = {L16},
        pages = {L16},
          doi = {10.1088/2041-8205/743/1/L16},
archivePrefix = {arXiv},
       eprint = {1110.5567},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...743L..16O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fortney+2008,
       author = {{Fortney}, J.~J. and {Marley}, M.~S. and {Saumon}, D. and {Lodders}, K.},
        title = "{Synthetic Spectra and Colors of Young Giant Planet Atmospheres: Effects of Initial Conditions and Atmospheric Metallicity}",
      journal = {\apj},
     keywords = {planetary systems, planets and satellites: formation, radiative transfer, Astrophysics},
         year = 2008,
        month = aug,
       volume = {683},
       number = {2},
        pages = {1104-1116},
          doi = {10.1086/589942},
archivePrefix = {arXiv},
       eprint = {0805.1066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...683.1104F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows+2006,
       author = {{Burrows}, Adam and {Sudarsky}, David and {Hubeny}, Ivan},
        title = "{L and T Dwarf Models and the L to T Transition}",
      journal = {\apj},
     keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = apr,
       volume = {640},
       number = {2},
        pages = {1063-1077},
          doi = {10.1086/500293},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...640.1063B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon+Marley-2008,
       author = {{Saumon}, D. and {Marley}, Mark S.},
        title = "{The Evolution of L and T Dwarfs in Color-Magnitude Diagrams}",
      journal = {\apj},
     keywords = {stars: atmospheres, stars: evolution, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = dec,
       volume = {689},
       number = {2},
        pages = {1327-1344},
          doi = {10.1086/592734},
archivePrefix = {arXiv},
       eprint = {0808.2611},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...689.1327S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremblin+2016,
       author = {{Tremblin}, P. and {Amundsen}, D.~S. and {Chabrier}, G. and {Baraffe}, I. and {Drummond}, B. and {Hinkley}, S. and {Mourier}, P. and {Venot}, O.},
        title = "{Cloudless Atmospheres for L/T Dwarfs and Extrasolar Giant Planets}",
      journal = {\apjl},
     keywords = {brown dwarfs, methods: numerical, methods: observational, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {L19},
        pages = {L19},
          doi = {10.3847/2041-8205/817/2/L19},
archivePrefix = {arXiv},
       eprint = {1601.03652},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817L..19T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gratton+2024,
       author = {{Gratton}, R. and {Bonavita}, M. and {Mesa}, D. and {Zurlo}, A. and {Marino}, S. and {Desidera}, S. and {D'Orazi}, V. and {Rigliaco}, E. and {Squicciarini}, V. and {Nogueira}, P.~H.},
        title = "{Implications of the discovery of AF Lep b. The mass-luminosity relation for planets in the {\ensuremath{\beta}} Pic Moving Group and the L-T transition for young companions and free-floating planets}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, planets and satellites: formation, planets and satellites: fundamental parameters, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = apr,
       volume = {684},
          eid = {A69},
        pages = {A69},
          doi = {10.1051/0004-6361/202348012},
archivePrefix = {arXiv},
       eprint = {2402.09067},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A\&A...684A..69G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Nasedkin+2024,
       author = {{Nasedkin}, E. and {Molli{\`e}re}, P. and {Lacour}, S. and {Nowak}, M. and {Kreidberg}, L. and {Stolker}, T. and {Wang}, J.~J. and {Balmer}, W.~O. and {Kammerer}, J. and {Shangguan}, J. and {Abuter}, R. and {Amorim}, A. and {Asensio-Torres}, R. and {Benisty}, M. and {Berger}, J. -P. and {Beust}, H. and {Blunt}, S. and {Boccaletti}, A. and {Bonnefoy}, M. and {Bonnet}, H. and {Bordoni}, M.~S. and {Bourdarot}, G. and {Brandner}, W. and {Cantalloube}, F. and {Caselli}, P. and {Charnay}, B. and {Chauvin}, G. and {Chavez}, A. and {Choquet}, E. and {Christiaens}, V. and {Cl{\'e}net}, Y. and {Coud{\'e} Du Foresto}, V. and {Cridland}, A. and {Davies}, R. and {Dembet}, R. and {Dexter}, J. and {Drescher}, A. and {Duvert}, G. and {Eckart}, A. and {Eisenhauer}, F. and {F{\"o}rster Schreiber}, N.~M. and {Garcia}, P. and {Garcia Lopez}, R. and {Gendron}, E. and {Genzel}, R. and {Gillessen}, S. and {Girard}, J.~H. and {Grant}, S. and {Haubois}, X. and {Hei{\ss}el}, G. and {Henning}, Th. and {Hinkley}, S. and {Hippler}, S. and {Houll{\'e}}, M. and {Hubert}, Z. and {Jocou}, L. and {Keppler}, M. and {Kervella}, P. and {Kurtovic}, N.~T. and {Lagrange}, A. -M. and {Lapeyr{\`e}re}, V. and {Le Bouquin}, J. -B. and {Lutz}, D. and {Maire}, A. -L. and {Mang}, F. and {Marleau}, G. -D. and {M{\'e}rand}, A. and {Monnier}, J.~D. and {Mordasini}, C. and {Ott}, T. and {Otten}, G.~P.~P.~L. and {Paladini}, C. and {Paumard}, T. and {Perraut}, K. and {Perrin}, G. and {Pfuhl}, O. and {Pourr{\'e}}, N. and {Pueyo}, L. and {Ribeiro}, D.~C. and {Rickman}, E. and {Ruffio}, J.~B. and {Rustamkulov}, Z. and {Shimizu}, T. and {Sing}, D. and {Stadler}, J. and {Straub}, O. and {Straubmeier}, C. and {Sturm}, E. and {Tacconi}, L.~J. and {van Dishoeck}, E.~F. and {Vigan}, A. and {Vincent}, F. and {von Fellenberg}, S.~D. and {Widmann}, F. and {Winterhalder}, T.~O. and {Woillez}, J. and {Yazici}, {\c{S}}. and {Gravity Collaboration}},
        title = "{Four-of-a-kind? Comprehensive atmospheric characterisation of the HR 8799 planets with VLTI/GRAVITY}",
      journal = {\aap},
     keywords = {radiative transfer, instrumentation: interferometers, methods: observational, planets and satellites: atmospheres, planets and satellites: composition, Astrophysics - Earth and Planetary Astrophysics},
         year = 2024,
        month = jul,
       volume = {687},
          eid = {A298},
        pages = {A298},
          doi = {10.1051/0004-6361/202449328},
archivePrefix = {arXiv},
       eprint = {2404.03776},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A\&A...687A.298N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Xuan+2018,
       author = {{Xuan}, W. Jerry and {Mawet}, Dimitri and {Ngo}, Henry and {Ruane}, Garreth and {Bailey}, Vanessa P. and {Choquet}, {\'E}lodie and {Absil}, Olivier and {Alvarez}, Carlos and {Bryan}, Marta and {Cook}, Therese and {Femen{\'\i}a Castell{\'a}}, Bruno and {Gomez Gonzalez}, Carlos and {Huby}, Elsa and {Knutson}, Heather A. and {Matthews}, Keith and {Ragland}, Sam and {Serabyn}, Eugene and {Zawol}, Zo{\"e}},
        title = "{Characterizing the Performance of the NIRC2 Vortex Coronagraph at W. M. Keck Observatory}",
      journal = {\aj},
     keywords = {instrumentation: adaptive optics, planets and satellites: detection, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = oct,
       volume = {156},
       number = {4},
          eid = {156},
        pages = {156},
          doi = {10.3847/1538-3881/aadae6},
archivePrefix = {arXiv},
       eprint = {1808.05297},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..156X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Malin+2025,
       author = {{M{\^a}lin}, Mathilde and {Boccaletti}, Anthony and {Perrot}, Cl{\'e}ment and {Baudoz}, Pierre and {Rouan}, Daniel and {Lagage}, Pierre-Olivier and {Waters}, Rens and {G{\"u}del}, Manuel and {Henning}, Thomas and {Vandenbussche}, Bart and {Absil}, Olivier and {Barrado}, David and {Charnay}, Benjamin and {Choquet}, Elodie and {Cossou}, Christophe and {Danielski}, Camilla and {Decin}, Leen and {Glauser}, Adrian M. and {Pye}, John and {Olofsson}, Goran and {Glasse}, Alistair and {Patapis}, Polychronis and {Royer}, Pierre and {Scheithauer}, Silvia and {Serabyn}, Eugene and {Tremblin}, Pascal and {Whiteford}, Niall and {van Dishoeck}, Ewine F. and {Ostlin}, G{\"o}ran and {Ray}, Tom P. and {Wright}, Gillian},
        title = "{First unambiguous detection of ammonia in the atmosphere of a planetary mass companion with JWST/MIRI coronagraphs}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: observational, techniques: image processing, planets and satellites: atmospheres, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2025,
        month = jan,
       volume = {693},
          eid = {A315},
        pages = {A315},
          doi = {10.1051/0004-6361/202452695},
archivePrefix = {arXiv},
       eprint = {2501.00104},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025A\&A...693A.315M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Malin+2024,
       author = {{M{\^a}lin}, Mathilde and {Boccaletti}, Anthony and {Perrot}, Cl{\'e}ment and {Baudoz}, Pierre and {Rouan}, Daniel and {Lagage}, Pierre-Olivier and {Waters}, Rens and {G{\"u}del}, Manuel and {Henning}, Thomas and {Vandenbussche}, Bart and {Absil}, Olivier and {Barrado}, David and {Cossou}, Christophe and {Decin}, Leen and {Glauser}, Adrian M. and {Pye}, John and {Olofsson}, Goran and {Glasse}, Alistair and {Lahuis}, Fred and {Patapis}, Polychronis and {Royer}, Pierre and {Scheithauer}, Silvia and {Whiteford}, Niall and {Serabyn}, Eugene and {Choquet}, Elodie and {Colina}, Luis and {Ostlin}, G{\"o}ran and {Ray}, Tom P. and {Wright}, Gillian},
        title = "{Unveiling the HD 95086 system at mid-infrared wavelengths with JWST/MIRI}",
      journal = {\aap},
     keywords = {methods: observational, planets and satellites: atmospheres, infrared: planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2024,
        month = oct,
       volume = {690},
          eid = {A316},
        pages = {A316},
          doi = {10.1051/0004-6361/202450470},
archivePrefix = {arXiv},
       eprint = {2408.16843},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A\&A...690A.316M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Miles+2018,
       author = {{Miles}, Brittany E. and {Skemer}, Andrew J. and {Barman}, Travis S. and {Allers}, Katelyn N. and {Stone}, Jordan M.},
        title = "{Methane in Analogs of Young Directly Imaged Exoplanets}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: VHS J125601.92{\textendash}125723.9b, PSO J318.5338{\textendash}22.8603, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = dec,
       volume = {869},
       number = {1},
          eid = {18},
        pages = {18},
          doi = {10.3847/1538-4357/aae6cd},
archivePrefix = {arXiv},
       eprint = {1810.04684},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...869...18M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chauvin+2017,
       author = {{Chauvin}, G. and {Desidera}, S. and {Lagrange}, A. -M. and {Vigan}, A. and {Gratton}, R. and {Langlois}, M. and {Bonnefoy}, M. and {Beuzit}, J. -L. and {Feldt}, M. and {Mouillet}, D. and {Meyer}, M. and {Cheetham}, A. and {Biller}, B. and {Boccaletti}, A. and {D'Orazi}, V. and {Galicher}, R. and {Hagelberg}, J. and {Maire}, A. -L. and {Mesa}, D. and {Olofsson}, J. and {Samland}, M. and {Schmidt}, T.~O.~B. and {Sissa}, E. and {Bonavita}, M. and {Charnay}, B. and {Cudel}, M. and {Daemgen}, S. and {Delorme}, P. and {Janin-Potiron}, P. and {Janson}, M. and {Keppler}, M. and {Le Coroller}, H. and {Ligi}, R. and {Marleau}, G.~D. and {Messina}, S. and {Molli{\`e}re}, P. and {Mordasini}, C. and {M{\"u}ller}, A. and {Peretti}, S. and {Perrot}, C. and {Rodet}, L. and {Rouan}, D. and {Zurlo}, A. and {Dominik}, C. and {Henning}, T. and {Menard}, F. and {Schmid}, H. -M. and {Turatto}, M. and {Udry}, S. and {Vakili}, F. and {Abe}, L. and {Antichi}, J. and {Baruffolo}, A. and {Baudoz}, P. and {Baudrand}, J. and {Blanchard}, P. and {Bazzon}, A. and {Buey}, T. and {Carbillet}, M. and {Carle}, M. and {Charton}, J. and {Cascone}, E. and {Claudi}, R. and {Costille}, A. and {Deboulbe}, A. and {De Caprio}, V. and {Dohlen}, K. and {Fantinel}, D. and {Feautrier}, P. and {Fusco}, T. and {Gigan}, P. and {Giro}, E. and {Gisler}, D. and {Gluck}, L. and {Hubin}, N. and {Hugot}, E. and {Jaquet}, M. and {Kasper}, M. and {Madec}, F. and {Magnard}, Y. and {Martinez}, P. and {Maurel}, D. and {Le Mignant}, D. and {M{\"o}ller-Nilsson}, O. and {Llored}, M. and {Moulin}, T. and {Orign{\'e}}, A. and {Pavlov}, A. and {Perret}, D. and {Petit}, C. and {Pragt}, J. and {Puget}, P. and {Rabou}, P. and {Ramos}, J. and {Rigal}, R. and {Rochat}, S. and {Roelfsema}, R. and {Rousset}, G. and {Roux}, A. and {Salasnich}, B. and {Sauvage}, J. -F. and {Sevin}, A. and {Soenke}, C. and {Stadler}, E. and {Suarez}, M. and {Weber}, L. and {Wildi}, F. and {Antoniucci}, S. and {Augereau}, J. -C. and {Baudino}, J. -L. and {Brandner}, W. and {Engler}, N. and {Girard}, J. and {Gry}, C. and {Kral}, Q. and {Kopytova}, T. and {Lagadec}, E. and {Milli}, J. and {Moutou}, C. and {Schlieder}, J. and {Szul{\'a}gyi}, J. and {Thalmann}, C. and {Wahhaj}, Z.},
        title = "{Discovery of a warm, dusty giant planet around HIP 65426}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, instrumentation: high angular resolution, methods: observational, planets and satellites: atmospheres, planets and satellites: formation, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = sep,
       volume = {605},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201731152},
archivePrefix = {arXiv},
       eprint = {1707.01413},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A\&A...605L...9C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonatto-2019,
       author = {{Bonatto}, Charles},
        title = "{An efficient approach to extract parameters from star cluster CMDs: fitCMD}",
      journal = {\mnras},
     keywords = {open clusters and associations: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {483},
       number = {2},
        pages = {2758-2765},
          doi = {10.1093/mnras/sty3291},
archivePrefix = {arXiv},
       eprint = {1812.01650},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2758B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cheetham+2019,
       author = {{Cheetham}, A.~C. and {Samland}, M. and {Brems}, S.~S. and {Launhardt}, R. and {Chauvin}, G. and {S{\'e}gransan}, D. and {Henning}, T. and {Quirrenbach}, A. and {Avenhaus}, H. and {Cugno}, G. and {Girard}, J. and {Godoy}, N. and {Kennedy}, G.~M. and {Maire}, A. -L. and {Metchev}, S. and {M{\"u}ller}, A. and {Musso Barcucci}, A. and {Olofsson}, J. and {Pepe}, F. and {Quanz}, S.~P. and {Queloz}, D. and {Reffert}, S. and {Rickman}, E. and {van Boekel}, R. and {Boccaletti}, A. and {Bonnefoy}, M. and {Cantalloube}, F. and {Charnay}, B. and {Delorme}, P. and {Janson}, M. and {Keppler}, M. and {Lagrange}, A. -M. and {Langlois}, M. and {Lazzoni}, C. and {Menard}, F. and {Mesa}, D. and {Meyer}, M. and {Schmidt}, T. and {Sissa}, E. and {Udry}, S. and {Zurlo}, A.},
        title = "{Spectral and orbital characterisation of the directly imaged giant planet HIP 65426 b}",
      journal = {\aap},
     keywords = {stars: individual: HIP 65426, planets and satellites: atmospheres, techniques: high angular resolution, planets and satellites: detection, planetary systems, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A80},
        pages = {A80},
          doi = {10.1051/0004-6361/201834112},
archivePrefix = {arXiv},
       eprint = {1812.07198},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A\&A...622A..80C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Samland+2017,
       author = {{Samland}, M. and {Molli{\`e}re}, P. and {Bonnefoy}, M. and {Maire}, A. -L. and {Cantalloube}, F. and {Cheetham}, A.~C. and {Mesa}, D. and {Gratton}, R. and {Biller}, B.~A. and {Wahhaj}, Z. and {Bouwman}, J. and {Brandner}, W. and {Melnick}, D. and {Carson}, J. and {Janson}, M. and {Henning}, T. and {Homeier}, D. and {Mordasini}, C. and {Langlois}, M. and {Quanz}, S.~P. and {van Boekel}, R. and {Zurlo}, A. and {Schlieder}, J.~E. and {Avenhaus}, H. and {Beuzit}, J. -L. and {Boccaletti}, A. and {Bonavita}, M. and {Chauvin}, G. and {Claudi}, R. and {Cudel}, M. and {Desidera}, S. and {Feldt}, M. and {Fusco}, T. and {Galicher}, R. and {Kopytova}, T.~G. and {Lagrange}, A. -M. and {Le Coroller}, H. and {Martinez}, P. and {Moeller-Nilsson}, O. and {Mouillet}, D. and {Mugnier}, L.~M. and {Perrot}, C. and {Sevin}, A. and {Sissa}, E. and {Vigan}, A. and {Weber}, L.},
        title = "{Spectral and atmospheric characterization of 51 Eridani b using VLT/SPHERE}",
      journal = {\aap},
     keywords = {stars: individual: 51 Eridani, planets and satellites: atmospheres, methods: data analysis, techniques: high angular resolution, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201629767},
archivePrefix = {arXiv},
       eprint = {1704.02987},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A\&A...603A..57S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell+2015,
       author = {{Bell}, Cameron P.~M. and {Mamajek}, Eric E. and {Naylor}, Tim},
        title = "{A self-consistent, absolute isochronal age scale for young moving groups in the solar neighbourhood}",
      journal = {\mnras},
     keywords = {techniques: photometric, stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: pre-main-sequence, open clusters and associations: general, solar neighbourhood, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = nov,
       volume = {454},
       number = {1},
        pages = {593-614},
          doi = {10.1093/mnras/stv1981},
archivePrefix = {arXiv},
       eprint = {1508.05955},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.454..593B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zuckerman+2011,
       author = {{Zuckerman}, B. and {Rhee}, Joseph H. and {Song}, Inseok and {Bessell}, M.~S.},
        title = "{The Tucana/Horologium, Columba, AB Doradus, and Argus Associations: New Members and Dusty Debris Disks}",
      journal = {\apj},
     keywords = {circumstellar matter, stars: evolution, stars: kinematics and dynamics, stars: pre-main sequence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = may,
       volume = {732},
       number = {2},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/732/2/61},
archivePrefix = {arXiv},
       eprint = {1104.0284},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...732...61Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Burrows+1995,
       author = {{Burrows}, C.~J. and {Krist}, J.~E. and {Stapelfeldt}, K.~R. and {WFPC2 Investigation Definition Team}},
        title = "{HST Observations of the Beta Pictoris Circumstellar Disk}",
    booktitle = {American Astronomical Society Meeting Abstracts},
         year = 1995,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {187},
        month = dec,
          eid = {32.05},
        pages = {32.05},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995AAS...187.3205B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeRosa+2016,
       author = {{De Rosa}, Robert J. and {Rameau}, Julien and {Patience}, Jenny and {Graham}, James R. and {Doyon}, Ren{\'e} and {Lafreni{\`e}re}, David and {Macintosh}, Bruce and {Pueyo}, Laurent and {Rajan}, Abhijith and {Wang}, Jason J. and {Ward-Duong}, Kimberly and {Hung}, Li-Wei and {Maire}, J{\'e}r{\^o}me and {Nielsen}, Eric L. and {Ammons}, S. Mark and {Bulger}, Joanna and {Cardwell}, Andrew and {Chilcote}, Jeffrey K. and {Galvez}, Ramon L. and {Gerard}, Benjamin L. and {Goodsell}, Stephen and {Hartung}, Markus and {Hibon}, Pascale and {Ingraham}, Patrick and {Johnson-Groh}, Mara and {Kalas}, Paul and {Konopacky}, Quinn M. and {Marchis}, Franck and {Marois}, Christian and {Metchev}, Stanimir and {Morzinski}, Katie M. and {Oppenheimer}, Rebecca and {Perrin}, Marshall D. and {Rantakyr{\"o}}, Fredrik T. and {Savransky}, Dmitry and {Thomas}, Sandrine},
        title = "{Spectroscopic Characterization of HD 95086 b with the Gemini Planet Imager}",
      journal = {\apj},
     keywords = {infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, stars: individual: HD 95086, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.3847/0004-637X/824/2/121},
archivePrefix = {arXiv},
       eprint = {1604.01411},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824..121D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rajan+2017,
       author = {{Rajan}, Abhijith and {Rameau}, Julien and {De Rosa}, Robert J. and {Marley}, Mark S. and {Graham}, James R. and {Macintosh}, Bruce and {Marois}, Christian and {Morley}, Caroline and {Patience}, Jennifer and {Pueyo}, Laurent and {Saumon}, Didier and {Ward-Duong}, Kimberly and {Ammons}, S. Mark and {Arriaga}, Pauline and {Bailey}, Vanessa P. and {Barman}, Travis and {Bulger}, Joanna and {Burrows}, Adam S. and {Chilcote}, Jeffrey and {Cotten}, Tara and {Czekala}, Ian and {Doyon}, Rene and {Duch{\^e}ne}, Gaspard and {Esposito}, Thomas M. and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Fortney}, Jonathan J. and {Goodsell}, Stephen J. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Johnson-Groh}, Mara and {Kalas}, Paul and {Konopacky}, Quinn and {Lafreni{\`e}re}, David and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Morzinski}, Katie M. and {Nielsen}, Eric L. and {Oppenheimer}, Rebecca and {Palmer}, David and {Patel}, Rahul I. and {Perrin}, Marshall and {Poyneer}, Lisa and {Rantakyr{\"o}}, Fredrik T. and {Ruffio}, Jean-Baptiste and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, R{\'e}mi and {Thomas}, Sandrine and {Vasisht}, Gautam and {Wallace}, J. Kent and {Wang}, Jason J. and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{Characterizing 51 Eri b from 1 to 5 {\ensuremath{\mu}}m: A Partly Cloudy Exoplanet}",
      journal = {\aj},
     keywords = {instrumentation: adaptive optics, planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: gaseous planets, stars: individual: 51 Eridani, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jul,
       volume = {154},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/1538-3881/aa74db},
archivePrefix = {arXiv},
       eprint = {1705.03887},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154...10R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Couture+2023,
       author = {{Couture}, Dominic and {Gagn{\'e}}, Jonathan and {Doyon}, Ren{\'e}},
        title = "{Addressing Systematics in the Traceback Age of the {\ensuremath{\beta}} Pictoris Moving Group}",
      journal = {\apj},
     keywords = {Stellar kinematics, Stellar associations, Stellar ages, Radial velocity, Astrometry, 1608, 1582, 1581, 1332, 80, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = mar,
       volume = {946},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4357/acb4eb},
archivePrefix = {arXiv},
       eprint = {2302.04348},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...946....6C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard+2012,
       author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B.},
        title = "{Models of very-low-mass stars, brown dwarfs and exoplanets}",
      journal = {Philosophical Transactions of the Royal Society of London Series A},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jun,
       volume = {370},
       number = {1968},
        pages = {2765-2777},
          doi = {10.1098/rsta.2011.0269},
archivePrefix = {arXiv},
       eprint = {1112.3591},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012RSPTA.370.2765A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Helling+2008,
       author = {{Helling}, Christiane and {Dehn}, Matthias and {Woitke}, Peter and {Hauschildt}, Peter H.},
        title = "{Consistent Simulations of Substellar Atmospheres and Nonequilibrium Dust Cloud Formation}",
      journal = {\apjl},
     keywords = {astrochemistry, methods: numerical, stars: atmospheres, Astrophysics},
         year = 2008,
        month = mar,
       volume = {675},
       number = {2},
        pages = {L105},
          doi = {10.1086/533462},
archivePrefix = {arXiv},
       eprint = {0801.3733},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...675L.105H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon+2008,
       author = {{Saumon}, D. and {Marley}, Mark S.},
        title = "{The Evolution of L and T Dwarfs in Color-Magnitude Diagrams}",
      journal = {\apj},
     keywords = {stars: atmospheres, stars: evolution, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = dec,
       volume = {689},
       number = {2},
        pages = {1327-1344},
          doi = {10.1086/592734},
archivePrefix = {arXiv},
       eprint = {0808.2611},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...689.1327S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Karalidi+2021,
       author = {{Karalidi}, Theodora and {Marley}, Mark and {Fortney}, Jonathan J. and {Morley}, Caroline and {Saumon}, Didier and {Lupu}, Roxana and {Visscher}, Channon and {Freedman}, Richard},
        title = "{The Sonora Substellar Atmosphere Models. II. Cholla: A Grid of Cloud-free, Solar Metallicity Models in Chemical Disequilibrium for the JWST Era}",
      journal = {\apj},
     keywords = {185, 498, 2120, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = dec,
       volume = {923},
       number = {2},
          eid = {269},
        pages = {269},
          doi = {10.3847/1538-4357/ac3140},
archivePrefix = {arXiv},
       eprint = {2110.11824},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923..269K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley+2021-son,
       author = {{Marley}, Mark S. and {Saumon}, Didier and {Visscher}, Channon and {Lupu}, Roxana and {Freedman}, Richard and {Morley}, Caroline and {Fortney}, Jonathan J. and {Seay}, Christopher and {Smith}, Adam J.~R.~W. and {Teal}, D.~J. and {Wang}, Ruoyan},
        title = "{The Sonora Brown Dwarf Atmosphere and Evolution Models. I. Model Description and Application to Cloudless Atmospheres in Rainout Chemical Equilibrium}",
      journal = {\apj},
     keywords = {Brown dwarfs, T dwarfs, L dwarfs, L subdwarfs, T subdwarfs, Y dwarfs, Stellar atmospheres, 185, 1679, 894, 896, 1680, 1827, 1584, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {85},
        pages = {85},
          doi = {10.3847/1538-4357/ac141d},
archivePrefix = {arXiv},
       eprint = {2107.07434},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920...85M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{currie+2011,
       author = {{Currie}, Thayne and {Burrows}, Adam and {Itoh}, Yoichi and {Matsumura}, Soko and {Fukagawa}, Misato and {Apai}, Daniel and {Madhusudhan}, Nikku and {Hinz}, Philip M. and {Rodigas}, T.~J. and {Kasper}, Markus and {Pyo}, T. -S. and {Ogino}, Satoshi},
        title = "{A Combined Subaru/VLT/MMT 1-5 {\ensuremath{\mu}}m Study of Planets Orbiting HR 8799: Implications for Atmospheric Properties, Masses, and Formation}",
      journal = {\apj},
     keywords = {brown dwarfs, instrumentation: adaptive optics, planetary systems, stars: individual: HR 8799, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = mar,
       volume = {729},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.1088/0004-637X/729/2/128},
archivePrefix = {arXiv},
       eprint = {1101.1973},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729..128C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chabrier+2000,
       author = {{Chabrier}, G. and {Baraffe}, I. and {Allard}, F. and {Hauschildt}, P.},
        title = "{Evolutionary Models for Very Low-Mass Stars and Brown Dwarfs with Dusty Atmospheres}",
      journal = {\apj},
     keywords = {Hertzsprung-Russell, Stars: Evolution, Stars: Low-Mass, Brown Dwarfs, Stars: Luminosity Function, Mass Function, Astrophysics},
         year = 2000,
        month = oct,
       volume = {542},
       number = {1},
        pages = {464-472},
          doi = {10.1086/309513},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005557},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...542..464C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirkpatrick+1999,
       author = {{Kirkpatrick}, J. Davy and {Reid}, I. Neill and {Liebert}, James and {Cutri}, Roc M. and {Nelson}, Brant and {Beichman}, Charles A. and {Dahn}, Conard C. and {Monet}, David G. and {Gizis}, John E. and {Skrutskie}, Michael F.},
        title = "{Dwarfs Cooler than ``M``: The Definition of Spectral Type ``L'' Using Discoveries from the 2 Micron All-Sky Survey (2MASS)}",
      journal = {\apj},
     keywords = {INFRARED: STARS, STARS: ATMOSPHERES, STARS: DISTANCES, STARS: FUNDAMENTAL PARAMETERS, STARS: LOW-MASS, BROWN DWARFS, Infrared: Stars, Stars: Atmospheres, Stars: Distances, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs},
         year = 1999,
        month = jul,
       volume = {519},
       number = {2},
        pages = {802-833},
          doi = {10.1086/307414},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...519..802K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cushing+2008,
       author = {{Cushing}, Michael C. and {Marley}, Mark S. and {Saumon}, D. and {Kelly}, Brandon C. and {Vacca}, William D. and {Rayner}, John T. and {Freedman}, Richard S. and {Lodders}, Katharina and {Roellig}, Thomas L.},
        title = "{Atmospheric Parameters of Field L and T Dwarfs}",
      journal = {\apj},
     keywords = {infrared: stars, radiative transfer, stars: fundamental parameters, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = may,
       volume = {678},
       number = {2},
        pages = {1372-1395},
          doi = {10.1086/526489},
archivePrefix = {arXiv},
       eprint = {0711.0801},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...678.1372C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett+2010L,
       author = {{Leggett}, S.~K. and {Burningham}, Ben and {Saumon}, D. and {Marley}, M.~S. and {Warren}, S.~J. and {Smart}, R.~L. and {Jones}, H.~R.~A. and {Lucas}, P.~W. and {Pinfield}, D.~J. and {Tamura}, Motohide},
        title = "{Mid-Infrared Photometry of Cold Brown Dwarfs: Diversity in Age, Mass, and Metallicity}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {2},
        pages = {1627-1640},
          doi = {10.1088/0004-637X/710/2/1627},
archivePrefix = {arXiv},
       eprint = {1001.0762},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710.1627L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonnefoy+2013,
       author = {{Bonnefoy}, M. and {Boccaletti}, A. and {Lagrange}, A. -M. and {Allard}, F. and {Mordasini}, C. and {Beust}, H. and {Chauvin}, G. and {Girard}, J.~H.~V. and {Homeier}, D. and {Apai}, D. and {Lacour}, S. and {Rouan}, D.},
        title = "{The near-infrared spectral energy distribution of {\ensuremath{\beta}} Pictoris b}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, techniques: photometric, planetary systems, stars: individual:{\ensuremath{\beta}}Pic b, planets and satellites: atmospheres, planets and satellites: fundamental parameters, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jul,
       volume = {555},
          eid = {A107},
        pages = {A107},
          doi = {10.1051/0004-6361/201220838},
archivePrefix = {arXiv},
       eprint = {1302.1160},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A\&A...555A.107B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matthews+2024,
       author = {{Matthews}, E.~C. and {Carter}, A.~L. and {Pathak}, P. and {Morley}, C.~V. and {Phillips}, M.~W. and {P.~M.}, S. Krishanth and {Feng}, F. and {Bonse}, M.~J. and {Boogaard}, L.~A. and {Burt}, J.~A. and {Crossfield}, I.~J.~M. and {Douglas}, E.~S. and {Henning}, Th. and {Hom}, J. and {Ko}, C. -L. and {Kasper}, M. and {Lagrange}, A. -M. and {Petit dit de la Roche}, D. and {Philipot}, F.},
        title = "{A temperate super-Jupiter imaged with JWST in the mid-infrared}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2024,
        month = sep,
       volume = {633},
       number = {8031},
        pages = {789-792},
          doi = {10.1038/s41586-024-07837-8},
archivePrefix = {arXiv},
       eprint = {2503.01599},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024Natur.633..789M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kirkpatrick-2005,
       author = {{Kirkpatrick}, J. Davy},
        title = "{New Spectral Types L and T}",
      journal = {\araa},
         year = 2005,
        month = sep,
       volume = {43},
       number = {1},
        pages = {195-245},
          doi = {10.1146/annurev.astro.42.053102.134017},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ARA\&A..43..195K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morley+2014,
       author = {{Morley}, Caroline V. and {Marley}, Mark S. and {Fortney}, Jonathan J. and {Lupu}, Roxana},
        title = "{Spectral Variability from the Patchy Atmospheres of T and Y Dwarfs}",
      journal = {\apjl},
     keywords = {brown dwarfs, planets and satellites: atmospheres, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = jul,
       volume = {789},
       number = {1},
          eid = {L14},
        pages = {L14},
          doi = {10.1088/2041-8205/789/1/L14},
archivePrefix = {arXiv},
       eprint = {1406.0863},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...789L..14M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morley+2012,
       author = {{Morley}, Caroline V. and {Fortney}, Jonathan J. and {Marley}, Mark S. and {Visscher}, Channon and {Saumon}, Didier and {Leggett}, S.~K.},
        title = "{Neglected Clouds in T and Y Dwarf Atmospheres}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = sep,
       volume = {756},
       number = {2},
          eid = {172},
        pages = {172},
          doi = {10.1088/0004-637X/756/2/172},
archivePrefix = {arXiv},
       eprint = {1206.4313},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756..172M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Visscher+2010,
       author = {{Visscher}, Channon and {Lodders}, Katharina and {Fegley}, Jr., Bruce},
        title = "{Atmospheric Chemistry in Giant Planets, Brown Dwarfs, and Low-mass Dwarf Stars. III. Iron, Magnesium, and Silicon}",
      journal = {\apj},
     keywords = {astrochemistry, brown dwarfs, planets and satellites: individual: Jupiter, stars: individual: Gliese 229B HD 209458, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jun,
       volume = {716},
       number = {2},
        pages = {1060-1075},
          doi = {10.1088/0004-637X/716/2/1060},
archivePrefix = {arXiv},
       eprint = {1001.3639},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...716.1060V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burgasser+2002,
       author = {{Burgasser}, Adam J. and {Kirkpatrick}, J. Davy and {Brown}, Michael E. and {Reid}, I. Neill and {Burrows}, Adam and {Liebert}, James and {Matthews}, Keith and {Gizis}, John E. and {Dahn}, Conard C. and {Monet}, David G. and {Cutri}, Roc M. and {Skrutskie}, Michael F.},
        title = "{The Spectra of T Dwarfs. I. Near-Infrared Data and Spectral Classification}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs, Techniques: Spectroscopic, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {421-451},
          doi = {10.1086/324033},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108452},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..421B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett+2002,
       author = {{Leggett}, S.~K. and {Golimowski}, David A. and {Fan}, Xiaohui and {Geballe}, T.~R. and {Knapp}, G.~R. and {Brinkmann}, J. and {Csabai}, Istv{\'a}n and {Gunn}, James E. and {Hawley}, Suzanne L. and {Henry}, Todd J. and {Hindsley}, Robert and {Ivezi{\'c}}, {\v{Z}}eljko and {Lupton}, Robert H. and {Pier}, Jeffrey R. and {Schneider}, Donald P. and {Smith}, J. Allyn and {Strauss}, Michael A. and {Uomoto}, Alan and {York}, D.~G.},
        title = "{Infrared Photometry of Late-M, L, and T Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {452-465},
          doi = {10.1086/324037},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108435},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..452L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Radigan+2014b,
       author = {{Radigan}, Jacqueline},
        title = "{An Independent Analysis of the Brown Dwarf Atmosphere Monitoring (BAM) Data: Large-amplitude Variability is Rare Outside the L/T Transition}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = dec,
       volume = {797},
       number = {2},
          eid = {120},
        pages = {120},
          doi = {10.1088/0004-637X/797/2/120},
archivePrefix = {arXiv},
       eprint = {1408.5919},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...797..120R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Burgasser-2011,
       author = {{Burgasser}, A.~J.},
        title = "{The Brown Dwarf-Exoplanet Connection}",
    booktitle = {Molecules in the Atmospheres of Extrasolar Planets},
         year = 2011,
       editor = {{Beaulieu}, J.~P. and {Dieters}, S. and {Tinetti}, G.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {450},
        month = dec,
        pages = {113},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ASPC..450..113B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodders+2002,
       author = {{Lodders}, Katharina and {Fegley}, Bruce},
        title = "{Atmospheric Chemistry in Giant Planets, Brown Dwarfs, and Low-Mass Dwarf Stars. I. Carbon, Nitrogen, and Oxygen}",
      journal = {\icarus},
         year = 2002,
        month = feb,
       volume = {155},
       number = {2},
        pages = {393-424},
          doi = {10.1006/icar.2001.6740},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002Icar..155..393L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang+2018a,
       author = {{Zhang}, Z.~H. and {Pinfield}, D.~J. and {G{\'a}lvez-Ortiz}, M.~C. and {Homeier}, D. and {Burgasser}, A.~J. and {Lodieu}, N. and {Mart{\'\i}n}, E.~L. and {Zapatero Osorio}, M.~R. and {Allard}, F. and {Jones}, H.~R.~A. and {Smart}, R.~L. and {L{\'o}pez Mart{\'\i}}, B. and {Burningham}, B. and {Rebolo}, R.},
        title = "{Primeval very low-mass stars and brown dwarfs - III. The halo transitional brown dwarfs}",
      journal = {\mnras},
     keywords = {brown dwarfs, stars: chemically peculiar, stars: individual: ULAS J020858.62+020657.0, ULAS J135058.85+081506.8, ULAS J230711.01+014447.1, stars: Population II, subdwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = sep,
       volume = {479},
       number = {1},
        pages = {1383-1391},
          doi = {10.1093/mnras/sty1352},
archivePrefix = {arXiv},
       eprint = {1805.08033},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479.1383Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang+2018b,
       author = {{Zhang}, Z.~H. and {Galvez-Ortiz}, M.~C. and {Pinfield}, D.~J. and {Burgasser}, A.~J. and {Lodieu}, N. and {Jones}, H.~R.~A. and {Mart{\'\i}n}, E.~L. and {Burningham}, B. and {Homeier}, D. and {Allard}, F. and {Zapatero Osorio}, M.~R. and {Smith}, L.~C. and {Smart}, R.~L. and {L{\'o}pez Mart{\'\i}}, B. and {Marocco}, F. and {Rebolo}, R.},
        title = "{Primeval very low-mass stars and brown dwarfs - IV. New L subdwarfs, Gaia astrometry, population properties, and a blue brown dwarf binary}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, brown dwarfs, stars: chemically peculiar, stars: Population II, stars: subdwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = nov,
       volume = {480},
       number = {4},
        pages = {5447-5474},
          doi = {10.1093/mnras/sty2054},
archivePrefix = {arXiv},
       eprint = {1807.10560},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.5447Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley+2002,
       author = {{Marley}, Mark S. and {Seager}, S. and {Saumon}, D. and {Lodders}, Katharina and {Ackerman}, Andrew S. and {Freedman}, Richard S. and {Fan}, Xiaohui},
        title = "{Clouds and Chemistry: Ultracool Dwarf Atmospheric Properties from Optical and Infrared Colors}",
      journal = {\apj},
     keywords = {Stars: Atmospheres, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2002,
        month = mar,
       volume = {568},
       number = {1},
        pages = {335-342},
          doi = {10.1086/338800},
archivePrefix = {arXiv},
       eprint = {astro-ph/0105438},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...568..335M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skemer+2014,
       author = {{Skemer}, Andrew J. and {Marley}, Mark S. and {Hinz}, Philip M. and {Morzinski}, Katie M. and {Skrutskie}, Michael F. and {Leisenring}, Jarron M. and {Close}, Laird M. and {Saumon}, Didier and {Bailey}, Vanessa P. and {Briguglio}, Runa and {Defrere}, Denis and {Esposito}, Simone and {Follette}, Katherine B. and {Hill}, John M. and {Males}, Jared R. and {Puglisi}, Alfio and {Rodigas}, Timothy J. and {Xompero}, Marco},
        title = "{Directly Imaged L-T Transition Exoplanets in the Mid-infrared}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, planets and satellites: gaseous planets, stars: individual: HR 8799 2M1207 b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = sep,
       volume = {792},
       number = {1},
          eid = {17},
        pages = {17},
          doi = {10.1088/0004-637X/792/1/17},
archivePrefix = {arXiv},
       eprint = {1311.2085},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792...17S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Daemgen+2017,
       author = {{Daemgen}, Sebastian and {Todorov}, Kamen and {Silva}, Jasmin and {Hand}, Derek and {Garcia}, Eugenio V. and {Currie}, Thayne and {Burrows}, Adam and {Stassun}, Keivan G. and {Ratzka}, Thorsten and {Debes}, John H. and {Lafreniere}, David and {Jayawardhana}, Ray and {Correia}, Serge},
        title = "{Mid-infrared characterization of the planetary-mass companion ROXs 42B b}",
      journal = {\aap},
     keywords = {stars: pre-main sequence, planets and satellites: individual: ROXS42Bb, planets and satellites: detection, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A65},
        pages = {A65},
          doi = {10.1051/0004-6361/201629949},
archivePrefix = {arXiv},
       eprint = {1702.06549},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A\&A...601A..65D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodieu+2018,
       author = {{Lodieu}, N. and {Zapatero Osorio}, M.~R. and {B{\'e}jar}, V.~J.~S. and {Pe{\~n}a Ram{\'\i}rez}, K.},
        title = "{The optical + infrared L dwarf spectral sequence of young planetary-mass objects in the Upper Scorpius association}",
      journal = {\mnras},
     keywords = {techniques: photometric, techniques: spectroscopic, surveys, brown dwarfs, stars: low-mass, stars: luminosity function, mass function, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {473},
       number = {2},
        pages = {2020-2059},
          doi = {10.1093/mnras/stx2279},
archivePrefix = {arXiv},
       eprint = {1709.02139},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.2020L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Nasedkin+2023,
       author = {{Nasedkin}, E. and {Molli{\`e}re}, P. and {Wang}, J. and {Cantalloube}, F. and {Kreidberg}, L. and {Pueyo}, L. and {Stolker}, T. and {Vigan}, A.},
        title = "{Impacts of high-contrast image processing on atmospheric retrievals}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, methods: data analysis, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = oct,
       volume = {678},
          eid = {A41},
        pages = {A41},
          doi = {10.1051/0004-6361/202346585},
archivePrefix = {arXiv},
       eprint = {2308.01343},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A\&A...678A..41N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Xuan+2022,
       author = {{Xuan}, Jerry W. and {Wang}, Jason and {Ruffio}, Jean-Baptiste and {Knutson}, Heather and {Mawet}, Dimitri and {Molli{\`e}re}, Paul and {Kolecki}, Jared and {Vigan}, Arthur and {Mukherjee}, Sagnick and {Wallack}, Nicole and {Wang}, Ji and {Baker}, Ashley and {Bartos}, Randall and {Blake}, Geoffrey A. and {Bond}, Charlotte Z. and {Bryan}, Marta and {Calvin}, Benjamin and {Cetre}, Sylvain and {Chun}, Mark and {Delorme}, Jacques-Robert and {Doppmann}, Greg and {Echeverri}, Daniel and {Finnerty}, Luke and {Fitzgerald}, Michael P. and {Horstman}, Katelyn and {Inglis}, Julie and {Jovanovic}, Nemanja and {L{\'o}pez}, Ronald and {Martin}, Emily C. and {Morris}, Evan and {Pezzato}, Jacklyn and {Ragland}, Sam and {Ren}, Bin and {Ruane}, Garreth and {Sappey}, Ben and {Schofield}, Tobias and {Skemer}, Andrew and {Venenciano}, Taylor and {Wallace}, J. Kent and {Wizinowich}, Peter},
        title = "{A Clear View of a Cloudy Brown Dwarf Companion from High-resolution Spectroscopy}",
      journal = {\apj},
     keywords = {Brown dwarfs, Atmospheric composition, High resolution spectroscopy, High angular resolution, Atmospheric clouds, Exoplanet atmospheric composition, 185, 2120, 2096, 2167, 2180, 2021, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = oct,
       volume = {937},
       number = {2},
          eid = {54},
        pages = {54},
          doi = {10.3847/1538-4357/ac8673},
archivePrefix = {arXiv},
       eprint = {2208.01657},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...937...54X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Xuan+2024,
       author = {{Xuan}, Jerry W. and {Hsu}, Chih-Chun and {Finnerty}, Luke and {Wang}, Jason and {Ruffio}, Jean-Baptiste and {Zhang}, Yapeng and {Knutson}, Heather A. and {Mawet}, Dimitri and {Mamajek}, Eric E. and {Inglis}, Julie and {Wallack}, Nicole L. and {Bryan}, Marta L. and {Blake}, Geoffrey A. and {Molli{\`e}re}, Paul and {Hejazi}, Neda and {Baker}, Ashley and {Bartos}, Randall and {Calvin}, Benjamin and {Cetre}, Sylvain and {Delorme}, Jacques-Robert and {Doppmann}, Greg and {Echeverri}, Daniel and {Fitzgerald}, Michael P. and {Jovanovic}, Nemanja and {Liberman}, Joshua and {L{\'o}pez}, Ronald A. and {Morris}, Evan and {Pezzato}, Jacklyn and {Sappey}, Ben and {Schofield}, Tobias and {Skemer}, Andrew and {Wallace}, J. Kent and {Wang}, Ji and {Agrawal}, Shubh and {Horstman}, Katelyn},
        title = "{Are These Planets or Brown Dwarfs? Broadly Solar Compositions from High-resolution Atmospheric Retrievals of {\ensuremath{\sim}}10{\textendash}30 M $_{Jup}$ Companions}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Brown dwarfs, High resolution spectroscopy, Exoplanet atmospheric composition, Atmospheric clouds, Exoplanet formation, Substellar companion stars, 487, 185, 2096, 2021, 2180, 492, 1648, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = jul,
       volume = {970},
       number = {1},
          eid = {71},
        pages = {71},
          doi = {10.3847/1538-4357/ad4796},
archivePrefix = {arXiv},
       eprint = {2405.13128},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...970...71X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ruffio+2024,
       author = {{Ruffio}, Jean-Baptiste and {Perrin}, Marshall D. and {Hoch}, Kielan K.~W. and {Kammerer}, Jens and {Konopacky}, Quinn M. and {Pueyo}, Laurent and {Madurowicz}, Alex and {Rickman}, Emily and {Theissen}, Christopher A. and {Agrawal}, Shubh and {Greenbaum}, Alexandra Z. and {Miles}, Brittany E. and {Barman}, Travis S. and {Balmer}, William O. and {Llop-Sayson}, Jorge and {Girard}, Julien H. and {Rebollido}, Isabel and {Soummer}, R{\'e}mi and {Allen}, Natalie H. and {Anderson}, Jay and {Beichman}, Charles A. and {Bellini}, Andrea and {Bryden}, Geoffrey and {Espinoza}, N{\'e}stor and {Glidden}, Ana and {Huang}, Jingcheng and {Lewis}, Nikole K. and {Libralato}, Mattia and {Louie}, Dana R. and {Sohn}, Sangmo Tony and {Seager}, Sara and {van der Marel}, Roeland P. and {Wakeford}, Hannah R. and {Watkins}, Laura L. and {Ygouf}, Marie and {Mountain}, C. Matt},
        title = "{JWST-TST High Contrast: Achieving Direct Spectroscopy of Faint Substellar Companions Next to Bright Stars with the NIRSpec Integral Field Unit}",
      journal = {\aj},
     keywords = {Direct imaging, High contrast spectroscopy, High resolution spectroscopy, Near infrared astronomy, Extrasolar gaseous giant planets, 387, 2370, 2096, 1093, 509, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = aug,
       volume = {168},
       number = {2},
          eid = {73},
        pages = {73},
          doi = {10.3847/1538-3881/ad5281},
archivePrefix = {arXiv},
       eprint = {2310.09902},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....168...73R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lagrange+2009,
       author = {{Lagrange}, A. -M. and {Gratadour}, D. and {Chauvin}, G. and {Fusco}, T. and {Ehrenreich}, D. and {Mouillet}, D. and {Rousset}, G. and {Rouan}, D. and {Allard}, F. and {Gendron}, {\'E}. and {Charton}, J. and {Mugnier}, L. and {Rabou}, P. and {Montri}, J. and {Lacombe}, F.},
        title = "{A probable giant planet imaged in the {\ensuremath{\beta}} Pictoris disk. VLT/NaCo deep L'-band imaging}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, stars: early-type, stars: planetary systems, stars: individual: {\ensuremath{\beta}} Pic, Astrophysics},
         year = 2009,
        month = jan,
       volume = {493},
       number = {2},
        pages = {L21-L25},
          doi = {10.1051/0004-6361:200811325},
archivePrefix = {arXiv},
       eprint = {0811.3583},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A\&A...493L..21L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Artigau+2015,
       author = {{Artigau}, {\'E}tienne and {Gagn{\'e}}, Jonathan and {Faherty}, Jacqueline and {Malo}, Lison and {Naud}, Marie-Eve and {Doyon}, Ren{\'e} and {Lafreni{\`e}re}, David and {Beletsky}, Yuri},
        title = "{BANYAN. VI. Discovery of a Companion at the Brown Dwarf/Planet-Mass Limit to a Tucana-Horologium M Dwarf}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: late-type, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jun,
       volume = {806},
       number = {2},
          eid = {254},
        pages = {254},
          doi = {10.1088/0004-637X/806/2/254},
archivePrefix = {arXiv},
       eprint = {1505.01747},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806..254A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chauvin+2005,
       author = {{Chauvin}, G. and {Lagrange}, A. -M. and {Zuckerman}, B. and {Dumas}, C. and {Mouillet}, D. and {Song}, I. and {Beuzit}, J. -L. and {Lowrance}, P. and {Bessell}, M.~S.},
        title = "{A companion to AB Pic at the planet/brown dwarf boundary}",
      journal = {\aap},
     keywords = {Astrophysics},
         year = 2005,
        month = aug,
       volume = {438},
       number = {3},
        pages = {L29-L32},
          doi = {10.1051/0004-6361:200500111},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504658},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A\&A...438L..29C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cushing+2006,
       author = {{Cushing}, Michael C. and {Roellig}, Thomas L. and {Marley}, Mark S. and {Saumon}, D. and {Leggett}, S.~K. and {Kirkpatrick}, J. Davy and {Wilson}, John C. and {Sloan}, G.~C. and {Mainzer}, Amy K. and {Van Cleve}, Jeff E. and {Houck}, James R.},
        title = "{A Spitzer Infrared Spectrograph Spectral Sequence of M, L, and T Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = sep,
       volume = {648},
       number = {1},
        pages = {614-628},
          doi = {10.1086/505637},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605639},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...648..614C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Snellen+Brown-2018,
       author = {{Snellen}, I.~A.~G. and {Brown}, A.~G.~A.},
        title = "{The mass of the young planet Beta Pictoris b through the astrometric motion of its host star}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = aug,
       volume = {2},
        pages = {883-886},
          doi = {10.1038/s41550-018-0561-6},
archivePrefix = {arXiv},
       eprint = {1808.06257},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..883S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brandt+2019,
       author = {{Brandt}, Timothy D. and {Dupuy}, Trent J. and {Bowler}, Brendan P.},
        title = "{Precise Dynamical Masses of Directly Imaged Companions from Relative Astrometry, Radial Velocities, and Hipparcos-Gaia DR2 Accelerations}",
      journal = {\aj},
     keywords = {astrometry, brown dwarfs, celestial mechanics, methods: statistical, stars: low-mass, white dwarfs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = oct,
       volume = {158},
       number = {4},
          eid = {140},
        pages = {140},
          doi = {10.3847/1538-3881/ab04a8},
archivePrefix = {arXiv},
       eprint = {1811.07285},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....158..140B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Franson+2022,
       author = {{Franson}, Kyle and {Bowler}, Brendan P. and {Brandt}, Timothy D. and {Dupuy}, Trent J. and {Tran}, Quang H. and {Brandt}, G. Mirek and {Li}, Yiting and {Kraus}, Adam L.},
        title = "{Dynamical Mass of the Young Substellar Companion HD 984 B}",
      journal = {\aj},
     keywords = {185, 387, 1175, 1332, 80, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = feb,
       volume = {163},
       number = {2},
          eid = {50},
        pages = {50},
          doi = {10.3847/1538-3881/ac35e8},
archivePrefix = {arXiv},
       eprint = {2111.01803},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163...50F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Franson+2023,
       author = {{Franson}, Kyle and {Bowler}, Brendan P.},
        title = "{Dynamical Mass of the Young Brown Dwarf Companion PZ Tel B}",
      journal = {\aj},
     keywords = {Brown dwarfs, Direct imaging, Astrometry, Orbit determination, 185, 387, 80, 1175, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2023,
        month = jun,
       volume = {165},
       number = {6},
          eid = {246},
        pages = {246},
          doi = {10.3847/1538-3881/acca18},
archivePrefix = {arXiv},
       eprint = {2304.01302},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....165..246F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Currie+2023,
       author = {{Currie}, Thayne and {Brandt}, G. Mirek and {Brandt}, Timothy D. and {Lacy}, Brianna and {Burrows}, Adam and {Guyon}, Olivier and {Tamura}, Motohide and {Liu}, Ranger Y. and {Sagynbayeva}, Sabina and {Tobin}, Taylor and {Chilcote}, Jeffrey and {Groff}, Tyler and {Marois}, Christian and {Thompson}, William and {Murphy}, Simon J. and {Kuzuhara}, Masayuki and {Lawson}, Kellen and {Lozi}, Julien and {Deo}, Vincent and {Vievard}, Sebastien and {Skaf}, Nour and {Uyama}, Taichi and {Jovanovic}, Nemanja and {Martinache}, Frantz and {Kasdin}, N. Jeremy and {Kudo}, Tomoyuki and {McElwain}, Michael and {Janson}, Markus and {Wisniewski}, John and {Hodapp}, Klaus and {Nishikawa}, Jun and {He{\l}miniak}, Krzysztof and {Kwon}, Jungmi and {Hayashi}, Masahiko},
        title = "{Direct imaging and astrometric detection of a gas giant planet orbiting an accelerating star}",
      journal = {Science},
     keywords = {ASTRONOMY; PLANET SCI, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = apr,
       volume = {380},
       number = {6641},
        pages = {198-203},
          doi = {10.1126/science.abo6192},
archivePrefix = {arXiv},
       eprint = {2212.00034},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023Sci...380..198C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









